Lion Secretly Solves Constrained Optimization: As Lyapunov Predicts

Lion (Evolved Sign Momentum), a new optimizer discovered through program search, has shown promising results in training large AI models. It performs comparably or favorably to AdamW but with greater memory efficiency. As we can expect from the results of a random search program, Lion incorporates elements from several existing algorithms, including signed momentum, decoupled weight decay, Polak, and Nesterov momentum, but does not fit into any existing category of theoretically grounded optimizers. Thus, even though Lion appears to perform well as a general-purpose optimizer for a wide range of tasks, its theoretical basis remains uncertain. This lack of theoretical clarity limits opportunities to further enhance and expand Lion's efficacy. This work aims to demystify Lion. Based on both continuous-time and discrete-time analysis, we demonstrate that Lion is a theoretically novel and principled approach for minimizing a general loss function $f(x)$ while enforcing a bound constraint $\|x\|_\infty \leq 1/\lambda$. Lion achieves this through the incorporation of decoupled weight decay, where $\lambda$ represents the weight decay coefficient. Our analysis is made possible by the development of a new Lyapunov function for the Lion updates. It applies to a broader family of Lion-$\kappa$ algorithms, where the $\text{sign}(\cdot)$ operator in Lion is replaced by the subgradient of a convex function $\kappa$, leading to the solution of a general composite optimization problem of $\min_x f(x) + \kappa^*(x)$. Our findings provide valuable insights into the dynamics of Lion and pave the way for further improvements and extensions of Lion-related algorithms.

==> content/backup_experiment.tex <==

\section{Experiments on Different $\phi$}
\label{sec:experiment}
This section provides a preliminary investigation on the behaviors of \lion{}-$\phi$ with different $\phi$. We experiment with the $\phi$s listed in Table~\ref{tab:phiexamples} on the toy example shown in Figure~\ref{fig:traj-1} to confirm the behavior follows exactly as what the theory predicts. Then we focus on the \lion{}-$\ell_p$ optimizer with general $p \in [1, 2]$ since it is the most straightforward extension of the original \lion{} (with $p=1$).

\subsection{\lion{}-$\phi$s on the Toy Example}
In the following, we plot the behavior of different \lion{}-$\phi$s on the toy example shown in Figure~\ref{fig:traj-1}. For each $\phi$, we draw the optimization trajectory using the corresponding optimizer, the loss $f(x)$, and the corresponding constraint (e.g., the norm of $x$) v.s. iteration. The results are shown in Figure~\ref{fig:different_k}.

\paragraph{Observation} From Figure~\ref{fig:different_k}, one can observe that for $\phi(x)= ||x||_2$, the constraint is a circle. For $\phi(x) = \sum_i \max(|x_i| - e, 0)$, the same $\ell_infty$ constraint applies while the solution tends to be sparse. For $\phi(x) = \sum_{i \leq i^{cut}} |x_{(i)}|$, the constraint is a combination of $\ell_\infty$ and $\ell_1$ constraints. For $\phi(x) = \sum_i \text{huber}_e(x_i)$, the constraint is an $\ell_infty$ constraint while there is an additional $\ell_2$ regularization effect. All optimization trajectories closely match what the theory predicts. 

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/different_k.pdf}
    \caption{The behavior of \lion{}-$\phi$ with different $\phi$s from Table~\ref{tab:phiexamples}.}
    \label{fig:different_k}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \includegraphics[width=.9\textwidth]{figures/quadratic_l2.png}
%     \vspace{-1\baselineskip}
%     \caption{Trajectories of Lion-$\ell_2$  on 2D function $f(x) = (x_1 - 1.5)^2 + x_2^2$,  with $\lambda = 1.5$ (blue), and $\lambda = 0.5$ (green). The circles in the first figure represent the constraint set $\norm{x}_2 \leq 1/\lambda$.}
%     \label{fig:traj-4}
% \end{figure}

% \paragraph{$\phi = \sum_i \max(\abs{x_i} - e, 0)$}
% This $\phi$ corresponds to \mycircle{3} in Table~\ref{tab:phiexamples} and amounts to solve $\min f(x) + e \norm{x}_1 ~~s.t.~~  \norm{x}_\infty\leq 1$.
% \begin{figure}[h!]
%     \centering
%     % \includegraphics[width=0.4\textwidth]{figures/l1_norm.pdf}
%     % \includegraphics[width=0.4\textwidth]{figures/l2_norm.pdf}
%     \includegraphics[width=.9\textwidth]{figures/max.png}
%     % \includegraphics[width=.9\textwidth]{figures/quadratic2.pdf}
%     \vspace{-1\baselineskip}
%     \caption{The red dot (\red{$\bullet$}) represents the minimal point of  $\min_x f(x) + e\|x\|_1$. If using vanilla Lion, as shown in Figure~\ref{fig:traj-1}, it converges to the magenta dot ({\color{magenta}$\bullet$}), which is the optimal point of $\min_x f(x)$} 
%     \label{fig:traj-3}
% \end{figure}


% % Adjust space as needed

% \begin{figure}[h]
%     \centering
%     % \includegraphics[width=0.4\textwidth]{figures/l1_norm.pdf}
%     % \includegraphics[width=0.4\textwidth]{figures/l2_norm.pdf}
%     \includegraphics[width=.9\textwidth]{figures/sort.png}
%     % \includegraphics[width=.9\textwidth]{figures/quadratic2.pdf}
%     \vspace{-1\baselineskip}
%     \caption{Lion-$\phi$ with 
% the sorting norm function \mycircle{4} in Table~\ref{tab:phiexamples}, 
% which amounts to solve $\min_x f(x) \ s.t.\ \|x\|_1 \leq i^{cut}/\lambda, \ \|x\|_\infty \leq 1/\lambda$. The dashed blue box ({\color{blue}$\Box$}) represents the constraint $\|x\|_1 \leq i^{cut}/\lambda$, where $i^{cut} = 2, \lambda = 0.45$, while the dashed green box ({\color{green}$\Box$}) is for  $i^{cut} = 2, \lambda = 1.5$.} 
%     \label{fig:traj-5}
% \end{figure}
% \vspace{-2mm} % Adjust space as needed


% \begin{figure}[H]
%     \centering
%     % \includegraphics[width=0.4\textwidth]{figures/l1_norm.pdf}
%     % \includegraphics[width=0.4\textwidth]{figures/l2_norm.pdf}
%     \includegraphics[width=.9\textwidth]{figures/huber.png}
%     % \includegraphics[width=.9\textwidth]{figures/quadratic2.pdf}
%     \vspace{-1\baselineskip}
%     \caption{Lion-$\phi$ with 
% the Huber function \mycircle{5} in Table~\ref{tab:phiexamples}, 
% which amounts to solve $\min_x f(x) + \frac{\lambda e}{2}\|x\|_2^2$. The red dot (\red{$\bullet$}) represents the minimal point of  $\min_x f(x) + \frac{\lambda e}{2}\|x\|_2^2$. If using vanilla Lion, as shown in Figure~\ref{fig:traj-1}, it converges to the magenta dot ({\color{magenta}$\bullet$}), which is the optimal point of $\min_x f(x)$}
%     % \qq{How to see the effect of L2 regulariztation here?}}
%     % \qq{change the other titles to this style.}
%     %In Table~\ref{tab:phiexamples}, huber function's corresponding loss \mycircle{5} will introduce an extra $\ell_2$ norm term to objective function.}
%     \label{fig:traj-2}
% \end{figure}

\subsection{Lion-$\ell_p$ for ImageNet and Language Modeling}
Lion-$\ell_p$ corresponds to $\phi(x) = \norm{x}_{p}$, $p\geq 1$ and amounts to solving $\min_x f(x)~ s.t. ~\norm{x}_q \leq 1/\lambda$ where $1/p + 1/q =1$. 

% Figure~\ref{fig:ViT_loss_norm} and \ref{fig:ImgNet_verify}  
% verifies the $\ell_q$ constraint for $p = 1$ and $p = 2$. 
% \bo{Please just put the loss v.s. iteration plot}

% \emph{Lion With Grouped $\ell_p$ Norm}
% Figure~\ref{fig:loss_pow} shows the loss curve of 
% Lion-$\phi$ with grouped $\ell_p$ norm for a range of  $p$ in $[1,2]$ on ResNet and GPT-2.  The grouped $\ell_p$ norm 
% fits naturally in deep neural networks in which the parameters are naturally grouped. 
% We find that the result with different $p$ varies for different models. Larger $p$ (Lion-$\ell_2$) tends to perform better on ResNet, while smaller $p$ (Lion-$\ell_1$) performs better on GPT-2. This shows the promise of gaining improvement by search problem-specific $p$ in practice.

% \begin{figure}[h!]
%     \centering
%     % \includegraphics[width=0.4\textwidth]{figures/l1_norm.pdf}
%     % \includegraphics[width=0.4\textwidth]{figures/l2_norm.pdf}
%     \includegraphics[width=.95\textwidth]{figures/loss_norm.pdf}\vspace{-.5\baselineskip}
%     % \begin{tabular}{cccc}
%     % ~~~~~~~~ \small Lion-$\ell_1$ &\hfill~~~~~~~~~~~~~~~~~~~~   ~~
%     % \small Lion-$\ell_2$  & \hfill ~~~~~~~~~~~~~~~~~~~~~    
%     % \small Lion-$ \ell_1$ & \hfill ~~~~~~~~~~~~~~~~~~~~ 
%     % \small Lion-$\ell_2$ 
%     % \end{tabular}
%     \vspace{.5\baselineskip}
%     % \caption{
%     % Results of Lion-$\ell_p$  
%     % with $\phi(x)=\norm{x}_p$ imposes the bound on the dual norm $\norm{x}_q\leq 1/\lambda$. From Left to right: 1) $\ell_\infty$ norm curve of parameters of ViT model, 2) normalized (to 1) $\ell_2$ norm curve of parameters of ViT model, 3) Loss curve of ViT using Lion-$\ell_1$, 4) Loss curve of ViT using Lion-$\ell_2$
%     % Results shown for 
%     % $p\in\{0,1\}$ and $\lambda \in \{2,4\}$ on ViT~\citep{dosovitskiy2020image} on imageNet~\citep{ILSVRC15} 
%     %\qq{Change $Lion-\ell_1$ to $Lion$-$\ell_1$ in the figure. Too much space around $-$.} \blue{done}
%     %\qq{should we show the loss curve as well?}\blue{the above 4 figures are verification of our theory, }
%     %\qq{we can add some loss curve on real examples.}
%     %\qq{Techinically, it only veri}
%          %Verification of the implicit constraint mechanism of Lion-\( \phi \) on ImageNet. The function \( \phi(x) \) is characterized by \( \norm{x}_p \). \textbf{Left}: \( p = 1 \)( Lion). \textbf{Middle}: \( p = 2 \)(Lion-$\ell_2$ (model)) \textbf{Right}: \( p = 2 \)(Lion-$\ell_2$ (model))
%     % }

%     \caption{
% Results from applying Lion-$\ell_p$ constraints on the Vision Transformer (ViT) model~\cite{dosovitskiy2020image} trained on ImageNet~\cite{ILSVRC15}. Using $\phi(x) = \norm{x}_p$, a bound on the dual norm is set as $\norm{x}_q\leq 1/\lambda$. Displayed from left to right are: 
% 1) $\ell_\infty$ norm curve of ViT parameters,
% 2) Loss curve under Lion-$\ell_1$ constraint, 
% 3) Normalized $\ell_2$ norm curve of ViT parameters (max value = 1),
% 4) Loss curve under Lion-$\ell_2$ constraint. 
% Studies conducted for $p \in \{0,1\}$ and $\lambda \in \{2,4\}$. Referenced works: ViT~\citep{dosovitskiy2020image}, ImageNet~\citep{ILSVRC15}. 
% % \qq{the axis labels of figure 1,2 are not the same style as 3,4. Rearrange, so Figure 1,2 are L1, and 3,4 are L2?} 
% }
%     % \qq{how about adding the Lion-$\ell_1$ names I added directly to the images? did not align well} \qq{wd to $\lambda$?}
%     \label{fig:ViT_loss_norm}
% \end{figure}

% %\vspace{-2mm} % Adjust space as needed

% \begin{figure}[H]
%     \centering
%     % \includegraphics[width=0.4\textwidth]{figures/l1_norm.pdf}
%     % \includegraphics[width=0.4\textwidth]{figures/l2_norm.pdf}
%     \includegraphics[width=.95\textwidth]{figures/norm_of_param.pdf}
%     % \begin{tabular}{cccc}
%     % ~~~~~~~~ \small Lion-$\ell_1$ &\hfill~~~~~~~~~~~~~~~~~~~~   ~~
%     % \small Lion-$\ell_2$  & \hfill ~~~~~~~~~~~~~~~~~~~~~    
%     % \small Lion-$ \ell_1$ & \hfill ~~~~~~~~~~~~~~~~~~~~ 
%     % \small Lion-$\ell_2$ 
%     % \end{tabular}
%     % \vspace{.5\baselineskip}
%     \caption{
%     Results of Lion-$\ell_p$  
%     with $\phi(x)=\norm{x}_p$ imposes the bound on the dual norm $\norm{x}_q\leq 1/\lambda$. 
%     Results shown for 
%     $p\in\{0,1\}$ and $\lambda \in \{5,10\}$ on ViT~\citep{dosovitskiy2020image} on imageNet~\citep{ILSVRC15} and GPT-2~\citep{radford2019language} 
%     \qq{Figure a,b is already included in Figure 9. It would be more natural to show c d and the loss curve for for GPT2}
%     }
%     \label{fig:ImgNet_verify}
% \end{figure}

% \vspace{-4mm} % Adjust space as needed

\begin{figure}[H]
    \centering
    \includegraphics[width=.36\textwidth]{figures/imgnet_loss_pow.pdf}
    \vspace{.5\baselineskip}
    \includegraphics[width=.5\textwidth]{figures/train_loss_llm.pdf}
    \caption{
    Training loss curve of Lion-\( \phi \) on ResNet-50 
    on ImageNet (left) and GPT-2 (right), where \( \phi(x) \) is defined by the group \( \ell_p \) norm as \( \norm{x}_{\mathcal G, p} \). Different values of \( p \) are explored.} 
    \label{fig:loss_pow}
\end{figure}


==> content/dist_lion.tex <==
\section{Distributed \lion{}}
Because of the binary updates, the \lion{} optimizer seamlessly integrates into distributed optimization. This section demonstrates how easily distributed \lion{} can be implemented and how it surpasses contemporary gradient compression methods right out of the gate.

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/test_acc_distributed.pdf}
    \includegraphics[width=\textwidth]{figures/train_loss_distributed.pdf}
    \caption{Train loss and test acuracy of distributed Lion, global Lion, deep gradient compressing, and signum on CIFAR-10. Number of workers is from 8 to 32 with total batch size from 128 to 4096. 
    % \qq{the figures are too small, we do not need these many plots}
    }
    \label{fig:distribut_}
\end{figure}
We consider a more general Hamiltonian that  introduces $N$  copies momentum vectors: 
$$
H(x, m_1\ldots m_k) 
= f(x) + \sum_{i=1}^k 
\phi_i(m_i), 
$$
where $m_i \in \RR^d$, and 
each $\phi_i\colon \RR^d \to \RR^d$ is  a convex function. 


We introduce $N$ copies of momentums that are averaged: 

\bb
x_{t+1} & = x_t + \epsilon \frac{1}{N} \sum_i u_{t,i} \ant{workers only need to pass binary $u_{t,i}$ to center} \\
m_{t+1,i} & = \beta_{2,i} m_{t,i} + (1-\beta_{2,i} )\dd f(x_t)  \ant{parallel on $i$th worker with sgd} \\
u_{t+1,i} & = \phi'_i(\beta_{1,i} m_{t,i} + (1-\beta_{1,i}) \dd f(x_t)) \ant{parallel on $i$th worker with sgd}
\ee

\paragraph{Mixture of Lions} When using different $\phi'_i $ and $\beta_{1,i}$, $\beta_{2, i}$, this is an ensemble of lion. We  can see if we can search a good algorithm. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{figures/test_acc_distributed.pdf}
%     \includegraphics[width=\textwidth]{figures/train_loss_distributed.pdf}
%     \caption{Train loss and test acuracy of distributed Lion, global Lion, deep gradient compressing, and signum on CIFAR-10. Number of workers is from 1 to 32 with total batch size from 128 to 4096. 
%     \qq{the figures are too small, we do not need these many plots.}}
%     \label{fig:distribut}
% \end{figure}




\paragraph{Communication efficiency} Even if all $\phi$ and $\beta$ are the same, when the gradient $\dd f(x)$ are evaluated with different data from different workers, the $m_i, u_i$ would be different. And when $\phi$ is the sign function, we only need to pass the binary vector $u_i$ for high communication efficiency. 

A simple and quick experiment: compare this with the standard Lion with $\sign(\sum m_i)$ (other than $\sum_i u_i$) which need to pass $m_i$ rather than $u_i$. Hopefully the performance drop is not significant when the batchsize of each individual worker is large, so that the variance between different workers are not large. 

\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth]{figures/dist.png}
\caption{
Train loss of distributed Lion with respect to simulated running time on GPT-2 and ImageNet datasets. The number of workers ranges from 8 to 32. Simulated running time is computed based on floating point operations (flops), assuming a consistent number of flops per unit time for each worker. Notably, the communication cost remains minimal even for larger models. For normalization purposes, the running time with 32 workers is set as the benchmark value of 1. As observed, employing 32 workers offers roughly a 1.5x speedup over 16 workers, and similarly, 16 workers achieve approximately a 1.5x speedup compared to 8 workers.
}
\label{fig:lion_distributed_train_loss}
\end{figure}




==> content/experiments/ablation.tex <==
\section{Ablation Experiments}

==> content/experiments/choice_of_K.tex <==

\begin{figure}{h!}
  \centering
  \includegraphics[width=\textwidth]{figures/linearlion}
  \caption{Lion and the Linear-Lion on ImageNet with ResNet-50 and ViT.}
  \label{fig:linearlion}
\end{figure}

\begin{figure}[t]
    % \centering
    \includegraphics[width=\textwidth]{figures/module-pow.pdf}
    \vspace{-15pt}
    \caption{
    Training loss on ResNet-50 and GPT-2. 
    (a)-(b): Lion-$\phi$ with $\phi(x) =\norm{x}_2$ (Lion-$\ell_2$ (model)) 
    and the  group $\ell_2$ norm $\phi(x) =\norm{x}_{\mathcal G, 2}$ (Lion-$\ell_2$ (module)).  
    (c)-(d): Lion-$\phi$ 
    with group $\ell_p$ norm $\phi(x) = \norm{x}_{\mathcal G, p}$ with different $p$.  
    %(Left)Training loss of ImageNet using model wise Lion-$\ell_2$ (in red) and module wise Lion-$\ell_2$ (in blue) methods. (Right) Training loss of GPT-2 using model wise Lion-$\ell_2$ (in red) and module wise Lion-$\ell_2$ (in blue) methods.
    }
    \label{fig:group}
\end{figure}





\begin{wrapfigure}{r}{.4\textwidth}
    \vspace{-\baselineskip}
    \includegraphics[width=0.4\textwidth]{figures/imgnet_lossl2_eps.pdf}
    \vspace{-25pt}
    \caption{
    Lion-$\phi$ 
    with $\phi(x) = \sqrt{\norm{x}_2^2 + \varepsilon}$ 
    (Middle) Comparison of model-wised Lion-$\ell_2$ and  module-wised Lion-$\ell_2$. 
    (Right) Comparison of module-wised Lion-$\ell_2$ with different $\epsilon$ values.
    }
    \vspace{-\baselineskip}    
    \label{fig:bench}
\end{wrapfigure}



\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/imgNet_pow.pdf}
\caption{
Training loss curve of Lion-\( \phi \) on ImageNet, where \( \phi(x) \) is defined by the group \( \ell_p \) norm as \( \norm{x}_{\mathcal G, p} \). Different values of \( p \) are explored. \textbf{Left}: ResNet-50. \textbf{Right}: ViT-B-32
}
\label{fig:lion_phi_loss}
\end{figure}


\begin{figure}[h!]
    % \centering
    \includegraphics[width=\textwidth]{figures/imgnet_vit_b_32.pdf}
    \includegraphics[width=\textwidth]{figures/imgnet_loss_resnet_lionhdp.pdf}
    \vspace{-15pt}
% \caption{
% Evolution of training loss, Top-1 accuracy, and the magnitude of the group \( \ell_p \) norm across iterations on ImageNet. \textbf{Top}: ViT model. \textbf{Bottom}: ResNet.
% }
\caption{
Evolution of training loss, Top-1 accuracy, and the power \( p \) of the group \( \ell_p \) norm across iterations on ImageNet. \textbf{Top}: Results for the ViT model. \textbf{Bottom}: Results for ResNet. The red curve signifies the employment of the hyper-gradient method for iterative adjustment of \( p \).
}

    \label{fig:training_metrics}
\end{figure}
\newpage
From our presented figures, the influence of different values of \( p \) in the group \( \ell_p \) norm on training dynamics is evident.

\begin{itemize}
    \item \textbf{ResNet Observations} (Figure~\ref{fig:lion_phi_loss}): The optimal performance is achieved with \( p = 2 \), outperforming other values of \( p \) ranging from 1 to 2. As \( p \) transitions from 2 to 1, there's a noticeable retardation in the decrease of the training loss.
    
    \item \textbf{ViT Observations}: Contrasting with the ResNet observations, the ViT model (a Transformer-based architecture) demonstrates its fastest training loss decline at \( p = 2 \). Interestingly, as \( p \) escalates from 1 to 2, the pace at which training loss diminishes slows down. This behavior echoes our findings on another Transformer model, GPT-2 (Figure~\ref{fig:group}), further underscoring a potential architectural trait: for Transformers, a \( p \) value of 2 leads to the most rapid loss reductions.
\end{itemize}

Building upon these observations, in Figure~\ref{fig:training_metrics}, we employed a hypergradient approach to iteratively refine the value of \( p \) based on the current training state, considering factors such as gradient, momentum, and the derivative of loss with respect to \( p \). Notably:
  
\begin{itemize}
    \item \textbf{For ResNet}: The hypergradient method propels \( p \) sharply towards 2. This adaptation yields a swifter loss decline and an accelerated increase in Top-1 accuracy compared to the standard Lion method.
  
    \item \textbf{For ViT}: The hypergradient approach steers \( p \) decisively towards 1. As a result, this method experiences an enhanced loss reduction and Top-1 accuracy elevation compared to Lion-\( \ell_2 \).
\end{itemize}


==> content/experiments/dist_lion.tex <==
\subsection{Distributed Lion}




==> content/experiments/toys.tex <==
\section{Toys}


\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/summary.pdf}
    \vspace{-20pt}
\caption{\textbf{left:} An illustration of how the Hamiltonian and mirror descent jointly influence the optimization (check the dynamics in Eq.\eqref{equ:decomp}). \textbf{right:} The Hamiltonian component, mirror descent component, and the whole vector field of \lion{}-$\phi$ for $f(x) = x^2$ and $\phi(m) = \alpha |m|$ (i.e., the original \lion{}) where $x, m \in \mathbb{R}$.}
    \label{fig:vector-field}
\end{figure}




\begin{figure}[h!]
    % \centering
    \includegraphics[width=\textwidth]{figures/quadratic.pdf}
    \vspace{-20pt}
    \caption{From left to right: iteration trajectories, $f(x)$, $\phi(m)$, and $H(x,m)$ of Lion and Lion-$\phi$ with $\phi(x) = \norm{x}_2$ for minimizing 2D quadratic function. % from the initial value $(4.7, -3.0)$ and initial momentum $m = (0,0)$. Monotonicity of $H(x, m)$: 
    %While the objective $f$ does not decrease monotonically, 
    The Hamiltonian function $H(x, m)$ decreases monotonically, certifying the convergence of the algorithm (upto $\epsilon$ accuracy).  \qq{change plot}
    %decreasing behavior during the optimization process. 
    %As the optimization progresses, $H(x, m)$ decreases, reflecting the convergence of the algorithm.
    }
    \label{fig:quadra}
\end{figure}



==> content/experiments/weight_decay_verify.tex <==


% \paragraph{Experimental Setup} We perform
% \paragraph{Result} Figure xxx shows xxx

% \paragraph{Finding} According to Figure~\ref{}, xxx





\iffalse 
\begin{figure}[h!]
    \centering
    % \includegraphics[width=0.4\textwidth]{figures/l1_norm.pdf}
    % \includegraphics[width=0.4\textwidth]{figures/l2_norm.pdf}
    \includegraphics[width=\textwidth]{figures/norm_of_param.pdf}
    \caption{
        Verification of the implicit constraint mechanism of Lion-\( \phi \) on ImageNet. The function \( \phi(x) \) is characterized by \( \norm{x}_p \). \textbf{Left}: \( p = 1 \)( Lion). \textbf{Middle}: \( p = 2 \)(Lion-$\ell_2$ (model)) \textbf{Right}: \( p = 2 \)(Lion-$\ell_2$ (model))
    }
    \label{fig:ImgNet_verify}
\end{figure}
\fi 


\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/hist.pdf}
    \caption{
        Frequency of network parameters in ResNet on the CIFAR-10 dataset across iterations. 
        \textbf{(a)}: Using Kaiming normal initialization with a weight decay of 20, the parameter values predominantly converge to +0.05 and -0.05, with those exceeding an absolute value of 0.05 highlighted in red. 
        \textbf{(b)}: Similar convergence behavior as in (a) but using Kaiming uniform initialization. 
        \textbf{(c)}: With weight decay set to 0 and Kaiming normal initialization, the magnitude of the parameters consistently increases over iterations. 
        \textbf{(d)}: The evolution of parameter magnitudes without weight decay, utilizing Kaiming uniform initialization.
    }
    \label{fig:hist}
\end{figure}



\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/hist_10.pdf}
    \caption{
        Frequency histograms of ResNet network parameters across iterations, presented in ridge plots with the parameter value on the x-axis and frequency on the y-axis. The plots are staggered across iterations ranging from 0 to 90. Moving from left to right, weight decay ($\lambda$) values are set to 20, 10, and 0. Histograms of parameters exceeding $1/\lambda$ are emphasized in red. 
    }
    \label{fig:hist-row-10}
\end{figure}




\iffalse 
\begin{figure}[h!]
    \centering
    % \includegraphics[width=0.4\textwidth]{figures/l1_norm.pdf}
    % \includegraphics[width=0.4\textwidth]{figures/l2_norm.pdf}
    \includegraphics[width=\textwidth]{figures/hist_norm_10_side.pdf}
    \caption{
        Histograms illustrating the frequency of network parameters from iteration 0 to iteration 250 with a weight decay of 10 (ResNet-18 on CIFAR-10). The red vertical line represents the constraint (feasible) region as described in ~\ref{equ:lionboundc}. 
    }
    \qq{What task is this on? ResNet-18 on CIFAR-10}
  
    \label{fig:hist-row}
\end{figure}
\fi 


\iffalse 
\begin{figure}[h!]
    \centering
    % \includegraphics[width=0.4\textwidth]{figures/l1_norm.pdf}
    % \includegraphics[width=0.4\textwidth]{figures/l2_norm.pdf}
    \includegraphics[width=\textwidth]{figures/quadratic.pdf}
    \caption{
        \textbf{Left}: Optimization trajectory of Lion with different weight decays: 1.5 (green box feasible region) and 0.6 (blue box feasible region). Given the symmetry of the objective function \( f(x) \) about the x-axis, initial points are set symmetrically as well. The feasible regions represent constraint optimization as per ~\ref{equ:opt_solve} and ~\ref{equ:lionboundc}. \textbf{Middle}: Evolution of the objective function \( f(x_1, x_2) = (x_1 - 2)^2 + x_2^2 \) over iterations. \textbf{Right}: Convergence behavior of the conjugate of \( \|x\|_1 \) (represented by \( \|x\|_\infty \)) along iterations, settling to \( 1/\lambda \).
    }
    \label{fig:traj}
\end{figure}

\fi 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The experimental section aims to elucidate Lion's optimization dynamics and its underlying mechanism, especially in the light of the Lyapunov function approach. We embark on a detailed empirical study, supplemented by the figures to uncover the constrained optimization mechanism Lion is inherently solving.


\subsection{Experimental Setup}
To ensure robustness and generality of our findings, experiments are conducted on multiple datasets, including CIFAR-10, CIFAR-100, and ImageNet. We evaluate Lion and its variants on a variety of model architectures such as ResNet, VGG, and Transformer-based models (ViT and GPT-2). Hyperparameters, including learning rates and weight decay coefficients, are selected based on preliminary grid-search experiments.

\subsection{Weight Decay $\Longrightarrow$ Constraint Optimization}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/wd_l1.png}
    \caption{
    Exploration of the Lion under an \( \ell_\infty \) norm constraint with a ResNet model on CIFAR-10.
    \textbf{Left}: Varying weight decay (\( \lambda \)) from 5 to 25 shows the \( \ell_\infty \) norm decreasing exponentially, converging to \( 1/\lambda \). 
    \textbf{Middle}: For different initialization levels (initial \( \ell_\infty \) norms) with \( \lambda \) set to 10, all curves converge to \( 1/\lambda \). 
    \textbf{Right}: Parameters initialized to satisfy the \( \ell_\infty \) constraint first show a decrease, then an increase in the norm, before stabilizing at \( 1/\lambda \).
    }
\label{fig:lion_norm_exploration}
\end{figure}


\paragraph{Observation} We explore the impact of weight decay (\( \lambda \)) on the \( \ell_\infty \) norm of model parameters when trained with Lion.
As shown in Figure \ref{fig:lion_norm_exploration}, varying weight decay values from 5 to 25 leads to an exponential decrease in the \( \ell_\infty \) norm, converging to \( 1/\lambda \), hinting towards the constraint optimization that Lion seems to be solving. Despite different initialization levels of the \( \ell_\infty \) norm, the convergence of all curves to \( 1/\lambda \). The right plot presents an intriguing trajectory of the \( \ell_\infty \) norm: it initially decreases, then increases, and finally stabilizes at \( 1/\lambda \). Similar trajectory in ~\ref{fig:traj-1}. In section~\ref{sec::intro}, we show that based our proof, the optimization dynamic consists of 2 phases: in the first phase,


\paragraph{Finding}
The result is consistent with our theoretical findings. It suggests that weight decay plays a crucial role in enforcing the bound constraint, driving the \( \ell_\infty \) norm of the model parameters.

\subsection{Implicit Constraint Mechanism Verification}

To ascertain Lion's capabilities further, we inspected its implicit constraint mechanism, especially its behavior under different norms. Figure \ref{fig:ImgNet_verify} showcases this on the ImageNet dataset. Remarkably, the function $\phi(x)$, characterized by $\|x\|_p$, was consistently enforced across different norms of constraints.

\subsection{Optimization Trajectory Insights}

To visualize and understand how Lion progresses in its optimization landscape, we delved into an in-depth trajectory analysis. Figure \ref{fig:traj-1} captures this essence by portraying how different weight decay settings influence the optimizer's path. A compelling observation is the symmetry of the objective function f(x) and how initial points set symmetrically evolve. The feasibility regions highlighted provide concrete evidence of Lion's prowess in maintaining bound constraints.

\section{Conclusion}
This research unpacked the theoretical basis of Lion, a recently discovered optimizer. Our Lyapunov function approach deciphered its dynamics and revealed its ability to solve a constrained optimization problem. Empirical evaluations cemented Lion's efficacy and the potential of its extensions. With these insights, we are better equipped to harness and enhance Lion's potential in future AI endeavors.



==> content/old_proof_sgd_lionk.tex <==
\subsection{Analysis with Stochastic Gradient for Lion-$\phi$}




In this section, we are going to have the convergence analysis of discrete time Lion-$\phi$. The proof idea is adapted for section~\ref{sec:discreteapp}, by defining the same Hamiltonian function, we obtain the bound for $\Delta_t^1$ and $\Delta_t^2$. 

Compared with the deterministic case, 
the main challenge 
is to bound an additional correlation term 
due to 
the stochastic gradient at each iteration $t$:  
\begin{align} \label{equ:covgm} 
%\sum_{t=0}^{T+1}  
V_t \defeq \cov(g_t, ~ \dd\phi(\tilde m_{t+1}))
= \cov(g_t, ~ \dd\phi(\beta_1 m_t + (1-\beta_1) g_t)),
\end{align} 
where $\cov(X,Y) = \E[(X-\E[X])\tt (Y-\E[Y])]$. 
As $g_t$ and $m_t$ are independent, 
we would expect that the correlation
is small if $ 1-\beta_1$ is small (i.e.,  the momentum is large). However, upper bounding \eqref{equ:covgm} becomes non-trivial when $\dd\phi$ is dis-continuous. 
For example, 
when $\dd\phi(x) = \sign(x)$, we have 
$$
V_t = \E[(g_t - \E[g_t])\tt  \sign(\beta_1 m_t + (1-\beta_1)  g_t))], ~~~~~~~~
$$
We expect that $V_t$ decays to zero as batch-size gets infinity. This is realized in the following Lemma ~\ref{lem:XY} proved 
using 
Stein's identity, while dealing with the non-smoothness of $\phi(x) = \norm{x}_1$ using the notion of weak derivative. 
% , because the chances that $ \sign(\bone m_t + (1-\beta_1)  g_t)$ is dominated by that of $g_t$ becomes small with small $1-\beta_1$. However, if 
% $m_t=0$, we have $V_t = \E[\abs{g_t-\E[g_t]}]$, which does not decay to zero with $1-\beta_1$. 

% The idea to obtain a sharp bound on $V_t$ is to observe that, in a stochastic gradient setting, the momentum $m_t$ is also stochastic, and the chance of getting $m_t$ equaling zero exactly is small. 


\begin{mydef}
For a random variable $X$ on $\RR^d$, its (trace of) variance $\var(X)$ and Fisher information $J(X)$, when exists, are defined as  
\bb 
\var(X) = \E[\norm{X - \E[X]}^2_2], && 
J(X) = \E[\norm{\dd \log \pi(X) }^2], 
\ee 
where $\pi$ denotes the density function of $X$. 
\end{mydef} 
\begin{mydef} 
The Fisher information of a random variable $X$ on $\RR^d$, if exists, is defined as
$$
J(X) = \E\left [\norm{\dd \log \pi(X)}_2^2 \right ], 
$$
where $\pi(x)$ denotes the density function of $X$. 
\end{mydef}

\begin{mydef}
For a locally integrable function $\phi\colon \RR^d \to \RR$, a function, denoted as $\dd \phi$ (with abuse of notation), is called the weak derivative of $\phi$ if 
the following holds for any compactly supported infinitely differentiable function \blue{$h(\cdot)$}: 
$$
\int \dd \phi(x) \tt h(x) \dx = 
- \int \phi(x) \tt \dd h(x)  \d x. 
$$
\end{mydef} 
For $\phi(x) = \norm{x}_1$, the sign function $\dd \phi(x) = \sign(x)$ is a weak derivative of $\phi$. 

\begin{ass}\label{ass:batch}
Assume 
\bb 
\var(g_t) \leq \frac{v_{\max}}{n_{batch}},  && 
J(g_t) \leq j_{\max} n_{batch},   ~~~\forall t\geq0.
 \ee 
 and $J(m_0) \leq j_{\max} n_{batch}$, 
 where $n_{batch}$ represents the batch size. 
\end{ass} 

\begin{ass}\label{ass::sample}
    $\mathcal{D}$ is the data distribution, the stochastic sample $\xi_t \sim \mathcal{D}$ is i.i.d., given a function $f(x;\xi)$, the gradient $\dd f(x;\xi)$ is taken with respect to variable $x$, and $\E[\dd f(x, \xi)] = \dd f(x)$
\end{ass}

\begin{thm}\label{thm:sgd}
    Under the assumptions delineated in \ref{ass::sample} and \ref{ass:batch}, consider a function $f\colon \mathbb{R}^d\to \mathbb{R}$ that is $L$-smooth. Additionally, let $\phi\colon \mathbb{R}^d\to \mathbb{R}$ be a closed and convex function, consider the following scheme: 
\bbb \label{equ:finiteupdate}
\begin{split}
m_{t+1} & = \btwo m_t  - (1-\btwo) g_t \\ 
\tilde m_{t+1} & = \bone m_{t} - (1-\bone) g_t \\ 
x_{t+1} & = x_t + \lr
(\dd \phi(\tilde m_{t+1}) - \lambda x_{t+1}), 
\end{split}
\eee
where $g_t = \dd f(x_t;\xi_t)$ as shown in ~\ref{ass::sample}, $m_0, g_1, \ldots, g_t, \ldots$ are independent random variables with $\E[g_t] = \dd f(x_t)$. 
$\dd\phi$ is a weak gradient of $\phi$ with $\dd \phi(0) = 0$, $\|\dd \phi(x) - \dd \phi(y)\|_2 \leq L_\phi \|x-y\|_2, \forall x,y \in \RR^d$, and
$\bone,\btwo \in (0,1)$, and $\btwo>\bone$, and $\epsilon, \lambda > 0$. 

Let $\phi^*$ be the conjugate function of $\phi$. 
Define the following Lyapunov function:
$$
H(x, m ) = f(x) + \frac{1}{\lambda } \phi^*(\lambda x) + \frac{\bone}{\epsilon \lambda  (1-\bone) + (1-\btwo)}(\phi^*(\lambda x) + \phi(m) - \lambda x \tt m ), 
$$
and
\bb
\Delta_t^1  & =(\dd \phi(\tm_{t+1}) - \lambda x_{t+1})
\tt 
( \tm_{t+1}  - \dd\phi^*(\lambda x_{t+1})), \\ 
\Delta^2_t & = 
 (\dd\phi(\tilde m_{t+1}) - \dd\phi(m_{t+1}))\tt  ( \tm_{t+1} - m_{t+1}), 
\ee 
where $\dd\phi^*$ is a subgradient of $\phi^*$. 
Then we have $\Delta_t^1\geq0$ and $\Delta_t^2 \geq 0$ from Lemma~\ref{lem:diff}, and 
\bb 
\E\left[H(x_{t+1}, m_{t+1}) - H(x_t, m_t)\right]
\leq 
\E\left[- \epsilon (a  \Delta_t^1 
+ b \Delta_t^2)  + \frac{L\epsilon^2}{2} \norm{\dd \phi(\tm_{t+1}) - \lambda x_{t+1}}_2^2\right] \\
+ \epsilon \frac{L_\phi}{\beta_1(1+\lambda\epsilon)}\sqrt{\frac{1+\beta_2}{1-\beta_2}} \frac{\sqrt{J_{max}}v_{max}}{\sqrt{n_{batch}}}
\ee 
where 
\bb 
a = \frac{\lr \lambda \bone }{\lr \lambda (1-\bone) + (1-\btwo) } + 1 \geq 0, &&  
b = \frac{\bone(1-\btwo)}{(\btwo-\bone)(\lr \lambda (1-\bone) + (1-\btwo)) }\geq 0. 
\ee 
$j_{\max}$, $v_{\max}$, $n_{batch}$ are defined in ~\ref{ass:batch}
%Moreover, when $\epsion < 1/L$, we have 

Hence, a telescoping sum yields 
$$
\frac{1}{T}\sum_{t=0}^{T-1} \E\left[a \Delta_t^1 + b \Delta_t^2 \right]
\leq \E\left[\frac{H(x_0,m_0) - H(x_{T}, m_T)}{\epsilon T} + \frac{L\epsilon }{2} B_t + \frac{C_t}{\sqrt{n_{\text{batch}}}}\right], 
$$
where $B_t = \frac{1}{T}\sum_{t=1}^T \norm{\dd\phi(\tm_{t+1}) - \lambda x_{t+1}}^2_2$, and 
$C_t = \frac{L_\phi}{\beta_1(1+\lambda\epsilon)}\sqrt{\frac{1+\beta_2}{1-\beta_2}} {\sqrt{J_{max}}v_{max}}$.
%{\sqrt{n_{batch}}}$
\end{thm}

\begin{proof}
    The proof is a simple extended variant of ~\ref{thm:discretemain}.
Following the proof of Theorem~\ref{thm:discreteapp}, 
define %nd  
\bb 
H(x,m) = 
(a - c) f(x)  + 
\frac{a}{\lambda }  \phi^*(\lambda x)  + 
\frac{c}{\lambda } \phi(m)  - 
c  x \tt   m, &&\text{with}&& 
c = (a+b) \bone - b  \btwo,
\ee
where 
\bb 
a = \frac{\lr \lambda \bone }{\lr \lambda (1-\bone) + (1-\btwo) } + 1 \geq 0, &&  
b = \frac{\bone(1-\btwo)}{(\btwo-\bone)(\lr \lambda (1-\bone) + (1-\btwo)) }\geq 0, && c = a - 1. 
\ee 
By the definition of $\Delta_t^1, \Delta_t^2$, we have
\bbb \label{eqn:delta}
&a \Delta_t^1 + b \Delta_t^2 \nonumber\\
&= a  (\dd \phi(\tm_{t+1}) - \lambda x_{t+1})\tt (\tm_{t+1} - \dd\phi^*(\lambda x_{t+1})) \nonumber\\
&\quad \quad \quad \quad + b  (\dd\phi(\tilde m_{t+1}) - \dd\phi(m_{t+1}))\tt  ( \tm_{t+1} - m_{t+1}) \nonumber\\
&=(\dd \phi(\tm_{t+1}) - \lambda x_{t+1})\tt 
(a ( \dd\phi^*(\lambda x_{t+1}) - \tm_{t+1})  + b  ( \tm_{t+1}-m_{t+1}) ) \nonumber \\ 
& \quad \quad \quad \quad  + b (\dd\phi(m_{t+1}) - \lambda x_{t+1})\tt (m_{t+1} - \tm_{t+1})\nonumber \\
& =-(\dd \phi(\tm_{t+1}) - \lambda x_{t+1})\tt (a  \dd\phi^*(\lambda x_{t+1})   
-((a+b) \bone -  b \btwo) m_t + (a - (a+b) \bone  + b \btwo)\dd f(x_t) ) \nonumber\\ 
& \quad \quad \quad \quad - b \frac{\beta_2 - \beta_1}{1 -\beta_2} \frac{\lambda}{c} (\frac{c}{\lambda}\dd\phi(m_{t+1}) - c x_{t+1})\tt 
(m_{t+1} - m_t) \nonumber\\
&=-\left[(a-c) g_t + a \dd \phi^*(\lambda x_{t+1}) - c m_t\right]\tt (\dd \phi(\tm_{t+1}) - \lambda x_{t+1}) \nonumber\\
    &\quad \quad \quad \quad - \frac{1}{\epsilon}\left[\frac{c}{\lambda} \dd \phi(m_{t+1}) - c x_{t+1}\right]\tt (m_{t+1} - m_t)\nonumber\\
&=-\frac{1}{\epsilon}\left[(a-c) g_t + a \dd \phi^*(\lambda x_{t+1}) - c m_t\right]\tt (x_{t+1} - x_t)\nonumber \\
    &\quad\quad \quad \quad - \frac{1}{\epsilon}\left[\frac{c}{\lambda} \dd \phi(m_{t+1}) - c x_{t+1}\right]\tt (m_{t+1} - m_t)
\eee


By Lemma~\ref{lem:diff}, 
$$
H(x_{t+1}, m_{t+1}) 
- H(x_{t}, m_t) 
\leq 
\hat \dd_x H_t \tt (x_{t+1}- x_t) 
+ \hat \dd_m H_t \tt (m_{t+1} - m_t) 
+ \frac{L}{2} \norm{x_{t+1} - x_t}_2^2,
$$
where 
%where $H(x,)$
\bb 
& \hat \dd_x H_t = (a-c) \dd f(x_t) + a  \dd\phi^*(\lambda x_{t+1}) - c m_t,  \\ 
&  \hat \dd_m H_t 
=  \frac{c}{\lambda }\dd \phi(m_{t+1}) - c x_{t+1} = \frac{c}{\epsilon\lambda} (\hat V_{x,t} 
 - \dd\phi(\tilde m_{t+1}) + \dd\phi(m_{t+1} ))
\ee 
%On the other hand, by the update rule, 
%where 
with
\bb 
& V_{x,t} =x_{t+1} - x_t    = \epsilon (\dd \phi(\tilde m_{t+1}) - \lambda x_{t+1}) \\ 
& V_{m,t}  = m_{t+1} - m_t   = - (1-\beta_2) (g_t - m_t) \\
&\tilde m_{t+1} - m_{t+1} =  - (\beta_2 - \beta_1) (g_t - m_t) = - (\beta_2 - \beta_1) V_{m,t} \\ 
& \hat V_{m,t} = 
 - \dd\phi(\tilde m_{t+1} ) + \dd\phi(m_{t+1})  \\
%= \dd\phi(\beta_1 m_t - (1-\beta_1) g_t) - \dd\phi(\beta_2 m_t - (1-\beta_2) g_t). 
\ee
This gives 
\bb 
& H(x_{t+1}, m_{t+1}) 
- H(x_{t}, m_t)  \\ 
& \leq 
\hat \dd_x H_t \tt (x_{t+1}- x_t) 
+ \hat \dd_m H_t \tt (m_{t+1} - m_t) 
+ \frac{L}{2} \norm{x_{t+1} - x_t}_2^2 \\
& 
\ee 

    
Hence,
    \bb
    H(x_{t+1}, m_{t+1}) - H(x_t, m_t) &\leq \left[(a-c) \dd f(x_t) + a \dd \phi^*(\lambda x_{t+1}) - c m_t\right]\tt (x_{t+1} - x_t) \\
    &\quad + \left[\frac{c}{\lambda} \dd \phi(m_{t+1}) - c x_{t+1}\right]\tt (m_{t+1} - m_t) + \frac{L}{2}\|x_{t+1} - x_t\|_2^2 \\
    &= \left[(a-c) g_t + a \dd \phi^*(\lambda x_{t+1}) - c m_t\right]\tt (x_{t+1} - x_t) \\
    &\quad + \left[\frac{c}{\lambda} \dd \phi(m_{t+1}) - c x_{t+1}\right]\tt (m_{t+1} - m_t) + \frac{L}{2}\|x_{t+1} - x_t\|_2^2\\
    &\quad + \epsilon (a-c)(\dd f(x_t) - g_t)\tt (\dd \phi(\tm_{t+1}) - \lambda x_{t+1}) \\
    &=- \epsilon (a  \Delta_t^1+ b \Delta_t^2) + \frac{L}{2}\|x_{t+1} - x_t\|_2^2 \ant{by equation~\ref{eqn:delta}}\\
    &\quad + \epsilon (a-c)(\dd f(x_t) - g_t)\tt (\dd \phi(\tm_{t+1}) - \lambda x_{t+1})
    \ee 
    It suffices to bound $\E \left[(\dd f(x_t) - g_t)\tt (\dd \phi(\tm_{t+1}) - \lambda x_{t+1})\right]$. 
    
    Note that 
    \bb
    &\E \left[(\dd f(x_t) - g_t)\tt (\dd \phi(\tm_{t+1}) -\lambda x_{t+1})\right] \\
    &= \E \left[(\dd f(x_t) - g_t)\tt (\frac{1}{1+\lambda\epsilon}\dd \phi(\tm_{t+1}) - \frac{\lambda}{1+\lambda \epsilon} x_{t})\right] \\
    &=\frac{1}{1+\lambda\epsilon}\E \left[(\dd f(x_t) - g_t)\tt \dd \phi(\tm_{t+1})\right] + \frac{\lambda}{1+\lambda \epsilon}\E \left[(\dd f(x_t) - g_t)\tt  x_{t}\right] 
    \ee
    By Assumption~\ref{ass::sample}, 
    \bb
    \E\left[ (\dd f(x_t) - g_t)\tt \lambda x_{t}) \right] &= \lambda\E_{x_t} \left[\E_{\xi_t}\left[ (\dd f(x_t) - \dd f(x_t, \xi_t))\tt x_t ~|~ x_{t} \right]\right]\\
    & = 0\ant{by \ref{ass::sample}~ $\E[\dd f(x, \xi)] = \dd f(x)$}
    \ee
    
    Next, let us bound $\E\left[(\dd f(x_t) - g_t)\tt \dd \phi(\tm_{t+1})\right]$. 
    \bb
    \E \left[\left(\dd f(x_t) - g_t\right)\tt \dd \phi(\tm_{t+1})\right] & =  \E \left[\left(\dd f(x_t) - g_t \right)\tt \dd \phi(\beta_1 m_{t} - (1-\beta_1) g_t)\right]\\
    & \leq  \epsilon L_{\kappa} var(g_t)\sqrt{J(\beta_1 m_t)} \ant{by \ref{lem:XY}}\\
    & \leq  \frac{1}{\beta_1} L_\phi \sqrt{\frac{1+\beta_2}{1-\beta_2}} \frac{\sqrt{J_{max}}v_{max}}{\sqrt{n_{batch}}}, \ant{by \ref{lem:XY}~\ref{lem:fisher}}
    \ee
where $J_{\max} = \max(\max_{i\leq t-1} J(g_i), J(m_0))$.
Hence,
 \bb
    &\E \left[(\dd f(x_t) - g_t)\tt (\dd \phi(\tm_{t+1}) -\lambda x_{t+1})\right] \\
    &=\frac{1}{1+\lambda\epsilon}\E \left[(\dd f(x_t) - g_t)\tt \dd \phi(\tm_{t+1})\right] + \frac{\lambda}{1+\lambda \epsilon}\E \left[(\dd f(x_t) - g_t)\tt  x_{t+1}\right] \\
    &\leq \frac{L_\phi}{\beta_1(1+\lambda\epsilon)}\sqrt{\frac{1+\beta_2}{1-\beta_2}} \frac{\sqrt{J_{max}}v_{max}}{\sqrt{n_{batch}}}
\ee





\begin{lem}\citep{dembo1991information} \label{lem:cover}
For any two independent random variables $X$ and $Y$, we have
$$
J(\sqrt{\lambda }X + \sqrt{1-\lambda} Y) \leq 
\lambda J(X) + (1-\lambda )J(Y), ~~~~~\forall \lambda \in[0,1], 
$$
$$
J(X)^{-1} + J(Y)^{-1} \leq  J(X + Y)^{-1}. 
$$
\end{lem} 


\begin{lem}\label{lem:Jineq}
Let $X, X_1,\ldots, X_n$ be independent random variables on $\RR^d$, and $a, a_1,\ldots a_n \in \RR$. We have 
\bb
& J(a_1 X_1 + \cdots +  a_n X_n)
\leq  (a_1^2+\cdots  + a_n^2)^{-1} (\sum_{i=1}^n w_i J(X_i)^{-1})^{-1},
\ee 
where $w_i = a_i^2/(a_1^2+\cdots  + a_n^2).$
\end{lem}

Because $J(X)$ is finite only when $X$ yields a differentiable density function, it prevents the singular case of $X=0$ and hence makes the bound possible. 

Roughly speaking, $J(X)^{-1}$ behaves similar to $\var(X)$, as we have 
%$J(aX)^{-1} = a^2 J(X)^{-1}$, and %the following Key lemma: 
%The following are some basic properties of Fisher information that we will use: 
%\begin{lem}\label{lem:Jineq}
 %on $\RR^d$, and $a_1,\ldots a_n \in \RR$. We have 
\bb 
J\left ( {X_1 + \cdots +  X_n} \right )^{-1}  
\leq \sum_{i=1}^n J(X_i)^{-1}, &&
J(aX)^{-1} = a^2 J(X)^{-1}, ~~\forall a\in \RR, 
\ee 
 when $X_1,\ldots, X_n$  are independent. 
 Hence, it is reasonable to make the following assumption 
 when $g_t$ is estimated with a mini-batch of size 
 $n_{batch}$.  
\begin{lem}\label{lem:fisher} 
Assume $m_{t+1} = \btwo m_t - (1-\btwo) g_t$, where  $\btwo\in(0,1)$, 
 and $m_0, g_0, \ldots g_t$ are independent random variables, with $J_{\max} = \max(\max_{i\leq t-1} J(g_i), J(m_0)),$ we have 
 $$
J(m_{t})
\leq \frac{1+\btwo}{1-\btwo}  J_{\max} . 
$$
\end{lem}

\begin{proof}
\bb
m_{t} = -(1-\btwo) (g_{t-1} + \btwo g_{t-2} + \cdots  \beta^{t-1}_2 g_0) + \btwo^{t} m_0.  
\ee 
Note that 
\bb 
(1-\btwo)^2 (1 + \btwo^{2} + \cdots + \beta_2^{2(t-1)}) + \btwo^{2t}
& = (1-\btwo)^2 \frac{1-\btwo^{2t}}{1-\btwo^2}  + \btwo^{2t} \\ 
& = \frac{(1-\btwo)(1-\btwo^{2t})}{1+\btwo} + \btwo^{2t}  \\
& \geq 
\frac{(1-\btwo)(1-\btwo^{2t})}{1+\btwo} + \frac{1-\btwo}{1+\btwo} \btwo^{2t}  \\
& = \frac{1-\btwo}{1+\btwo}. 
\ee 
Using Lemma~\ref{lem:Jineq} gives the result.
 $$
J(m_{t})
\leq \frac{1+\btwo}{1-\btwo} \max(\max_{i\leq t-1} J(g_i), J(m_0)) . 
$$
Furthermore, since $J(aX)^{-1} = a^2 J(X)^{-1}$, we have 
\bb
J(\beta_1 m_{t}) &= \frac{1}{\beta_1^2} J(m_t)\leq \frac{1+\btwo}{\beta_1^2(1-\btwo)} \max(\max_{i\leq t-1} J(g_i), J(m_0)) . 
\ee

\end{proof} 




\begin{lem}\label{lem:XY}
Let $X,Y$ be two independent $\RR^d$-valued random variables with $\var(Y)<+\infty$, $J(X)<+\infty$,  and assume $\phi$ yields a weak derivative $\dd\phi$. We have
$$\E[(Y - \E Y)\tt \dd\phi(X+\epsilon Y)] \leq \epsilon 
L_\phi \var(Y) \sqrt{J(X)}
%\E[\norm{\dd\log \pi_2(X)}_2]. 
$$
\end{lem}
\begin{proof}
For any fixed $y$, 
\bb 
\E[ (Y-\E [Y])\tt \dd\phi(X + \eps Y)~|~ Y=y] 
& = \int (y-\E [Y])\tt \dd\phi(x + \epsilon y) \pi_X(x) \d x \\ 
& = - \int \phi(x + \epsilon y) (Y-\E [Y]) \tt \dd \pi_X(x) \d x \\ 
& = - \E[ (Y-\E [Y]) \tt \dd \log \pi_X(X) \phi(X + \epsilon Y) ~|~ Y=y ].
\ee 
Then taking expectation on $Y$: 
\bb 
\E[ (Y-\E [Y])\tt \dd\phi(X + \eps Y) ] 
& = - \E [(Y-\E [Y]) \tt \dd \log \pi_X(X) \phi(X + \epsilon Y) ] \\
& = - \E [(Y-\E [Y])\tt \dd \log \pi_X(X) (\phi(X + \epsilon Y) - \phi(X+\epsilon \E[Y])) ] \\
& \leq \epsilon  L_\phi  \E [\abs{(Y-\E [Y])\tt \dd \log \pi_X(X)}\norm{(Y-\E [Y])}_2]  \\
& \leq \epsilon L_\phi \E[\norm{(Y-\E [Y])}_2^2] \E[\norm{\dd \log \pi_X(X)}_2] \\
& \leq \epsilon L_\phi \E[\norm{(Y-\E [Y])}_2^2] \sqrt{\E[\norm{\dd \log \pi_X(X)}^2_2]}  \\
& = \epsilon L_\phi \var(Y) \sqrt{J(X)}. 
\ee 
\end{proof}

==> content/rebuttal.tex <==
\newpage \clearpage 
\red{==========}
\section{Rebuttal}

\paragraph{General Response}
We sincerely appreciate all reviewers' valuable feedback and suggestions. We provide a quick summary of the additional experiments we conducted in the following and address reviewers' specific questions in individual responses.

we have added three additional experiment results on exploring different $\mathcal{K}$s and the implication of the weight decay $\lambda$, and one theoretical result that shows Lion-$\mathcal{K}$ converges under stochastic gradient.

Experiment I (the implication of weight decay). In Section \bo{add}, we add a paragraph stating that there exists an optimal weight decay $\lambda$ that results in fast convergence with no sacrifice of training loss. The best $\lambda$ corresponds to the largest $\lambda$ such that the constraint formed by $\lambda$ contains the optimal solution. In Figure 4, we plot the performance of applying Lion with different weight decay $\lambda$ and confirms that 1) larger $\lambda$ in general speeds up the learning, and 2) with $\lambda < \lambda_0$ for some critical $\lambda_0$, the final performance stays unchanged. When $\lambda$ goes beyond $\lambda_0$, the performance starts to drop. This implies tuning the best weight decay for Lion is crucial.

Experiment II (the toy example with different $\mathcal{K}$ shown in Table 2): In Section \bo{add} Figure~\ref{fig:different_k}, we plot the behavior of Lion with different $\mathcal{K}$ on the same toy example used in Figure~\ref{fig:traj-1}, to demonstrate that the observed behavior closely matches what the theory predicts.

Experiment III (comparison of Lion-$\ell_p$ on ImageNet and Language Modeling): In Section 5 Figure~\ref{fig:imagenet}, we show the performance of applying Lion-$\ell_p$ with $p \in \{1.0, 1.2, 1.4, 1.6, 1.8, 2.0\}$ on ImageNet and Language Modeling using ResNet-50, ViT-16B, and GPT-2. Interestingly, results demonstrate that Lion-$\ell_p$ with smaller $p$ works well when ViT and GPT-2 are used (on ImageNet and Language Modeling correspondingly). However, when ResNet-50 is used on ImageNet, the trend is reversed and Lion-$\ell_2$ performs the best. This indicates that the choice of $\mathcal{K}$ might be architecture-dependent. We leave this as an interesting future research direction.



\paragraph{R1}  
Dear reviewer, thanks a lot for your comments. We will fix the typos and further the draft. 

1) %The analysis for 
The extension to the stochastic gradient case 
is straightforward given our results with the full gradient. We provide a new theorem in the Appendix (Check Theorem~\ref{thm:sgd}).

2) One convergence rate result implied from our framework is that $\Delta_1$ and $\Delta_2$ converge with an $O(1/t)$ rate. 
This is consistent with 
the results of classical algorithms on non-convex functions that the gradient (and momentum) norm converges to $O(1/t).$

It is also straightforward to obtain stronger convergence rates by placing stronger assumptions on $f$ (e.g., convexity or strong convexity), but since $f$ is non-convex in deep learning, we defer such derivations to future works. 

3)
We will add comments on Theorem 4. 
The main implication is that we get parallel results on the two-phase convergence for the discrete-time case. 
The main difference is that  
the rolling average of $\Delta^1_t$ and $\Delta^2_t$ converges with $O(1/(\epsilon  t) + \epsilon)$, where epsilon is step size, rather than $O(1/t)$ in the continuous case. 

The implicit form 
fits nicer with our proof as we tried to 
get a Lyapunov form in the discrete-time. 
We think it is mainly for technical reasons of the proof and as we explain in Section 4, the implicit form is equivalent to the explicit form with a different step size. 

\paragraph{R2} 
We thank the reviewer for your helpful comments. 

1) 
\red{Empirical comparison with other algorithms}


2) From Theorem 3.1, we have that (the rolling average of) $\Delta(x_t, m_t)$ converges with a $O(1/t)$. This is parallel to the standard results for classical gradient descent in which the gradient norm converges with $O(1/t)$. Different choices of $\mathcal K$ change the function $\Delta(x,m)$ (e.g., $\ell_1$ vs. $\ell_2$ norm), and hence are not completely comparable. 

Meanwhile, the authors think that the current standard (worst-case) convergence rate is too rough and assumption-dependent to explain the practical power of optimization algorithms such as AdamW in deep learning. 
It is likely the better algorithms may only have a better constant, rather than a better convergence rate. 
Hence, we do not attempt to make arguments on converge rate. 

We think that having a Lyapunov function posits a necessary condition for an update rule to be a valid optimizer.
It is then up to empirical results and insights to determine whether the algorithm performs well on the different problems of interest. 
%(or some further unknown insights) 


\paragraph{R3}
We thank the reviewer for the valuable comments. 

1) \red{\emph{Interpretation of empirical results}}

2) \red{\emph{Ablation of key components of Lion to justify theory}}

3) \red{\emph{Empirical validation of algorithms in Table 2}}

4) \red{\emph{Not connecting findings with the success of Lion. How does constraint help}} 

\paragraph{R4} 
Dear Reviewer, we thank you for your valuable comments. Below are answers to your question on the differentiability of $\mathcal K$. 

1) 
The main difference 
between the continuous and discrete time results 
is that the $\Delta(x,m)$,
which is a measure of stationarity of the problem 
decreases with $O(1/t)$ rate in the continuous time, 
while $O(1/(\epsilon T) + \epsilon)$ in the discrete time, where $T$ denotes the number of steps. 
%
Hence,   
the continuous-time and discrete-time 
results are  parallel and consistent, in the sense that 
we recover the continuous-time result when taking the step size $\epsilon$ to zero (with $t = \epsilon T$). 

3) 
If we assume $\mathcal K$ is smooth (with bounded Hessian), it is possible to improve the discrete-time rate to $O(1/(\epsilon T))$. Hence,   
the impact of the non-differentiability is the $O(\epsilon)$ term, 
which suggests that the algorithm converges up to a $\epsilon$ accuracy. 
This is a typical phenomenon in optimization with non-smooth objectives (like sub-gradient descent) 
or non-smooth update (like signed GD). 
Because in practice the step size is small or decaying, this may not have a big impact on practical performance. 

 4) The requirement 
 for differentiability in our statement of continuous-time results 
 is mainly for the simplicity of the presentation. 
 We can state a continuous-time result for non-smooth $\kappa$ using non-smooth versions of Lyapunov theory, 
 but we would need to recall sophistic technical tools such as Filippov's differential inclusion and Clarke's generalized gradient. See e.g., 
 \emph{Daniel Shevitz and Brad Padent,  Lyapunov Stability Theory of Nonsmooth Systems, 1993.}

5) The mirror descent with $\ell_1$ norm reduces to Signed GD: $x_{t+1} = x_t - \epsilon \sign(\nabla  f(x_t))$, which is different from $x_{t+1} = \sign(x_t - \nabla f(x_t))$. 
Hence it is the update (not the value of $x_t$) that is constrained in $[-1,1]$. With standard arguement, one can show that $\min_{s\leq T}||\nabla f(x_s)||_1 =O(1/(\epsilon T) + \epsilon)$, which is consistent with our result. 
%,%it does not have the problem o


%One thing that the authors believe is 

%and efforts. 


==> content/trash.tex <==


\newpage \clearpage 
\red{====== }
Set $b =1$, 
and \textbf{}
$$
\lr b (\btwo - \bone) \lambda = (1-\btwo) (a+b) \bone - b (1-\btwo) \btwo 
$$
\bb 
a  & = \frac{ (1-\btwo) \btwo +  (\btwo - \bone )\lr \lambda }{(1-\btwo) \bone} -  1  \\
& = \frac{(\btwo - \bone) (1-\btwo + \lr \lambda ) }{(1-\btwo )\bone} 
\ee 

\bb 
(a+1)\bone  - \btwo 
& =   \bone \frac{ (1-\btwo) \btwo +   (\btwo - \bone )\lr \lambda }{(1-\btwo) \bone}  - 
\btwo  \\ 
& =   \frac{ (1-\btwo) \btwo +   (\btwo - \bone )\lr \lambda }{(1-\btwo)}  - 
\btwo  \\ 
& = \frac{(\btwo - \bone)\epsilon \lambda }{1-\btwo}
\ee 

\bb 
(a+1)\bar \bone - \bar \btwo
& = (a+1)(1- \bone) - (1- \btwo) \\ 
& = a - (a+1) \bone + \btwo \\ 
& = a  - \frac{(\btwo - \bone)\epsilon \lambda }{1-\btwo}  \\
& = \frac{(\btwo - \bone) (1-\btwo + \lr \lambda ) }{(1-\btwo )\bone} -  \frac{(\btwo - \bone)\epsilon \lambda }{1-\btwo}  \\
& = \frac{(\btwo - \bone) (1-\btwo + (1-\bone)\lr \lambda   ) }{(1-\btwo )\bone} 
\ee 


\bb 
H = \frac{a}{\lambda }  \phi^*(\lambda x)  + 
(- (a+1) \bone+ \btwo) x \tt   m
- \frac{(- (a+1) \bone+ 1 \btwo)}{\lambda } \phi(m)
+ ((a+1) \bar\bone - \bar \btwo) f(x) 
) 
\ee 

\bb 
H = 
%+ %((a+1) \bar\bone -  \bar \btwo)
 \frac{(1-\btwo + (1-\bone)\lr \lambda   ) }{\bone} 
f(x)   
+ \frac{ (1-\btwo + (1-\bone)\lr \lambda )  }{\bone \lambda } 
 \phi^*(\lambda x)  + 
%(- (a+1) \bone+  \btwo) 
%- \frac{\lr \lambda }{1}
%+ %\frac{(- (a+1) \bone+  \btwo)}
%\frac{\epsilon  }{1}\frac{1}{1 } 
\lr ( \phi^*(\lambda x) + 
\phi(m)
-  \lambda 
x \tt   m). 
\ee 
Or 
\bb 
H = 
f(x) + \frac{1}{\lambda } \phi^*(\lambda x)  + 
%(- (a+1) \bone+  \btwo) 
%- \frac{\lr \lambda }{1}
%+ %\frac{(- (a+1) \bone+  \btwo)}
%\frac{\epsilon  }{1}\frac{1}{1 } 
 \lr 
 %+ %((a+1) \bar\bone -  \bar \btwo)
 \frac{\bone}{(1-\btwo + (1-\bone)\lr \lambda   ) }%{\bone} 
%f(x)   
%+ \frac{ (1-\btwo + (1-\bone)\lr \lambda )  }{\bone \lambda } 
 ( \phi^*(\lambda x) + 
\phi(m)
-  \lambda 
x \tt   m). 
\ee 

$1-\btwo = \lr \gamma$, $1-\bone = \varepsilon \lr \gamma$, then 
$$
\frac{1-\varepsilon \lr \gamma}{
 \gamma + \varepsilon \lr \lambda  \gamma }
$$


Hence, 
\bb 
(\dd \phi(\tm_{t+1}) - \lambda x_{t+1})\tt 
(a ( \dd\phi^*(\lambda x_{t+1}) - \tm_{t+1})  + b  (m_{t+1} - \tm_{t+1}) ) 
+ 
b (\dd\phi(m_{t+1}) - \lambda x_{t+1})\tt (-m_{t+1} + \tm_{t+1})
\leq 0.
\ee 

\bb 
(\dd \phi(\tm_{t+1}) - \lambda x_{t+1})\tt 
(a  \dd\phi^*(\lambda x_{t+1}) 
- (a+b) \tm_{t+1}  + b  m_{t+1}) 
+ 
b (\dd\phi(m_{t+1}) - \lambda x_{t+1})\tt (-m_{t+1} + \tm_{t+1}) 
\leq 0 
\ee 
Let 
$\tilde m_{t+1} 
=  \frac{1}{a+b} 
(b m_{t+1} + cm_t - \alpha \dd f(x_t))$, 
then 
%$$\tm_{t+1} - m_{t+1}= \frac{1}{a+b} ( - am_{t+1} + cm_t  - \alpha \dd f(x_t)). $$
\bb 
(\dd \phi(\tm_{t+1}) - \lambda x_{t+1})\tt 
(a  \dd\phi^*(\lambda x_{t+1}) 
- cm_t + \alpha \dd f(x_t) 
) 
+ 
b (\dd\phi(m_{t+1}) - \lambda x_{t+1})\tt (-m_{t+1} + \tm_{t+1})
\leq 0
\ee 

Define 
$$
H(x,m) 
= \alpha f(x) + 
\frac{a}{\lambda } \phi^*(\lambda x) 
+ \frac{c}{\lambda} \phi(m) 
- c x \tt m. 
$$
Then the equation is written as 
$$
(\hat \dd_x H_t ) 
\tt (\dd \phi(\tm_{t+1}) - \lambda x_{t+1}) 
+ (\hat \dd_m H_t)
\tt 
\frac{\lambda b}{c}(\tilde m_{t+1}-m_{t+1}) \leq \frac{\epsilon L}{2} \norm{\dd \phi(\tilde m_{t+1}) - \lambda x_{t+1}}_2^2 + (H_{t} - H_{t+1})/\epsilon. 
$$
Hence, we can set the update to be 
\bb 
x_{t+1} & = x_t + \lr (\dd \phi(\tm_{t+1}) - \lambda x_{t+1}) \\
m_{t+1}  & =  m_t +  \frac{\lr \lambda b }{c} (\tm_{t+1} - m_{t+1}) \\
\tm_{t+1} & = \frac{1}{a+b}
( b m_{t+1} + c m_t - \alpha \dd f(x_t)) 
\ee 
Or 
\bb 
m_{t+1}  
& =  m_t +  \frac{\lr \lambda b }{c} (\tm_{t+1} - m_{t+1})  \\
& = m_t +  \frac{\lr \lambda b }{c} 
\frac{1}{a+b} (-a m_{t+1} + c m_t - \alpha \dd f(x_t)) 
\ee 

\bb 
(a+b) c m_{t+1}   
%& =  m_t +  \frac{\lr \lambda b }{c} (\tm_{t+1} - m_{t+1})  \\
& = (a+b) c m_t +  {\lr \lambda b } 
 (-a m_{t+1} + c m_t - \alpha \dd f(x_t)) 
\ee 


\bb 
m_{t+1}   
%& =  m_t +  \frac{\lr \lambda b }{c} (\tm_{t+1} - m_{t+1})  \\
& =  
\frac{((a+b) c  +  {\lr \lambda b } c)}{((a+b) c + \epsilon \lambda b a) } m_t - 
 \frac{{\lr \lambda b } \alpha}{((a+b) c + \epsilon \lambda b a) } \dd f(x_t) 
\ee 
We want to set 
\bb 
& \frac{((a+b) c  +  {\lr \lambda b } c)}{((a+b) c + \epsilon \lambda b a) }  = \btwo  \\ 
& c + \alpha = a \\
 & \frac{1-\btwo}{\btwo - \bone}  = \frac{\epsilon \lambda b}{c} 
\ee  
Take $a+b = 1$, 
\bb 
& \frac{(c  +  {\lr \lambda b } c)}{( c + \epsilon \lambda b (1-b)) }  = \btwo  \\ 
& c + \alpha = (1-b) \\
 &r^{-1} =  \frac{1-\btwo}{\btwo - \bone}  = \frac{\epsilon \lambda b}{c} 
\ee 

$$
 \frac{( \epsilon \lambda b r (1  +  {\lr \lambda b }))}{( \epsilon \lambda b r + \epsilon \lambda b (1-b)) }  = 
  \frac{(  r (1  +  {\lr \lambda b }))}{(  r +  (1-b)) }  
 = \btwo  
$$
$$
r\btwo + (1-b)\btwo = r + \epsilon \lambda r b 
$$
\bb 
b & = \frac{r \btwo - \btwo - r}{\epsilon\lambda r + \btwo} \\ 
& = \frac{\frac{\btwo-\bone}{1-\btwo}(\btwo - 1) - \btwo }{ \epsilon \lambda \frac{\btwo-\bone}{1-\btwo} + \btwo }  \\
& = \frac{(\bone - 2 \btwo)(1-\btwo)}{\epsilon \lambda (\btwo-\bone) + \btwo - \btwo^2}
\ee 
But this $b <0$?  Not correct?  


\begin{lem}
If $m_{t+1} = \btwo m_t - (1-\btwo) g_t$ and $\tilde m_{t+1} = \bone m_t - (1-\bone) g_t$. Then $\tilde m_{t+1} = $
\end{lem}
\begin{proof}
\bb 
\tilde m_{t+1} = \frac{\bone}{\btwo} m_{t+1} - (1- \frac{\bone}{\btwo}) g_t
\ee  
\bb 
\tilde m_{t+1} - m_{t+1}
= 
%- (1-\frac{\bone}{\btwo}) 
-(\btwo-\bone)(m_{t} + g_t)
\ee 
\bb 
m_{t+1} - m_t = (1-\btwo) (m_{t} + g_t). 
\ee 
\bb 
m_{t+1} - m_t 
= \frac{1-\btwo}{\btwo - \bone} (\tm_{t+1} - m_{t+1})
\ee
\end{proof}

%But we know $m_{t+1} = \btwo m_t - (1-\btwo) \dd f(x_t)$

\red{======}
\bb 
(\dd \phi(\tm_{t+1}) - \lambda x_{t+1})\tt 
(a ( \dd\phi^*(\lambda x_{t+1}) - \tm_{t+1})  + b  (m_{t+1} - \tm_{t+1}) ) 
+ 
b (\dd\phi(m_{t+1}) - \lambda x_{t+1})\tt (-m_{t+1} + \tm_{t+1})
\leq 0.
\ee 

\bb 
(\dd \phi(\tm_{t+1}) - \lambda x_{t+1})\tt 
(a  \dd\phi^*(\lambda x_{t+1}) 
- (a+b) \tm_{t+1}  + b  m_{t+1}) 
+ 
b (\dd\phi(m_{t+1}) - \lambda x_{t+1})\tt (-m_{t+1} + \tm_{t+1}) 
\leq 0 
\ee 

\bb 
\tm_{t+1} = \bone m_t  - (1-\bone) g_t \\
m_{t+1} = \btwo m_t - (1-\btwo) g_t. 
\ee 
\bb 
& (\dd \phi(\tm_{t+1}) -          \lambda x_{t+1})\tt 
(a  \dd\phi^*(\lambda x_{t+1})  + 
(- (a+b) \bone+ b \btwo) m_t 
+ ((a+b) \bar\bone - b \bar \btwo)\dd f(x_t) 
) \\ 
& - 
b (\btwo - \bone)  (\dd\phi(m_{t+1}) - \lambda x_{t+1})\tt 
(m_t + \dd f(x_t))
%(-m_{t+1} + \tm_{t+1}) 
\leq 0 
\ee 
Define 
\bb 
H = \frac{a}{\lambda }  \phi^*(\lambda x)  + 
(- (a+b) \bone+ b \btwo) x \tt   m
- \frac{(- (a+b) \bone+ b \btwo)}{\lambda } \phi(m)
+ ((a+b) \bar\bone - b \bar \btwo) f(x) 
) 
\ee 
\bb 
\hat \dd_x H_t \tt V_x +  
\hat \dd_m H_t \tt \frac{b(\btwo - \bone)\lambda }{(a+b)\bone - b \btwo} (- m_t - \dd f(x_t)). 
\ee 

\bb 
\hat \dd_x H_t \tt  (x_{t+1} - x_t)/\lr  +  
\hat \dd_m H_t \tt \frac{b(\btwo - \bone)\lambda }{-(a+b)\bone + b \btwo} (m_{t+1} - m_t)/(1-\btwo). 
\ee 

We want 
$$
 \frac{b(\btwo - \bone)\lambda }{(a+b)\bone - b \btwo} = \frac{1-\btwo}{\epsilon}. 
$$
Set $b =1$, 
and 
$$
\lr b (\btwo - \bone) \lambda = (1-\btwo) (a+b) \bone - b (1-\btwo) \btwo 
$$
\bb 
a  & = \frac{ (1-\btwo) \btwo +  (\btwo - \bone )\lr \lambda }{(1-\btwo) \bone} -  1  \\
& = \frac{(\btwo - \bone) (1-\btwo + \lr \lambda ) }{(1-\btwo )\bone} 
\ee 

\bb 
(a+1)\bone  - \btwo 
& =   \bone \frac{ (1-\btwo) \btwo +   (\btwo - \bone )\lr \lambda }{(1-\btwo) \bone}  - 
\btwo  \\ 
& =   \frac{ (1-\btwo) \btwo +   (\btwo - \bone )\lr \lambda }{(1-\btwo)}  - 
\btwo  \\ 
& = \frac{(\btwo - \bone)\epsilon \lambda }{1-\btwo}
\ee 

\bb 
(a+1)\bar \bone - \bar \btwo
& = (a+1)(1- \bone) - (1- \btwo) \\ 
& = a - (a+1) \bone + \btwo \\ 
& = a  - \frac{(\btwo - \bone)\epsilon \lambda }{1-\btwo}  \\
& = \frac{(\btwo - \bone) (1-\btwo + \lr \lambda ) }{(1-\btwo )\bone} -  \frac{(\btwo - \bone)\epsilon \lambda }{1-\btwo}  \\
& = \frac{(\btwo - \bone) (1-\btwo + (1-\bone)\lr \lambda   ) }{(1-\btwo )\bone} 
\ee 


\bb 
H = \frac{a}{\lambda }  \phi^*(\lambda x)  + 
(- (a+1) \bone+ \btwo) x \tt   m
- \frac{(- (a+1) \bone+ 1 \btwo)}{\lambda } \phi(m)
+ ((a+1) \bar\bone - \bar \btwo) f(x) 
) 
\ee 

\bb 
H = 
%+ %((a+1) \bar\bone -  \bar \btwo)
 \frac{(1-\btwo + (1-\bone)\lr \lambda   ) }{\bone} 
f(x)   
+ \frac{ (1-\btwo + (1-\bone)\lr \lambda )  }{\bone \lambda } 
 \phi^*(\lambda x)  + 
%(- (a+1) \bone+  \btwo) 
%- \frac{\lr \lambda }{1}
%+ %\frac{(- (a+1) \bone+  \btwo)}
%\frac{\epsilon  }{1}\frac{1}{1 } 
\lr ( \phi^*(\lambda x) + 
\phi(m)
-  \lambda 
x \tt   m). 
\ee 
Or 
\bb 
H = 
f(x) + \frac{1}{\lambda } \phi^*(\lambda x)  + 
%(- (a+1) \bone+  \btwo) 
%- \frac{\lr \lambda }{1}
%+ %\frac{(- (a+1) \bone+  \btwo)}
%\frac{\epsilon  }{1}\frac{1}{1 } 
 \lr 
 %+ %((a+1) \bar\bone -  \bar \btwo)
 \frac{\bone}{(1-\btwo + (1-\bone)\lr \lambda   ) }%{\bone} 
%f(x)   
%+ \frac{ (1-\btwo + (1-\bone)\lr \lambda )  }{\bone \lambda } 
 ( \phi^*(\lambda x) + 
\phi(m)
-  \lambda 
x \tt   m). 
\ee 

$1-\btwo = \lr \gamma$, $1-\bone = \varepsilon \lr \gamma$, then 
$$
\frac{1-\varepsilon \lr \gamma}{
 \gamma + \varepsilon \lr \lambda  \gamma }
$$

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
%\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}x
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old_content/abstract.tex <==
\begin{abstract}
This paper studies \lion{}, a simple yet effective optimizer found by program search. \lion{} achieves comparable or superior performance against state-of-the-art adaptive gradient methods like \adamw{}, but can learn faster and only require storing the first-order momentum. Despite its effectiveness, why \lion{} works well remains a mystery.
Our study serves as an initial effort to decode the critical factors contributing to the success of \lion{} from two perspectives. Firstly, we examine \lion{}'s unique functionality that employs a sign operation for effective regularization and an innovative momentum tracking technique, leading to good generalization in deep learning tasks. Secondly, we carry out an analysis of \lion{} from the perspective of Hamiltonian mechanics.
Based on the insights drawn from our study, we propose a novel optimization algorithm that integrates essential components of \lion{}, while maintaining a stronger theoretical underpinning.

\end{abstract}

==> old_content/draft_sgd.tex <==

\subsection{\red{Try Weaker Smoothness on $f$ with stochastic gradient}}

\newcommand{\batch}{n_{\text{batch}}}
\begin{ass} 
Consider the stochastic Lion-$\phi$:
\bb 
m_{t+1} = \beta_2 m_t + (1-\beta_2) g_t \\ 
x_{t+1} = x_t - \epsilon \dd\phi(m_{t} + \beta g_t),
\ee 
where $m_0, g_1, \ldots, g_t, \ldots$ are independent random variables with $\E[g_t] = \dd f(x_t)$.   
Assume  $\beta = (1-\beta_1)/\beta_1$, and $\beta_1,\beta_2 \in (0,1)$, and $\epsilon >0$. 
\end{ass} 


%\paragraph{Remark} 
Compared with the deterministic case, 
the main challenge 
is to bound an additional correlation term 
due to 
the stochastic gradient at each iteration $t$:  
\begin{align} \label{equ:covgm} 
%\sum_{t=0}^{T+1}  
V_t \defeq \cov(g_t, ~ \dd\phi(\tilde m_{t+1})) 
= \cov(g_t, ~ \dd\phi(\beta_2 m_t + \varepsilon g_t)),  && \varepsilon = (1-\beta_2 + \beta), 
\end{align} 
where $\cov(X,Y) = \E[(X-\E[X])\tt (Y-\E[Y])]$. 
As $g_t$ and $m_t$ are independent, 
we would expect that the correlation 
is small if $\varepsilon = 1-\beta_2 + \beta$ is small (i.e.,  the momentum is large). However, upper bounding \eqref{equ:covgm} becomes non-trivial when $\dd\phi$ is dis-continuous. 
For example, 
when $\dd\phi(x) = \sign(x)$, we have 
$$
V_t = \E[(g_t - \E[g_t])\tt  \sign(\beta_2 m_t + \varepsilon  g_t))], ~~~~~~~~
$$
If $m_t \neq 0$, we expect that $V_t$ decays to zero with $\varepsilon$, because the chances that $ \sign(\beta_2 m_t + \varepsilon  g_t)$ is dominated by that of $g_t$ becomes small with small $\varepsilon$. However, if 
$m_t=0$, we have $V_t = \E[\abs{g_t-\E[g_t]}]$, which does not decay to zero with $\varepsilon$. 

The idea to obtain a sharp bound on $V_t$ is to observe that, in a stochastic gradient setting, the momentum $m_t$ is also stochastic, and the chance of getting $m_t$ equaling zero exactly is small.  This is realized in the following Lemma proved 
using 
Stein's identity, while dealing with the non-smoothness of $\phi(x) = \norm{x}_1$ using the notion of weak derivative. 


\begin{mydef}
For a locally integrable function $\phi\colon \RR^d \to \RR$, a function, denoted as $\dd \phi$ (with abuse of notation), is called the weak derivative of $\phi$ if 
the following holds for any compactly supported infinitely differentiable function \blue{$h(\cdot)$}: 
$$
\int \dd \phi(x) \tt h(x) \dx = 
- \int \phi(x) \tt \dd h(x)  \d x. 
$$
\end{mydef} 
For $\phi(x) = \norm{x}_1$, the sign function $\dd \phi(x) = \sign(x)$ is a weak derivative of $\phi$. 

\begin{mydef} 
For a random variable $X$ on $\RR^d$, its (trace of) variance $\var(X)$ and Fisher information $J(X)$, when exists, are defined as  
\bb 
\var(X) = \E[\norm{X - \E[X]}^2_2], && 
J(X) = \E[\norm{\dd \log \pi(X) }^2], 
\ee 
where $\pi$ denotes the density function of $X$. 
\end{mydef} 

\begin{lem}\label{lem:XY}
Let $X,Y$ be two independent  random variables on $\RR^d$ with $\E[Y]=0$, $\var(Y)<+\infty$, $J(X)<+\infty$,  and assume $\phi$ yields a weak derivative $\dd\phi$. Assume $\phi$ is $L_\phi$-Lipschitz, and $\epsilon \geq 0$. 
We have
$$\E[Y\tt \dd\phi(X+\epsilon Y)] \leq \epsilon 
L_\phi \var(Y) \sqrt{J(X)}. 
%\E[\norm{\dd\log \pi_2(X)}_2]. 
$$
\end{lem}
Because $J(X)$ is finite only when $X$ yields a differentiable density function, it prevents the singular case of $X=0$ and hence makes the bound possible. 

Roughly speaking, $J(X)^{-1}$ behaves similar to $\var(X)$, as we have 
%$J(aX)^{-1} = a^2 J(X)^{-1}$, and %the following Key lemma: 
%The following are some basic properties of Fisher information that we will use: 
%\begin{lem}\label{lem:Jineq}
 %on $\RR^d$, and $a_1,\ldots a_n \in \RR$. We have 
\bb 
J\left ( {X_1 + \cdots +  X_n} \right )^{-1}  
\leq \sum_{i=1}^n J(X_i)^{-1}, &&
J(aX)^{-1} = a^2 J(X)^{-1}, ~~\forall a\in \RR, 
\ee 
 when $X_1,\ldots, X_n$  are independent. 
 Hence, it is reasonable to make the following assumption 
 when $g_t$ is estimated with a mini-batch of size 
 $\batch$.  
\begin{ass} 
Assume 
\bb 
\var(g_t) \leq \frac{v_{\max}}{\batch},  && 
J(g_t) \leq j_{\max} \batch,   ~~~\forall t\geq0.
 \ee 
 and $J(m_0) \leq j_{\max} \batch$, 
 where $\batch$ represents the batch size. 
\end{ass} 


\begin{mydef}
$\phi\colon \RR^d\to \RR$ is said to be $q$-homogeneous for $q\in\RR$ if 
\bb 
\phi(a x) = \abs{a}^q \phi(x) 
~~~~~\text{for any $x\in\RR^d$, $a \in \RR$}. 
\ee 
\end{mydef}
The canonical example is when $\phi(x) = \norm{x}^q$ for some norm $\norm{\cdot}$. 
% is  norm function. \red{See Section \red{XXX} for examples.}
 
\begin{mydef}[Weak Smoothness] 
We say that  $f\colon\RR^d\to\RR$ is $\phi$-weak smooth if there exists $L_0,L_1<+\infty$ and $L_3 > 0$, such that when $\norm{x - y}_2\leq L_3$, 
$$
f(y) - f(x) 
\leq   \dd f(x)\tt (y-x)  +
\frac{1}{2} (L_0 + L_1 \phi(\dd f(x))) \norm{y-x}^2_2. 
%~~~~\forall x,y\in\RR^d.
$$
%for some $L_0,L_1 <+\infty$. 
\end{mydef} 

\begin{thm}\label{thm:weaksmooth}
Assume $f$ is $\phi$-weak smooth  as above  
and lower bounded ($\inf_x f(x) >-\infty$), and $\phi$ is convex and $q$-homogeneous for $q\in\RR$. 
Let  $\dd \phi$ be both a subgradient  and a weak derivative 
of $\phi$ with $\dd \phi(0) = 0$. 
 Assume $\phi$ is $L_\phi$-Lipschitz.  
Assume $\sup_t \norm{\dd\phi(m_t)}_2\defeq D < +\infty$. 
We have when $\epsilon \leq \min\left (\frac{L_3}{D}, \frac{1}{L_1 D} \left (\frac{1+\beta_2}{1-\beta_2}\right)^{q} \right )$,
$$
\frac{1}{T+1}\sum_{t=0}^T  \E[ D_{\phi_{m_t},\beta}(g_t, 0) ]
+  \E[ D_\phi(m_{t+1},0)  ] 
%= O\left (
\leq 
\frac{A}{\epsilon T} + B \epsilon + 
\frac{1-\beta_1\beta_2}{\sqrt{1-\beta_2} \sqrt{\batch}} C, 
%\frac{(H_0 - H_{T+1}) + \frac{L d \epsilon^2}{2} }{\epsilon T}. 
$$ 
where $A = f(x_0) - \inf_{x} f(x)$  and $B = L_0 D^2/2$,
and $C = \frac{\sqrt{1+\beta_2}}{\beta_1\beta_2}
v_{\max} \sqrt{j_{\max}} L_\phi$. 
\end{thm}


\begin{proof}
Assume $\E[g_t] = \dd f(x_t)$. 
Let $\tm_t = m_t + \beta g_t$. 
Let $D^2 = \sup_m \norm{\dd\phi(m)}_2^2$. 
By the $\phi$-weak smoothness of $f$,  when $\norm{x_{t+1} - x_t}_2 = \epsilon \norm{\dd\phi(\tilde m_{t+1})}_2 \leq \epsilon D  \leq L_3$, or $\epsilon \leq L_3/D$, 
we have 
\bb 
f(x_{t+1}) - f(x_t) 
\leq  - \lr  \dd f(x_t)\tt  \dd\phi(\tilde m_{t+1})  +
\frac{1}{2} \epsilon^2 (\bar L_0 + \bar L_1 \phi(\dd f(x_t))), 
%+   B_f(x_t -\lr \dd\phi(\tm_{t+1}), x_t) 
%\frac{\lr^2}{2} 
% \dd\phi(\tilde m_{t+1})  \tt \dd^2f(x_t) 
 % \dd\phi(\tilde m_{t+1}) 
%  + O(\lr^3 \norm{ \dd\phi(\tilde m_{t+1})}^3). 
\ee 
where $\bar L_0 = L_0 D^2$ and $\bar L_1 = L_1 D^2$. 
By the convexity of $\phi$: 
\bb 
\phi(m_{t+1}) - \phi(m_t) 
& \leq \lambda  \dd\phi(m_{t+1}) \tt ( g_t  - m_{t+1}) \\ 
& = \lambda \dd\phi(m_{t+1}) \tt  g_t  
- \lambda  D_\phi(m_{t+1},0)
%\dd\phi(m_{t+1}) \tt m_{t+1}. 
\ee 
Let 
$H_t =  f(x_t) + \frac{\epsilon}{\lambda} \phi(m_t)$. We have 
\bb 
H_{t+1} - H_t 
\leq - 
\lr D_{\phi_{m_t, \beta}}(g_t, 0) 
- \lr D_\phi(m_{t+1},0) 
+ \lr V_t 
+  \frac{\bar L_0}{2} \epsilon^2 +
\frac{\bar L_1}{2}  \epsilon^2 \phi(\dd f(x_t)),
\ee 
where $ V_t = (g_t - \dd f(x_t))\tt\dd\phi(\tilde m_{t+1})$ and it is the term that stems from the stochastic gradient. 

Summing over $t$ and using Lemma~\ref{lem:m2df}:
$$
\frac{1}{T+1}\sum_{t=0}^T \frac{1}{\beta} D_{\phi_{m_t,\beta}}(g_t, 0) 
+ (1 - \frac{\bar L_1}{2} \epsilon \left (\frac{1+\beta_2}{1-\beta_2}\right)^q ) D_\phi(m_{t+1},0) 
\leq 
\frac{(H_0 - H_{T+1}) + \frac{T \bar L_0 \epsilon^2}{2} }{\epsilon (T+1)} + 
\bar V, 
%+ \frac{L_1 d \epsilon^2}{2} }{\epsilon T} 
$$ 
where $\bar V = \sum_{t=0}^T V_t/(T+1)$. 
%Choosing
Choosing $\epsilon \leq \frac{1}{\bar L_1} \left (\frac{1-\beta_2}{1+\beta_2}\right)^q$. We get  
$$
\E 
\left [ \frac{1}{T+1}\sum_{t=0}^T \frac{1}{\beta}D_{\phi_{m_t,\beta}}(g_t, 0) 
+\frac{1}{2} D_\phi(m_{t+1},0)  \right ]  
\leq 
\frac{\E \left [(H_0 - H_{T+1}) \right]}{\epsilon (T+1)}  + 
\frac{\bar L_0  \epsilon}{2} +\E [\bar V], 
$$ 
where
$$
\E[\bar V] = \frac{1}{T+1} 
\sum_{t=0}^T \cov(g_t, \dd \phi(\tilde m_{t+1})),
$$
where $\cov(g_t, \dd\phi(\tilde m_{t+1})) 
= \E[(g_t - \dd f(x_t)) \dd\phi(\tilde m_{t+1})]$. 
Note that 
$$
\tm_{t+1} = \beta_2 m_t + (1-\beta_2 + \beta) g_t. 
$$
We expect that the correlation term decreases with $(1-\beta_2)$ and $\beta$, as in this case the contribution of $g_t$ inside $\tilde m_{t+1}$ decreases. 
Using
Lemma~\ref{lem:XY} and 
Lemma~\ref{lem:fisher}, we have 
$$
\E[V_t] 
\leq (1-\beta_2 + \beta) L_\phi \var(g_t) \sqrt{J(\beta_2 m_t)}  
\leq 
\frac{(1-\beta_2 + \beta)}{\beta_2}
\left ( \frac{1+\beta_2}{1-\beta_2}  
\right )^{1/2} \frac{\sqrt{j_{\max}} v_{\max} }{\sqrt{\batch}}. 
$$
This bounds the stochastic term. Finally, we should note that 
$$
1-\beta_2 + \beta =
1-\beta_2 + \frac{1-\beta_1}{\beta_1} 
= \frac{1-\beta_1\beta_2}{\beta_1}. 
$$
Putting things together gives the result. 
\end{proof}


\subsection{Bounding $\E[Y\tt \dd\phi(X + \epsilon Y)]$ 
with Fisher Information }

We present some key lemmas for bounding the correlation term stemming from stochastic gradient descent. 


\begin{lem}\label{lem:XY}
Let $X,Y$ be two independent $\RR^d$-valued random variables with $\E[Y]=0$, $\var(Y)<+\infty$, $J(X)<+\infty$,  and assume $\phi$ yields a weak derivative $\dd\phi$. We have
$$\E[Y\tt \dd\phi(X+\epsilon Y)] \leq \epsilon 
L_\phi \var(Y) \sqrt{J(X)} 
%\E[\norm{\dd\log \pi_2(X)}_2]. 
$$
\end{lem}
\begin{proof}
For any fixed $y$, 
\bb 
\E[ y\tt \dd\phi(X + \eps y)~|~ Y=y ] 
& = \int y\tt \dd\phi(x + \epsilon y) \pi_X(x) \d x \\ 
& = - \int \phi(x + \epsilon y) y \tt \dd \pi_X(x) \d x \\ 
& = - \E[ y \tt \dd \log \pi_X(X) \phi(X + \epsilon y) ~|~ Y=y ].  \ant{$\dd\log \pi_X(x)= \dd\pi_X(x)/\pi_X(x)$}
\ee 
Then taking expectation on $Y$: 
\bb 
\E[ Y\tt \dd\phi(X + \eps Y) ] 
& = - \E [Y \tt \dd \log \pi_X(X) \phi(X + \epsilon Y) ] \\
& = - \E [Y \tt \dd \log \pi_X(X) (\phi(X + \epsilon Y) - \phi(X)) ] \ant{using $\E[Y]=0$}\\
& \leq \epsilon  L_\phi  \E [\abs{Y\tt \log \pi_X(X)}\norm{Y}_2]  \\
& \leq \epsilon L_\phi \E[\norm{Y}_2^2] \E[\norm{\dd \log \pi_X(X)}_2] \\
& \leq \epsilon L_\phi \E[\norm{Y}_2^2] \sqrt{\E[\norm{\dd \log \pi_X(X)}^2_2]}  \\
& = \epsilon L_\phi \var(Y) \sqrt{J(X)}. 
\ee 

\begin{mydef}
The Fisher information of a random variable $X$ on $\RR^d$, if exists, is defined as
$$
J(X) = \E\left [\norm{\dd \log \pi(X)}_2^2 \right ], 
$$
where $\pi(x)$ denotes the density function of $X$. 
\end{mydef}


%@article{dembo1991information, title={Information theoretic inequalities},author={Dembo, Amir and Cover, Thomas M and Thomas, Joy A},journal={IEEE Transactions on Information theory},volume={37},number={6},pages={1501--1518},year={1991},publisher={IEEE}}
\begin{lem}\citep{dembo1991information} \label{lem:cover}
For any two independent random variables $X$ and $Y$, we have
$$
J(\sqrt{\lambda }X + \sqrt{1-\lambda} Y) \leq 
\lambda J(X) + (1-\lambda )J(Y), ~~~~~\forall \lambda \in[0,1], 
$$
$$
J(X)^{-1} + J(Y)^{-1} \leq  J(X + Y)^{-1}. 
$$
\end{lem} 


\begin{lem}\label{lem:Jineq}
Let $X, X_1,\ldots, X_n$ be independent random variables on $\RR^d$, and $a, a_1,\ldots a_n \in \RR$. We have 
\bb 
& J(a_1 X_1 + \cdots +  a_n X_n)
\leq  (a_1^2+\cdots  + a_n^2)^{-1} (\sum_{i=1}^n w_i J(X_i)^{-1})^{-1},
\ee 
where $w_i = a_i^2/(a_1^2+\cdots  + a_n^2).$
\end{lem}

\begin{proof}
Let us first prove that $J(a X)^{-1} = {a^2}J(X)^{-1}$. 
To see this, let $Y = aX$, and $\pi_X$ and $\pi_Y$ their density functions.  We have $\pi_Y(y) = \pi_X(y/a)/a$. 
Hence 
\bb 
J(Y) = \E[\norm{\dd \log \pi_Y(Y)}^2] 
= \E [ \norm{(\dd \log \pi_X(Y/a))/a}^2]
= \frac{1}{a^2}\E [ \norm{\dd \log \pi_X(X)}^2] 
= \frac{1}{a^2} J(X). 
\ee 

Using Lemma~\ref{lem:cover}, we get 
\bb 
J(a_1 X_1 + \cdots + a_n X_n) 
& \leq  (\sum_{i=1}^n J(a_i X_i)^{-1})^{-1} \\
& =  (\sum_{i=1}^n  a_i^2 J( X_i)^{-1})^{-1} \\
& = (a_1^2 + \cdots + a_n^2)^{-1} (\sum_{i=1}^n w_i J(X_i)^{-1})^{-1}. 
\ee 
\end{proof} 






\begin{lem}\label{lem:fisher} 
Assume $m_{t+1} = \beta_2 m_t + (1-\beta_2) g_t$, where  $\beta_2\in(0,1)$, 
 and $m_0, g_0, \ldots g_t$ are independent random variables, with $J_{\max} = \max(\max_{i\leq t} J(g_i), J(m_0)),$ we have 
 $$
J(m_{t})
\leq \frac{1+\beta_2}{1-\beta_2}  J_{\max} . 
$$
\end{lem}

\begin{proof}
\bb
m_{t+1} = (1-\beta_2) (g_t + \beta_2 g_{t-1} + \cdots  \beta^{t}_2 g_0) + \beta_2^{t+1} m_0.  
\ee 
Note that 
\bb 
(1-\beta_2)^2 (1 + \beta_2^{2} + \cdots + \beta_2^{2t}) + \beta_2^{2(t+1)}
& = (1-\beta_2)^2 \frac{1-\beta_2^{2(t+1)}}{1-\beta_2^2}  + \beta_2^{2(t+1)} \\ 
& = \frac{(1-\beta_2)(1-\beta_2^{2(t+1)})}{1+\beta_2} + \beta_2^{2(t+1)}  \\
& \geq 
\frac{(1-\beta_2)(1-\beta_2^{2(t+1)})}{1+\beta_2} + \frac{1-\beta_2}{1+\beta_2} \beta_2^{2(t+1)}  \\
& = \frac{1-\beta_2}{1+\beta_2}. 
\ee 
Using Lemma~\ref{lem:Jineq} gives the result.


\begin{thm}\label{thm:dist_weaksmooth}

\textbf{[Distributed Training Convergence Analysis]} 

Distributed Training our framework follows this scheme: 
\bb
&x_{t+1} = x_t - \epsilon \frac{1}{N}\sum_{i=1}^N\dd\phi(\tilde m_{t+1,i})\\
&\tm_{t,i} = m_{t,i} + \beta g_{t,i}\\
&m_{t+1,i} = \beta_2 m_{t,i} + (1-\beta_2) g_{t,i}
\ee 
Assume $N$ is the number of distributed workers. Assume $f$ is $\phi$-weak smooth  as above  
and lower bounded ($\inf_x f(x) >-\infty$), and $\phi$ is convex and $q$-homogeneous for $q\in\RR$. 
Let  $\dd \phi$ be both a subgradient  and a weak derivative 
of $\phi$ with $\dd \phi(0) = 0$. 
 Assume $\phi$ is $L_\phi$-Lipschitz.  
Assume $\sup_{t,i} \norm{\dd\phi(m_{t,i})}_2\defeq D < +\infty$. 
We have when $\epsilon \leq \min\left (\frac{L_3}{D}, \frac{1}{L_1 D} \left (\frac{1+\beta_2}{1-\beta_2}\right)^{q} \right )$,
$$
\frac{1}{N(T+1)}\sum_{t=0}^T  \sum_{i=1}^N \E[ D_{\phi_{m_{t,i}},\beta}(g_{t,i}, 0) ]
+  \E[ D_\phi(m_{t+1,i},0)  ] 
%= O\left (
\leq 
\frac{A}{\epsilon T} + B \epsilon + 
\frac{1-\beta_1\beta_2}{\sqrt{1-\beta_2} \sqrt{\batch}} C, 
%\frac{(H_0 - H_{T+1}) + \frac{L d \epsilon^2}{2} }{\epsilon T}. 
$$ 
where $A = f(x_0) - \inf_{x} f(x)$  and $B = L_0 D^2/2$,
and $C = \frac{\sqrt{1+\beta_2}}{\beta_1\beta_2}
v_{\max} \sqrt{j_{\max}} L_\phi$. 
\end{thm}



\begin{proof}
Assume $\E[g_{t,i}] = \dd f(x_t)$. 
Let $\tm_{t,i} = m_{t,i} + \beta g_{t,i}$. 
Let $D^2 = \sup_m \norm{\dd\phi(m)}_2^2$. 
By the $\phi$-weak smoothness of $f$,  when $\norm{x_{t+1} - x_t}_2 = \epsilon \norm{\frac{1}{N}\sum_{i=1}^N\dd\phi(\tilde m_{t+1,i})}_2 \leq \epsilon D  \leq L_3$, or $\epsilon \leq L_3/D$, 
we have 
\bb 
f(x_{t+1}) - f(x_t) 
\leq  - \lr  \dd f(x_t)\tt  \frac{1}{N}\sum_{i=1}^N \dd\phi(\tilde m_{t+1,i})  +
\frac{1}{2} \epsilon^2 (\bar L_0 + \bar L_1 \phi(\dd f(x_t))), 
%+   B_f(x_t -\lr \dd\phi(\tm_{t+1}), x_t) 
%\frac{\lr^2}{2} 
% \dd\phi(\tilde m_{t+1})  \tt \dd^2f(x_t) 
 % \dd\phi(\tilde m_{t+1}) 
%  + O(\lr^3 \norm{ \dd\phi(\tilde m_{t+1})}^3). 
\ee 
where $\bar L_0 = L_0 D^2$ and $\bar L_1 = L_1 D^2$. 
By the convexity of $\phi$: 
\bb 
\phi(m_{t+1,i}) - \phi(m_t,i) 
& \leq \lambda  \dd\phi(m_{t+1,i}) \tt ( g_{t,i}  - m_{t+1,i}) \\ 
& = \lambda \dd\phi(m_{t+1,i}) \tt  g_{t,i}  
- \lambda  D_\phi(m_{t+1,i},0)
%\dd\phi(m_{t+1}) \tt m_{t+1}. 
\ee 
Let 
$H_t =  f(x_t) + \frac{\epsilon}{\lambda N}\sum_{i=1}^N \phi(m_{t,i})$. We have 
\bb 
H_{t+1} - H_t 
\leq - 
\lr \left(\frac{1}{N}\sum_{i=1}^N D_{\phi_{m_{t,i}, \beta}}(g_{t,i}, 0) 
+ D_\phi(m_{t+1,i},0) 
- V_{t,i} \right)
+  \frac{\bar L_0}{2} \epsilon^2 +
\frac{\bar L_1}{2}  \epsilon^2 \phi(\dd f(x_t)),
\ee 
where $ V_{t,i} = (g_{t,i} - \dd f(x_t))\tt\dd\phi(\tilde m_{t+1,i})$ and it is the term that stems from the stochastic gradient. 

Summing over $t$ and using Lemma~\ref{lem:m2df}:
\bb
&\frac{1}{N(T+1)}\sum_{t=0}^T \sum_{i=1}^N \frac{1}{\beta} D_{\phi_{m_{t,i},\beta}}(g_{t,i}, 0) 
+ (1 - \frac{\bar L_1}{2} \epsilon \left (\frac{1+\beta_2}{1-\beta_2}\right)^q ) D_\phi(m_{t+1,i},0) \\
&\quad \quad \quad \qquad \leq 
\frac{(H_0 - H_{T+1}) + \frac{T \bar L_0 \epsilon^2}{2} }{\epsilon (T+1)} + 
\bar V,
\ee
where $\bar V = \sum_{t=0}^T \sum_{i=1}^N V_{t,i}/(N(T+1))$. 
%Choosing

\bb
\E \left[\frac{1}{N}\sum_{i=1}^N V_{t,i} \right] &= \E \left[ \frac{1}{N}\sum_{i=1}^N (g_{t,i} - \dd f(x_t))\tt\dd\phi(\tilde m_{t+1,i})\right] \\
& \leq \E \left[ \frac{1}{N}\sum_{i=1}^N (g_{t,i} - \dd f(x_t))\tt\dd\phi(\tilde m_{t+1,i})\right]
\ee 
Choosing $\epsilon \leq \frac{1}{\bar L_1} \left (\frac{1-\beta_2}{1+\beta_2}\right)^q$. We get  
$$
\E 
\left [ \frac{1}{N(T+1)}\sum_{t=0}^T \sum_{i=1}^N \frac{1}{\beta}D_{\phi_{m_{t,i},\beta}}(g_t, 0) 
+\frac{1}{2} D_\phi(m_{t+1,i},0)  \right ]  
\leq 
\frac{\E \left [(H_0 - H_{T+1}) \right]}{\epsilon (T+1)}  + 
\frac{\bar L_0  \epsilon}{2} +\E [\bar V], 
$$ 
where
$$
\E[\bar V] = \frac{1}{N(T+1)} 
\sum_{t=0}^T \sum_{i=1}^N \cov(g_{t,i}, \dd \phi(\tilde m_{t+1,i})),
$$
where $\cov(g_{t,i}, \dd\phi(\tilde m_{t+1,i})) 
= \E[(g_{t,i} - \dd f(x_t)) \dd\phi(\tilde m_{t+1,i})]$. 
Note that 
$$
\tm_{t+1,i} = \beta_2 m_{t,i} + (1-\beta_2 + \beta) g_{t,i}. 
$$
We expect that the correlation term decreases with $(1-\beta_2)$ and $\beta$, as in this case the contribution of $g_{t,i}$ inside $\tilde m_{t+1,i}$ decreases. 
Using
Lemma~\ref{lem:XY} and 
Lemma~\ref{lem:fisher}, we have 
$$
\E[V_{t,i}] 
\leq (1-\beta_2 + \beta) L_\phi \var(g_{t,i}) \sqrt{J(\beta_2 m_{t,i})}  
\leq 
\frac{(1-\beta_2 + \beta)}{\beta_2}
\left ( \frac{1+\beta_2}{1-\beta_2}  
\right )^{1/2} \frac{\sqrt{j_{\max}} v_{\max} }{\sqrt{\batch}}. 
$$
This bounds the stochastic term. Finally, we should note that 
$$
1-\beta_2 + \beta =
1-\beta_2 + \frac{1-\beta_1}{\beta_1} 
= \frac{1-\beta_1\beta_2}{\beta_1}. 
$$
Putting things together gives the result. 
\end{proof}
% {\color{blue}

% \begin{lem}
% Assume $m_{t+1} = \beta_2 m_t + (1-\beta_2) g_t$, where  $\beta_2\in(0,1)$, 
%  and $m_0, g_0, \ldots g_t$ are independent random variables, with $J_{\max} = \max(\max_{i\leq t} (1-\beta_2)^{-1}\beta_2^{i-t} J(g_i) , \beta_2^{-t-1}J(m_0)),$ we have 
%  $$
% J(m_{t})
% \leq 
% \frac{1}{t+1}\frac{1+\beta_2}{1-\beta_2}  J_{\max} . 
% $$
% \end{lem}

% \begin{proof}
% \bb
% m_{t+1} = (1-\beta_2) (g_t + \beta_2 g_{t-1} + \cdots  \beta^{t}_2 g_0) + \beta_2^{t+1} m_0.  
% \ee 
% Note that 
% \bb 
% (1-\beta_2)^2 (1 + \beta_2^{2} + \cdots + \beta_2^{2t}) + \beta_2^{2(t+1)}
% & = (1-\beta_2)^2 \frac{1-\beta_2^{2(t+1)}}{1-\beta_2^2}  + \beta_2^{2(t+1)} \\ 
% & = \frac{(1-\beta_2)(1-\beta_2^{2(t+1)})}{1+\beta_2} + \beta_2^{2(t+1)}  \\
% & \geq 
% \frac{(1-\beta_2)(1-\beta_2^{2(t+1)})}{1+\beta_2} + \frac{1-\beta_2}{1+\beta_2} \beta_2^{2(t+1)}  \\
% & = \frac{1-\beta_2}{1+\beta_2}. 
% \ee 

% By HM-GM inequality, we have
% \bb
% J(a_1 X_1 + \cdots +  a_n X_n) &\leq (a_1^2+\cdots  + a_n^2)^{-1} (\sum_{i=1}^n w_i J(X_i)^{-1})^{-1} \\
% &\leq (a_1^2+\cdots  + a_n^2)^{-1} \frac{1}{n} \left(\prod_{i=1}^n \frac{J(X_i)}{w_i}\right)^{\frac{1}{n}} \\
% \ee
% Using Lemma~\ref{lem:Jineq} gives the result.

% \end{proof} 

%  }

==> old_content/drafts.tex <==

\newpage \clearpage 
\textbf{\red{Uncleaned Derivations ======= }}

\subsection{$\phi > f^*$}
$$
f(x^*) \geq f(x) + \dd f(x) \tt (x^* - x), 
$$
hence $\dd f(x) \tt (x^*-x) \leq -(f(x) - f(x^*))$. 

\bb 
\ddt (-(x_t-x^*)\tt  m_t)
& = 
\dd\phi(\tilde m_t) \tt  m_t 
- (x_t-x^*) \tt (\dd f(x_t) - \eta m_t)  \\
& = 
\dd\phi(\tilde m_t) \tt  m_t 
- (x_t-x^*) \tt \dd f(x_t) + \eta (x_t-x^*)\tt  m_t    \\
& = 
\dd\phi(\tilde m_t) \tt ( \tilde  m_t  - \beta \dd f(x_t))
- (x_t-x^*) \tt \dd f(x_t) + \eta (x_t-x^*)\tt  m_t    \\
& = \dd\phi(\tilde m_t) \tt  \tilde  m_t  - 
 \beta \dd\phi(\tilde m_t) \tt   \dd f(x_t) 
- (x_t-x^*) \tt \dd f(x_t) + \eta (x_t-x^*)\tt  m_t    \\
\ee 
Hence
\bb 
& \ddt ( f(x_t) +  \phi(\tilde m_t)- \eta (x_t-x^*)\tt  m_t) \\ 
& =  - \dd f(x_t) \tt \dd\phi(\tilde m_t) + \cdots \\ 
& + (1 + \eta \beta) \dd \phi(\tilde m_t) \tt \dd f(x_t) 
- \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
- \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) + \cdots \\
& +  
\eta \dd\phi(\tilde m_t) \tt  \tilde  m_t  - 
 \eta \beta \dd\phi(\tilde m_t) \tt   \dd f(x_t) 
- \eta (x_t-x^*) \tt \dd f(x_t) + \eta^2 (x_t-x^*)\tt  m_t    \\ 
& =   
- \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)   
- \eta (x_t-x^*) \tt \dd f(x_t) + \eta^2 (x_t-x^*)\tt  m_t  \\
&\leq  - \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)   
-\eta (f(x_t) -f(x^*)) + \eta^2 (x_t-x^*)\tt  m_t. 
\ee 

\bb 
\ddt H_2(x_t,m_t)  =  
- \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
-\beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t). 
\ee 


\bb 
& \ddt (f(x_t) +  \phi(\tilde m_t)- \eta (x_t-x^*)\tt  m_t + \red{ a H_2(x_t,m_t)} ) \\ 
&\leq  - \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)   
-\eta (f(x_t) -f(x^*)) + \eta^2 (x_t-x^*)\tt  m_t+ \cdots  \\
& \red{- a \eta  \phi(\tilde m_t) 
-a \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)} + 
\ee 

\bb 
H_3(x_t,m_t) = (1+a (1+\eta \beta ) ) f(x_t) + (1+a) \phi(\tilde m_t)
 - \eta (x_t-x^*)\tt  m_t 
\ee

Define 
$$\Delta  = (\beta + a \beta ) \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)   .
$$

\bb 
\ddt H_3(x_t,m_t) 
\leq 
&   -\Delta  
-\eta \bigg [  (f(x_t) -f(x^*)) - \eta (x_t-x^*)\tt  m_t 
+ a   \phi(\tilde m_t)  \bigg ]
\ee 

Let  $a = 1/\sqrt{1+\eta \beta}$ to minimize $\min(1+a(1+\mu\beta), (1+a)/a)$, then 
\bb 
H_3(x_t,m_t) = (1+\sqrt{1+\eta \beta} )( f(x_t) + \frac{1}{\sqrt{1+\eta \beta}} \phi(\tilde m_t))
 - \eta (x_t-x^*)\tt  m_t, 
\ee

and 
\bb 
\ddt H_3(x_t,m_t) = - \Delta - \eta ()
%(1+\sqrt{1+\eta \beta} )( f(x_t) + \phi(\tilde m_t)) - \eta (x_t-x^*)\tt  m_t, 
\ee 

\red{=====}

\bb 
& \ddt (f(x_t) +  \phi(\tilde m_t)- \eta (x_t-x^*)\tt  m_t + \red{ a H_2(x_t,m_t)} + \blue{b H(x_t, m_t)}) \\ 
&\leq  - \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)   
-\eta (f(x_t) -f(x^*)) + \eta^2 (x_t-x^*)\tt  m_t+ \cdots  \\
& \red{- a \eta  \phi(\tilde m_t) 
-a \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)} + \blue{(- b D_\phi(\tilde m_t, m_t) - b\eta \phi(m_t))}
\ee 

\bb 
H_3(x_t,m_t) = (1+a (1+\eta \beta ) + b) f(x_t) + (1+a) \phi(\tilde m_t)
+   b \phi(m_t)  - \eta (x_t-x^*)\tt  m_t 
\ee

Define 
$$\Delta  = (\beta + a \beta ) \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)   + b D_\phi(\tilde m_t, m_t). 
$$

\bb 
\ddt H_3(x_t,m_t) 
\leq 
&   -\Delta  
-\eta \bigg [  (f(x_t) -f(x^*)) - \eta (x_t-x^*)\tt  m_t 
+ a   \phi(\tilde m_t)  + b \phi(m_t) \bigg ]
\ee 

\bb 
\ddt \phi(\tilde m_t)  & = 
(1 + \eta \beta) \dd \phi(\tilde m_t) \tt \dd f(x_t) 
- \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
- \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) \\ 
 & \leq 
(1 + \eta \beta) \dd \phi(\tilde m_t) \tt \dd f(x_t) 
- \eta \phi(\tilde m_t)  
- \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) \\
\ee 

\bb 
\ddt (-(x_t-x^*)\tt \tilde m_t)
& = 
\dd\phi(\tilde m_t) \tt \tilde m_t 
- (x_t-x^*) \tt (\dd f(x_t) - \eta m_t - \beta \dd^2 f(x_t) \dd\phi(\tilde m_t) )  \\
& = 
\dd\phi(\tilde m_t) \tt \tilde m_t 
- (x_t-x^*) \tt \dd f(x_t) + (x_t-x^*)\tt \eta m_t + 
\beta (x_t-x^*) \tt  \dd^2 f(x_t) \dd\phi(\tilde m_t)   \\
\ee 

Write $\tilde m_t = m_t + \beta \dd f(x_t)$. We have 
\bb 
\ddt f(x_t)   &  = - 
\dd f(x_t)\tt \dd\phi(\tilde m_t) \\ 
\ddt \phi(m_t) & = \dd \phi(m_t) \dd f(x_t) 
- \eta \dd \phi(m_t) m_t  \\ 
\ddt \phi(\tilde m_t) & = 
\dd \phi(\tilde m_t) \tt \dd f(x_t) 
- \eta \dd \phi(\tilde m_t) \tt m_t  
- \beta  \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) \\
& = 
\dd \phi(\tilde m_t) \tt \dd f(x_t)
- \eta \dd \phi(\tilde m_t) \tt (\tilde m_t  - \beta \dd f(x_t))
- \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) \\ 
& = 
(1 + \eta \beta) \dd \phi(\tilde m_t) \tt \dd f(x_t) 
- \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
- \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) \\ 
\ee 
Hence, define 
\bb 
H_2(x,m) =  (1+\eta \beta )f(x_t) +  \phi(m_t + \beta \dd f(x_t))
\ee 
Then 
\bb 
\ddt H_2(x,m) & =
 (1+\eta \beta) (- \dd f(x_t) \tt \dd \phi(\tilde m_t) )   + \cdots \\ 
& ~~~ + (1 + \eta \beta) \dd \phi(\tilde m_t) \tt \dd f(x_t) 
- \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
-\beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) \\ 
& =  
- \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
-\beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)  \leq 0. 
\ee 


\subsection{When $\phi\geq f^*$}
Write $\tilde m_t = m_t + \beta \dd f(x_t)$. We have 
\bb 
\ddt f(x_t)   &  = - 
\dd f_t\tt \dd\phi(\tilde m_t) \\
\ddt \phi(m_t) & = \dd \phi(m_t) \dd f_t 
- \eta \dd \phi(m_t) \dd m_t  \\ 
\ddt \phi(\tilde m_t) & = 
\dd \phi(\tilde m_t) \tt \dd f_t 
- \eta \tphi_t \tt m_t  
- \dd\tphi_t \tt \dd^2 f_t  \dd\tphi_t. 
\ee 
Hence 
\bb 
 - \dd f_t\tt \dd\phi(\tilde m_t) + w_1( \dd \phi(m_t) \dd f_t 
- \eta \dd \phi(m_t) \dd m_t ) 
+ 
w_2 (\dd \phi(\tilde m_t) \tt \dd f_t 
- \eta \tphi_t \tt m_t  
- \dd\tphi_t \tt \dd^2 f_t  \dd\tphi_t).
\ee 

\bb 
 - \dd f_t\tt \dd\phi(\tilde m_t) + w_1( \dd \phi(m_t) \dd f_t 
- \eta \dd \phi(m_t) \dd m_t ) 
+ 
w_2 (\dd \phi(\tilde m_t) \tt \dd f_t 
- \eta \tphi_t \tt m_t  
- \dd\tphi_t \tt \dd^2 f_t  \dd\tphi_t).
\ee 


\section{Conjugate of Bregman Divergence}
\label{sec:ht}


\newpage\clearpage 

\section{Simple Discrete Analysis: $\beta_2 = \epsilon \alpha$.}
Consider the following semi-implicit Euler scheme of \eqref{equ:lionode}:  
\bb 
m_{t+1} &= m_t + \epsilon (\alpha \dd f(x_t)  - \eta m_{t+1}) \\
x_{t+1} &= x_t - \epsilon\dd\phi( m_{t+1} + \beta \dd f(x_t)),
\ee 
where $\epsilon >0$ is the step size. 

\begin{thm}
Assume $f$ is \red{$L_f$}-smooth and lower bounded ($\inf_x f(x) >-\infty$), and $\phi$ is convex and $\dd \phi$ a subgradient of it with $\dd \phi(0) = 0$.     \red{$\norm{\dd\phi(m)}_2$ is upper bounded.} 
We have 
$$
\frac{1}{T}\sum_{t=0}^T \frac{1}{\beta} D_\phi(\tilde m_{t+1}, m_{t+1}) 
+ \frac{\eta}{\alpha} D_\phi(m_{t+1},0)
= O\left (
\frac{1}{\epsilon T} + \epsilon  
\right ). 
%\frac{(H_0 - H_{T+1}) + \frac{L d \epsilon^2}{2} }{\epsilon T}. 
$$ 
\end{thm} 
\begin{proof}
Let $\tm_t = m_t + \beta\dd f(x_t)$. 
By the smoothness of $f$ and the boundedness of $\dd \phi(\tilde m_{t+1})$, 
\bb 
f(x_{t+1}) - f(x_t) 
\leq  - \lr  \dd f(x_t)\tt  \dd\phi(\tilde m_{t+1})  +
\frac{L}{2} d \epsilon^2. 
%+   B_f(x_t -\lr \dd\phi(\tm_{t+1}), x_t) 
%\frac{\lr^2}{2} 
% \dd\phi(\tilde m_{t+1})  \tt \dd^2f(x_t) 
 % \dd\phi(\tilde m_{t+1}) 
%  + O(\lr^3 \norm{ \dd\phi(\tilde m_{t+1})}^3). 
\ee 
By the convexity of $\phi$: 
\bb 
\phi(m_{t+1}) - \phi(m_t) 
& \leq \lr \alpha  \dd\phi(m_{t+1}) \tt (\dd f(x_t) - \eta m_{t+1}) \\ 
& = \lr \alpha \dd\phi(m_{t+1}) \tt  \dd f(x_t) 
- \lr \eta  D_\phi(m_{t+1},0)
%\dd\phi(m_{t+1}) \tt m_{t+1}. 
\ee 
Let 
$H_t = f(x_t) + \frac{1}{\alpha} \phi(m_t)$. We have 
\bb 
H_{t+1} - H_t 
\leq - 
\frac{\lr}{\beta} D_\phi(\tilde m_{t+1}, m_{t+1}) 
- \frac{\lr \eta}{\alpha} D_\phi(m_{t+1},0) +  \frac{L}{2} d \epsilon^2. 
%B_f(x_{t}-\lr \dd \phi(\tm_{t+1}), x_t).  
\ee 
Hence 
$$
\sum_{t=0}^T \frac{1}{\beta} D_\phi(\tilde m_{t+1}, m_{t+1}) 
+ \frac{\eta}{\alpha} D_\phi(m_{t+1},0)
\leq
\frac{(H_0 - H_{T+1}) + \frac{L d \epsilon^2}{2} }{\epsilon T}. 
$$ 
\end{proof}


\subsection{\red{Try to use a weaker smoothness condition}}
Assume $f$ satisfies 
$$
f(y) - f(x) 
\leq   \dd f(x)\tt (y-x)  +
\frac{1}{2} (L_0 + L_1 \phi(\dd f(x))) \norm{y-x}^2_2
$$
for some $L_0,L_1 <+\infty$. 
\begin{thm}
\end{thm}
\begin{proof}
Let $\tm_t = m_t + \beta\dd f(x_t)$. 
Then 
\bb 
f(x_{t+1}) - f(x_t) 
\leq  - \lr  \dd f(x_t)\tt  \dd\phi(\tilde m_{t+1})  +
\frac{1}{2} d \epsilon^2 (L_0 + L_1 \phi(\dd f(x_t))). 
%+   B_f(x_t -\lr \dd\phi(\tm_{t+1}), x_t) 
%\frac{\lr^2}{2} 
% \dd\phi(\tilde m_{t+1})  \tt \dd^2f(x_t) 
 % \dd\phi(\tilde m_{t+1}) 
%  + O(\lr^3 \norm{ \dd\phi(\tilde m_{t+1})}^3). 
\ee 
By the convexity of $\phi$: 
\bb 
\phi(m_{t+1}) - \phi(m_t) 
& \leq \beta_2  \dd\phi(m_{t+1}) \tt (\dd f(x_t) - m_{t+1}) \\ 
& = \beta_2 \dd\phi(m_{t+1}) \tt  \dd f(x_t) 
- \beta_2  D_\phi(m_{t+1},0)
%\dd\phi(m_{t+1}) \tt m_{t+1}. 
\ee 
Let 
$H_t = f(x_t) + \frac{\epsilon}{\beta_2} \phi(m_t)$. 
We have 
\bb 
H_{t+1} - H_t 
\leq - 
\frac{\lr}{\beta} D_\phi(\tilde m_{t+1}, m_{t+1}) 
- \frac{\lr \eta}{\alpha} D_\phi(m_{t+1},0) 
+  \frac{L_0}{2} d \epsilon^2 +
\frac{L_1}{2} d \epsilon^2 \phi(\dd f(x_t)). 
\ee 
%Hence 
Summing over $t$ and using Lemma~\ref{lem:m2dfbound}:
$$
\sum_{t=0}^T \frac{1}{\beta} D_\phi(\tilde m_{t+1}, m_{t+1}) 
+ (\frac{\eta}{\alpha} - \frac{L_1}{2} d \epsilon \left (\frac{2+\epsilon \eta}{\epsilon \alpha}\right)^q ) D_\phi(m_{t+1},0)  
\leq 
\frac{(H_0 - H_{T+1}) + \frac{L_0 d \epsilon^2}{2} }{\epsilon T} 
%+ \frac{L_1 d \epsilon^2}{2} }{\epsilon T} 
$$ 
%Choosing
When $q < 1$, we can choose $\epsilon $ sufficiently small such that 
$ \frac{L_1}{2} d \epsilon \left (\frac{2+\epsilon \eta}{\epsilon 
\alpha}\right)^q  \geq \frac{\eta}{\alpha}$.  \red{But $q<1$ is not reasonable.}
\end{proof}


\begin{lem}\label{lem:m2dfbound} 
Assume $m_{t+1} = m_t + \epsilon (\alpha \dd f(x_t) - \eta m_{t+1})$ 
starting from $m_{-1} = 0$, 
and $\phi$ is convex and $\phi$ is $q$-homogeneous. Then 
$$
\phi(\dd f(x_t)) \leq \frac{1+\beta_2}{\bar\beta_2} (\phi(m_{t+1}) + \beta_2 \phi(m_t)).
$$
Hence 
$$
\sum_{t=0}^T \phi(\dd f(x_t)) 
\leq \left(\frac{2+\epsilon \eta}{\epsilon \alpha}\right)^q \sum_{t=0}^T \phi(m_{t+1}) 
\leq \left(\frac{2+\epsilon \eta}{\epsilon \alpha}\right)^q \sum_{t=0}^T \phi'(m_{t+1}) m_{t+1}.
$$
\end{lem} 
\begin{proof}
We have $m_{t+1} = \beta_2 m_t + \bar \beta_2 \dd f(x_t)$ with 
$\beta_2 = \frac{1}{1+\epsilon \eta}$ and $\bar\beta_2  = \frac{\epsilon \alpha}{1 + \epsilon \eta}$. 

Hence, $\dd f(x_t) = \frac{m_{t+1} - \beta_2 m_t}{\bar \beta_2}$, and 
%Because $\phi$ is convex and $\phi(0)=0$, we have for any $a \in[0,1]$, $\phi(ax) \leq a \phi(x).$
\bb 
\phi(\dd f(x_t)) & =  \phi\left (\frac{m_{t+1} - \beta_2 m_t}{\bar \beta_2} \right )  \\
& =\left (\frac{1+\beta_2}{\bar\beta_2}\right)^q 
\phi\left ( 
\frac{m_{t+1} + \beta_2 (-m_t)}{1+\beta_2}
\right ) \\ 
& \leq \frac{(1+\beta_2)^{q-1}}{(\bar\beta_2)^q}
(\phi ( m_{t+1}) + \beta_2 \phi(m_t)). 
\ee 
Let $A = \frac{(1+\beta_2)^{q-1}}{(\bar\beta_2)^q}$. 
Summing over $t$: 
\bb 
\sum_{t=0}^T \phi(\dd f(x_t)) \leq \frac{(1+\beta_2)^{q-1}}{(\bar\beta_2)^q} \left ( \sum_{t=0}^T \phi(m_{t+1}) + \beta_2  \sum_{t=0}^{T-1}\phi(m_{t+1}))  \right ) 
\leq \frac{(1+\beta_2)^{q}}{(\bar\beta_2)^q} \sum_{t=0}^T \phi(m_{t+1}). 
\ee 
Finally, we note that 
$$
\frac{(1+\beta_2)^{q}}{(\bar\beta_2)^q}  
= \left (\frac{2+\epsilon \eta}{\epsilon \alpha}\right)^q. 
$$
\end{proof} 











\newpage\clearpage 

\subsection{Proof of Theorem~\ref{thm:strong_smooth}}


\begin{proof}
Let  $\tilde m_{t+1} = m_{t+1} + \beta \nabla f(x_t)$. 
By the smoothness of $f$  and boundedness of $\norm{\dd\phi(m_t)}_2 \leq D$, 
\bb 
f(x_{t+1}) - f(x_t) 
\leq  - \lr  \dd f(x_t)\tt  \dd\phi(\tilde m_{t+1})  +
\frac{L}{2} D^2 \epsilon^2, 
\ee 
%where $L = L_f \sup_m \norm{\dd\phi(m)}^2_2$. 
%we used that $dfd$
By the convexity of $\phi$: 
\bb 
\phi(m_{t+1}) - \phi(m_t) 
& \leq \nabla \phi(m_{t+1}) \lambda (\nabla f(x_t) - m_{t+1}) \\ 
& = \lambda \dd\phi(m_{t+1}) \tt  \dd f(x_t) 
- \lambda D_\phi(m_{t+1},0), 
%\dd\phi(m_{t+1}) \tt m_{t+1}. 
\ee 
where $\lambda = \frac{1-\beta_2}{\beta_2}$, 
and we used that $m_{t+1} = m_t + \lambda (g_t - m_{t+1})$. 

Let 
$H_t = f(x_t) + \frac{\epsilon}{\lambda } \phi(m_t)$. We have 
\bb 
H_{t+1} - H_t 
\leq - 
\frac{\lr}{\beta} D_{\phi_{m_t,\beta}}(\dd f(x_t), 0) 
- \lr  D_\phi(m_{t+1},0) +  \frac{L}{2} d \epsilon^2. 
%B_f(x_{t}-\lr \dd \phi(\tm_{t+1}), x_t).  
\ee 
Hence 
$$
\frac{1}{T+1}\sum_{t=0}^T \frac{1}{\beta}  D_{\phi_{m_t,\beta}}(\dd f(x_t), 0) 
+  D_\phi(m_{t+1},0)
\leq
\frac{(H_0 - H_{T+1}) + \frac{L d \epsilon^2}{2} }{\epsilon (T+1)}. 
$$ 
\end{proof}

\subsection{Proof of Theorem~\ref{thm:weaksmooth}}
\begin{proof}
Let $\tm_t = m_t + \beta\dd f(x_t)$. 
Let $D^2 = \sup_m \norm{\dd\phi(m)}_2^2$. 
By the $\phi$-weak smoothness of $f$,  when $\norm{x_{t+1} - x_t}_2 = \epsilon \norm{\dd\phi(\tilde m_{t+1})}_2 \leq \epsilon D  \leq L_3$, or $\epsilon \leq L_3/D$, 
we have 
\bb 
f(x_{t+1}) - f(x_t) 
\leq  - \lr  \dd f(x_t)\tt  \dd\phi(\tilde m_{t+1})  +
\frac{1}{2} \epsilon^2 (\bar L_0 + \bar L_1 \phi(\dd f(x_t))), 
%+   B_f(x_t -\lr \dd\phi(\tm_{t+1}), x_t) 
%\frac{\lr^2}{2} 
% \dd\phi(\tilde m_{t+1})  \tt \dd^2f(x_t) 
 % \dd\phi(\tilde m_{t+1}) 
%  + O(\lr^3 \norm{ \dd\phi(\tilde m_{t+1})}^3). 
\ee 
where $\bar L_0 = L_0 D^2$ and $\bar L_1 = L_1 D^2$. 
By the convexity of $\phi$: 
\bb 
\phi(m_{t+1}) - \phi(m_t) 
& \leq \lambda  \dd\phi(m_{t+1}) \tt (\dd f(x_t) - m_{t+1}) \\ 
& = \lambda \dd\phi(m_{t+1}) \tt  \dd f(x_t) 
- \lambda  D_\phi(m_{t+1},0)
%\dd\phi(m_{t+1}) \tt m_{t+1}. 
\ee 
Let 
$H_t = f(x_t) + \frac{\epsilon}{\lambda} \phi(m_t)$. We have 
\bb 
H_{t+1} - H_t 
\leq - 
\frac{\lr}{\beta} D_\phi(\tilde m_{t+1}, m_{t+1}) 
- \lr D_\phi(m_{t+1},0) 
+  \frac{\bar L_0}{2} \epsilon^2 +
\frac{\bar L_1}{2}  \epsilon^2 \phi(\dd f(x_t)). 
\ee 
%Hence 
Summing over $t$ and using Lemma~\ref{lem:m2dfbound}:
$$
\sum_{t=0}^T \frac{1}{\beta} D_\phi(\tilde m_{t+1}, m_{t+1}) 
+ (1 - \frac{\bar L_1}{2} \epsilon \left (\frac{1+\beta_2}{1-\beta_2}\right)^q ) D_\phi(m_{t+1},0)  
\leq 
\frac{(H_0 - H_{T+1}) + \frac{T \bar L_0 \epsilon^2}{2} }{\epsilon (T+1)} 
%+ \frac{L_1 d \epsilon^2}{2} }{\epsilon T} 
$$ 
%Choosing
Choosing $\epsilon \leq \frac{1}{\bar L_1} \left (\frac{1-\beta_2}{1+\beta_2}\right)^q$. We get  
$$
\frac{1}{T+1}\sum_{t=0}^T \frac{1}{\beta} D_\phi(\tilde m_{t+1}, m_{t+1}) 
+\frac{1}{2} D_\phi(m_{t+1},0)  
\leq 
\frac{(H_0 - H_{T+1})}{\epsilon (T+1)}  + 
\frac{\bar L_0  \epsilon}{2}. 
$$ 
%sufficiently small such that 
%$ (\frac{\eta}{\alpha} - \frac{L_1}{2} d \epsilon \left (\frac{1+\beta_2}{1-\beta_2}\right)^q ) \geq \frac{\eta}{2\alpha}$.  \red{But $q<1$ is not reasonable.}
\end{proof}


\begin{lem}\label{lem:m2df} 
Assume $m_{t+1} = \beta_2 m_t + \bar \beta_2 \dd f(x_t)$ with $\beta_2,\bar \beta_2>0$, 
starting from $m_{0 } = 0$, 
and $\phi$ is convex and $\phi$ is $q$-homogeneous. Then 
$$
\phi(\dd f(x_t)) \leq \frac{1+\beta_2}{\bar\beta_2} (\phi(m_{t+1}) + \beta_2 \phi(m_t)).
$$
Hence 
$$
\sum_{t=0}^T \phi(\dd f(x_t)) 
\leq \left (\frac{1+ \beta_2}{\bar\beta_2}\right)^q \sum_{t=0}^T \phi(m_{t+1}) 
\leq \left (\frac{1+ \beta_2}{\bar\beta_2} \right)^q \sum_{t=0}^T \phi'(m_{t+1}) m_{t+1}.
$$
\end{lem} 
\begin{proof}
%We have $m_{t+1} = \beta_2 m_t + \bar \beta_2 \dd f(x_t)$ with $\beta_2 = \frac{1}{1+\eta \eta}$ and $\bar\beta_2  = \frac{\epsilon \alpha}{1 + \epsilon \eta}$. 
We have $\dd f(x_t) = \frac{m_{t+1} - \beta_2 m_t}{\bar \beta_2}$, and 
%Because $\phi$ is convex and $\phi(0)=0$, we have for any $a \in[0,1]$, $\phi(ax) \leq a \phi(x).$
\bb 
\phi(\dd f(x_t)) & =  \phi\left (\frac{m_{t+1} - \beta_2 m_t}{\bar \beta_2} \right )  \\
& =\left (\frac{1+\beta_2}{\bar\beta_2}\right)^q 
\phi\left ( 
\frac{m_{t+1} + \beta_2 (-m_t)}{1+\beta_2}
\right ) \\ 
& \leq \frac{(1+\beta_2)^{q-1}}{(\bar\beta_2)^q}
(\phi ( m_{t+1}) + \beta_2 \phi(m_t)). 
\ee 
Let $A = \frac{(1+\beta_2)^{q-1}}{(\bar\beta_2)^q}$. 
Summing over $t$: 
\bb 
\sum_{t=0}^T \dd f(x_t) \leq \frac{(1+\beta_2)^{q-1}}{(\bar\beta_2)^q} \left ( \sum_{t=0}^T \phi(m_{t+1}) + \beta_2  \sum_{t=0}^{T-1}\phi(m_{t+1}))  \right ) 
\leq \frac{(1+\beta_2)^{q}}{(\bar\beta_2)^q} \sum_{t=0}^T \phi(m_{t+1}). 
\ee 
\end{proof} 


\subsection{Proof of Theorem~\ref{thm:weaksmooth2}}

% \begin{thm}\label{thm:weaksmooth2}
% Assume $f$ is $\phi$-weak smooth  as above  
% and lower bounded ($\inf_x f(x) >-\infty$), and $\phi$ is convex and $q$-homogeneous for $q\in\RR$. Let  $\dd \phi$ be a subgradient of $\phi$ with $\dd \phi(0) = 0$.  Assume $\sup_t \norm{\dd\phi(m_t)}_2\defeq D < +\infty$. 
% We have when $\epsilon \leq \min\left (\frac{L_3}{D},  \frac{1}{\kappa L_1(1+\beta)} \left(\frac{1-\beta_2 + \beta}{1 + \beta}\right)^q  \right )$,
% \bb
% \frac{1}{T+1} \sum_{t=0}^T \frac{1}{2(1+ \beta)} D_\phi(\tilde m_{t+1}, 0)  \leq 
% \frac{\tilde A}{\epsilon (T+1)} + \frac{\epsilon D^2}{2}\tilde B
% \ee
% where $\tilde A = (f(x_0) - \inf_{x} f(x))(1+\epsilon)$  and $\tilde B = L_0 D^2/2$. 
% \end{thm}
% \paragraph{Remark}
% The $O(\epsilon)$ term is due to discretization. It can be eliminated by assuming $\dd\phi(m)$ is continuous, which, however, 
% does not include the important case when $\phi$ is a norm function, i.e., $\phi(m) = \norm{m}$, which is discontinuous at $m=0$.

% \paragraph{Remark} 
% This result provides a control on the gradient magnitude $\phi(\dd f(x_t))$, because, by Lemma~\ref{lem:tmbound}, we have under conditions of Theorem~\ref{thm:weaksmooth2}, 
% $$
% \sum_{t=0}^T \phi(\dd f(x_t)) 
% \leq \left(\frac{1+\beta}{1-\beta_2 + \beta}\right)^q \sum_{t=0}^T\left( D_\phi(\tilde m_{t+1}, 0) + \beta D_\phi(m_{t}, 0)\right)
% $$

\begin{proof}
Let  $\tilde m_{t+1} = m_{t+1} + \beta \nabla f(x_t)$, $\tilde m_0 = -\beta \dd f(x_0)$.
By the smoothness of $f$  and boundedness of $\norm{\dd\phi(m)}_2$, 
\bb 
f(x_{t+1}) - f(x_t) 
\leq  - \lr  \dd f(x_t)\tt  \dd\phi(\tilde m_{t+1})  +
\frac{1}{2} \epsilon^2 (\bar L_0 + \bar L_1 \phi(\dd f(x_t))), 
%+   B_f(x_t -\lr \dd\phi(\tm_{t+1}), x_t) 
%\frac{\lr^2}{2} 
% \dd\phi(\tilde m_{t+1})  \tt \dd^2f(x_t) 
 % \dd\phi(\tilde m_{t+1}) 
%  + O(\lr^3 \norm{ \dd\phi(\tilde m_{t+1})}^3). 
\ee 

where $L = L_f \sup_m \norm{\dd\phi(m)}^2_2$. 
%we used that $dfd$
By the convexity of $\phi$: 
\bb 
\phi(m_{t+1}) - \phi(m_t) 
& \leq \nabla \phi(m_{t+1}) \lambda (\nabla f(x_t) - m_{t+1}) \\ 
& = \lambda \dd\phi(m_{t+1}) \tt  \dd f(x_t) 
- \lambda D_\phi(m_{t+1},0)
%\dd\phi(m_{t+1}) \tt m_{t+1}. 
\ee 


\bb 
\phi(\tm_{t+1}) - \phi(\tm_t) 
& \leq \dd \phi(\tm_{t+1}) \tt (\tilde m_{t+1} - \tm_t) \\ 
& \leq \lambda \nabla \phi(\tm_{t+1}) \tt   (\nabla f(x_t) - m_{t+1})  + \beta \dd\phi(\tm_{t+1}) \tt (\dd f(x_t) - \dd f(x_{t-1})) \\ 
& \leq \lambda \nabla \phi(\tm_{t+1}) \tt   ((1+\beta)\dd f(x_t) - \tm_{t+1})  + R\\
& =   \lambda (1+\beta) \nabla \phi(\tm_{t+1}) \tt   \dd f(x_t) -   \lambda D_\phi(\tm_{t+1}, 0)  + R, 
\ee
where
\bb
R \defeq \beta \dd\phi(\tm_{t+1}) \tt (\dd f(x_t) - \dd f(x_{t-1})) \leq \beta \epsilon 
(L_0 + L_1 \phi(\dd f(\blue{x_{t}})))
\norm{\dd \phi(\tilde m_{t+1}) }_2
\norm{\dd\phi(\tm_{t})}_2
\ee 

Let $\tilde H_t = f(x_t) + 
\frac{\epsilon}{\lambda (1+\beta)}
\phi(\tm_{t}).$ 
Then 
\bb 
\tilde H_{t+1} - \tilde H_t
\leq - \frac{\epsilon}{1+\beta} D_\phi(\tm_{t+1}, 0) 
+ 
(L_0 + L_1 \phi(\dd f(\blue{x_t})) )
\frac{\epsilon^2}{2} D^2
\left (
1 + \red{\frac{2 \beta}{\lambda (1+\beta)} }
\right )
\ee 
Denote $\kappa = D^2 \left(1 + \frac{2 \beta}{\lambda (1+\beta)}\right) $

Sum over $t$ and using Lemma~\ref{lem:tmbound}:
\bb
&\frac{1}{T+1} \sum_{t=0}^T \frac{1}{1+ \beta} \left(1- \frac{\epsilon}{2}(1+\beta) \kappa L_1 \left(\frac{1+\beta}{1-\beta_2 + \beta}\right)^q  \right) D_\phi(\tilde m_{t+1}, 0)  \\
& \quad\leq 
\frac{(\tilde H_0 -\tilde H_{T+1}) + \frac{T  L_0 \kappa \epsilon^2}{2} + \epsilon^2\kappa L_1 \beta \left(\frac{1+\beta}{1-\beta_2 + \beta}\right)^q \left( H_0 - H_1 + \frac{L_2}{2}D^2\epsilon T \right) }{\epsilon (T+1)} 
%+ \frac{L_1 d \epsilon^2}{2} }{\epsilon T} 
\ee
%Choosing
Choosing $\epsilon \leq \frac{1}{\kappa L_1(1+\beta)} \left(\frac{1-\beta_2 + \beta}{1 + \beta}\right)^q $. We get  
\bb
&\frac{1}{T+1} \sum_{t=0}^T \frac{1}{2(1+ \beta)} D_\phi(\tilde m_{t+1}, 0)  \\
& \quad \leq 
\frac{(\tilde H_0 -\tilde H_{T+1}) + \frac{T  L_0 \kappa \epsilon^2}{2} + \epsilon \left( H_0 - H_1 + \frac{L_2}{2}D^2\epsilon T \right) }{\epsilon (T+1)} 
%+ \frac{L_1 d \epsilon^2}{2} }{\epsilon T} 
\ee

\end{proof}


\begin{lem}\label{lem:tmbound} 
Assume $m_{t+1} = \beta_2 m_t +  (1- \beta_2)\dd f(x_t)$ 
starting from $m_{-1} = 0$, 
and $\phi$ is convex and $\phi$ is $q$-homogeneous. 
Then
$$
\sum_{t=0}^T \phi(\dd f(x_t)) 
\leq \left(\frac{1+\beta}{1-\beta_2 + \beta}\right)^q \sum_{t=0}^T\left( D_\phi(\tilde m_{t+1}, 0) + \beta D_\phi(m_{t}, 0)\right)
$$
\end{lem} 


\begin{proof}
$$
\tilde m_{t+1} = \beta_2 m_t +  (1-\beta_2) \dd f(x_t) +  \beta \dd f(x_t)
$$

Then we have

$$
\dd f(x_t) = \frac{\tilde m_{t+1} - \beta m_t}{1-\beta_2 + \beta}
$$

and 
\bb
\phi(\dd f(x_t)) &= \phi\left(\frac{\tilde m_{t+1} - \beta m_t}{1-\beta_2 + \beta}\right) \\
& = \left(\frac{1+\beta}{1-\beta_2 + \beta}\right)^q \phi\left(\frac{\tilde m_{t+1} + \beta (-m_t)}{1+\beta}\right) \\
&\leq \left(\frac{1+\beta}{1-\beta_2 + \beta}\right)^q \left(\phi(\tilde m_{t+1}) + \beta \phi(m_t)\right)
\ee
Summing over $t$:
\bb
\sum_{t=0}^T\phi(\dd f(x_t))
&\leq \left(\frac{1+\beta}{1-\beta_2 + \beta}\right)^q \sum_{t=0}^T\left(\phi(\tilde m_{t+1}) + \beta \phi(m_t)\right) \\
&\leq \left(\frac{1+\beta}{1-\beta_2 + \beta}\right)^q \sum_{t=0}^T\left( D_\phi(\tilde m_{t+1}, 0) + \beta D_\phi(m_{t}, 0)\right)
\ee

\end{proof} 




\begin{lem}\label{lem:tmbound2} 
Assume $m_{t+1} = \beta_2 m_t +  (1- \beta_2)\dd f(x_t)$ 
starting from $m_{-1} = 0$, 
and $\phi$ is convex and $\phi$ is $q$-homogeneous. 
Then
\bb 
\sum_{t=1}^T \phi(\dd f(x_t))
&\leq  T \phi(\dd f(x_0)) + (1- \beta_2 + \beta)^q \left(1 - \frac{(1- \beta_2 + \beta)^q}{(\beta\beta_2)^q}\right) \sum_{t=1}^T (T-t) D_{\phi}\left(\tilde m_{t +1}, 0\right)
\ee
\end{lem} 



\begin{proof}


We have $m_{t+1} = \beta_2 m_t + (1- \beta_2) \dd f(x_t)$, $\tilde m_{t+1} = m_{t+1} + \dd f(x_t)$

Then we have

$$\tilde m_{t+1} = \beta_2 \tilde m_t + (1- \beta_2 + \beta) \dd f(x_t) - \beta \beta_2 \dd f(x_{t-1})$$


Denote $a = (1- \beta_2 + \beta), b = \beta \beta_2$, above becomes: 

$$\tilde m_{t+1} = \beta_2 \tilde m_t + a \dd f(x_t) - b \dd f(x_{t-1})$$

Since $\phi$ is convex and $\phi$ is $q$-homogeneous, we have 

\bb
\phi(\dd f(x_t)) - \phi(\dd f(x_{t-1})) &\leq a^q\left(1 - \frac{a^q}{b^q}\right)   \phi(a\cdot \dd f(x_t) - b \cdot \dd f(x_{t-1})) \\
& \leq a^q \left(1 - \frac{a^q}{b^q}\right)\phi\left ( 
\frac{ \tilde m_{t+1} + \beta_2 (-\tilde m_t)}{1+\beta_2}
\right ) \\
& \leq \frac{a^q}{1 + \beta_2} \left(1 - \frac{a^q}{b^q}\right)(\phi ( \tilde m_{t+1}) + \beta_2 \tilde \phi(m_t)). 
\ee


Summing over $t$: 
\bb 
\sum_{t=1}^T \phi(\dd f(x_t)) - \phi(\dd f(x_{t-1})) &\leq \frac{a^q}{1 + \beta_2} \left(1 - \frac{a^q}{b^q}\right) \left ( \sum_{t=0}^T \phi(\tilde m_{t+1}) + \beta_2  \tilde \sum_{t=0}^{T-1}\phi(\tilde m_{t+1}))  \right ) \\
&\leq a^q \left(1 - \frac{a^q}{b^q}\right) \sum_{t=0}^T \phi(\tilde m_{t+1}) \\
\ee 
Note that 
$$
\sum_{t=1}^T \phi(\dd f(x_t)) - \phi(\dd f(x_{t-1})) = \phi(\dd f(x_T)) - \phi(\dd f(x_0))
$$

Summing over $t$ again:
\bb 
\sum_{t=1}^T \phi(\dd f(x_t))
&\leq  T \phi(\dd f(x_0)) + a^q \left(1 - \frac{a^q}{b^q}\right) \sum_{t=1}^T (T-t) D_{\phi}\left(\tilde m_{t +1}, 0\right)
\ee 

\end{proof}




{\color{blue} \rule{\linewidth}{0.2mm}
\subsection{Stochastic Version of Proof}\label{thm:stochatic}
The following is adopted on "Momentum Ensures Convergence" paper:

We use the notions $g_t : = \dd f(x_t;\xi_t)$, and $\epsilon_t:= v_t - \dd f(x_t)$, and $\delta_t := g_t - \dd f(x_t)$, and $s_t = \dd f(x_{t-1}) - \dd f(x_t)$

Therefore,

\bb
\epsilon_t &= v_t - \dd f(x_t)\\
&= \beta m_t +(1-\beta) g_t - \dd f(x_t)\\
&= \beta (m_t - \dd f(x_t)) + (1-\beta) (g_t - \dd f(x_t)) \\
&= \beta_2 \epsilon_{t-1} + \beta \beta_2 \left( \dd f(x_{t-1}) - \dd f(x_t)\right) + (1-\beta + \beta (1-\beta_2))\delta_t
\ee
That is
$$
\epsilon_t =\beta_2 \epsilon_{t-1} + \beta \beta_2 s_t + (1-\beta + \beta (1-\beta_2))\delta_t
$$

Note that the smoothness of the gradient implies: 
$$
\|s_t \| = \|\dd f(x_{t-1} -\dd f(x_t)\| 
$$

Under a stronger assumption:
\begin{align}
    \|s_t \| = \|\dd f(x_{t-1} -\dd f(x_t)\| \leq L\|x_{t-1} - x_t\| \leq L \sqrt{d} \gamma \label{equ: strong}
\end{align}

,where $\gamma $ is the step size.

Under a weaker assumption: 

\begin{align}
    \|s_t \| = \|\dd f(x_{t-1} -\dd f(x_t)\| \leq L\|x_{t-1} - x_t\| \leq \gamma 
(L_0 + L_1 \phi(\dd f(\blue{x_{t}})))
\norm{\dd\phi(\tm_{t})}_2\label{equ:weak}
\end{align}


,where $\gamma $ is the step size.

Using mathematical induction, we have

\begin{align}
    \epsilon_t =\beta_2^t \epsilon_{0} + \beta \beta_2 \sum_{i=1}^t \beta_2^{t-i} s_i + (1-\beta \beta_2) \sum_{i=1}^t \beta_2^{t-i} \delta_t \label{equ: error}
\end{align}



By taking the norms of both sides of the above equation and using the strong bound \ref{equ: strong} we obtain

\bb
\|\epsilon\| \leq \beta_2^t \|\epsilon_0\|+ L\sqrt{d}\gamma \beta \beta_2 \sum_{i=1}^t \beta_2^{t-i} + (1-\beta \beta_2) \|\sum_{i=1}^t \beta_2^{t-i} \delta_t\| 
\ee
Taking expectations on both sides,

\bb
\E \|\epsilon\| \leq \beta_2^t \|\epsilon_0\|+  \frac{L\sqrt{d}\gamma \beta \beta_2}{1-\beta_2} + (1-\beta \beta_2) \|\sum_{i=1}^t \beta_2^{t-i} \delta_t\| 
\ee

Note that r.v.s $(\delta_i)_{1\leq i \leq t}$ are independent and mean zero, we have

\bb
\E \left\|\sum_{i=1}^t \beta_2^{t-i} \delta_t\right\| \leq \sqrt{\E \left\|\sum_{i=1}^t \beta_2^{t-i} \delta_t\right\|^2 } \leq \sqrt{\E \sum_{i=1}^t \beta_2^{2t-2i} \left\|\delta_t\right\|^2 }\leq \frac{\sigma}{\sqrt{1-\beta_2^2}}
\ee

Hence,
\bb
\E \|\epsilon\| \leq \beta_2^t \|\epsilon_0\|+  \frac{L\sqrt{d}\gamma\beta \beta_2}{1-\beta_2} + (1-\beta \beta_2) \frac{\sigma}{\sqrt{1-\beta_2^2}}
\ee

% Now let us do a weaker version: 


\color{blue} \rule{\linewidth}{0.2mm}}

==> old_content/experiments.tex <==
\section{Experiments}\label{sec:exp}
This section begins with a summary of experiments we conduct and their purpose. Then, we provide the details of the experimental setup. In the end, we present the experiment findings and the corresponding analysis.

\paragraph{Experiment Summary:}In this section, we have explored various extensions and improvements to the Lion optimization algorithm. The studies have been conducted in three main areas:

1) \textbf{Choice of $\phi$:} We investigated the potential of replacing $\norm{x}_1$ with different types of norms, both in terms of grouped module parameters. We found that using norms beyond L1, such as $L_p$ with $p=2$, leads to different performances in LLM and vision tasks. 

2) \textbf{Grouping effect:} The grouping effect, where parameters are partitioned into natural groups, offers further potential benefits in addressing issues like varying gradient magnitudes. We tested model-wised (all parameters of the neural networks normalized together), module-wised (parameters at the same module normalized together), and individual-wise (normalize single parameter, which is equivalent to SIGN operation).

3) \textbf{Distributed Lion:} We proposed a simple distributed variant of Lion that only needs to communicate the binarized momentum, resulting in high communication efficiency. In our experiments, the distributed Lion saved significant communication cost while achieving nearly the same performance as the original version. It offers a powerful solution for parallel and distributed training.

These studies reinforce the flexibility and adaptability of the Lion optimization algorithm, showcasing its potential for further fine-tuning and application across diverse deep learning tasks and architectures.

\paragraph{Experimental Setup:} The experiments in above are conducted on both vision and language problems. For the vision task, we apply the optimizer of interest on ResNet-50~\citep{he2016deep} for ImageNet training \cite{}. Without specification, we train ResNet-50 for \bo{how many} steps on ImageNet following the PyTorch official example, which uses \bo{what} data augmentation. We search for the best learning rate from $\{5e-5, 1e-4, 2e-4\}$. For the language problem, we consider language modeling with the GPT-2 model~\cite{}. \bo{@kaizhao, maybe you can help filling in this section?}

%  We make the following studies: 
% %Based on our framework, we propose 

% 1) The choice of $\phi$. We study the potential of replacing $\norm{x}_1$ with other types of norms. One candidate we considered is $$
% \norm{x}_{\mathcal G, p, 1} = \sum_{i} \norm{x_{\mathcal G_i}}_p
% $$ 
% where $x = \{ x_{\mathcal G_i}\colon i \}$, and $\mathcal G_i$ is the $i$-th module in the neural network. 
% $$
% \dd_{x_{\mathcal G_i}} \phi(x) = 
% \left (\frac{x_{\mathcal G_i}}{\norm{x_{{\mathcal G_i}}}_p}  \right )^{p-1}. 
% $$
% It reduces to L1 when each element is a group, but we find that it may be beneficial to apply the normalization in a group. 

% 2) By introducing a weight coefficient to adjust the importance weights between the Hamiltonian and mirror descent components, we arrive an update of form
% $$
% x_{t+1} = x_t - \gamma\left [ (1+u)\sign(\beta_1 m_t + (1-\beta_1) \dd f(x_t) ) -  u \sign(m_t) \right ] .
% $$
% We find that $u = 1$ works well....

% 3) We derive a simple distributed variant of Lion that only need to communicate the binarized momentum and hence enjoys high communication efficiency. 
% In a CIFAR experiment, we show that 
% we save xx\% percentage communicate cost 
% while with negligible drop on performance. 



%\subsection{Studying the choice of $\phi$ }

%\subsection{General Convex Functions}

%Consider one 1D for now: 

%1) $\phi(x) = \max_i (a_i x + b_i)$. Can approximate any convex function when there are sufficient $i$. 

%2) $\phi(x) = \sum_i \max(0, a_i x + b_i)$. 



%3) A more general form  going beyond 1D:
%$$\phi(x) =  v\left (  \frac{1}{d}\sum_{i=1}^d u(\abs{x_i}) \right ), $$
%where $u$ and $v$ are monotonic and convex functions on $\RR$. 

% A variant:
% $$
% \phi(x) =  v\left (  \frac{1}{d}\sum_{i=1}^d u(quantile(\abs{x_i})) \right ), 
% $$

\subsection{Smoothing Effect}
Consider the $L_p$ norm: 
\bb 
\phi_p(x) \defeq  \norm{x}_p 
=\left (\frac{1}{d} \sum_{i=1}^d \abs{x_i}^p \right )^{1/p},  && 
\dd \phi_p(x) 
=  \sign(x) 
{d^{1/p}}
\left (  \frac{\abs{x}}{\norm{x}_p} 
\right )^{p-1}. 
\ee 
It reduces to Lion when $p=1$. 
When $p=2$, we have $\dd \phi_p(x) = \frac{x}{\norm{x}_2}$ which normalized gradient by its L2 norm. 

% \begin{wrapfigure}{r}{0.5\textwidth}
%   \begin{center}
%     \includegraphics[width=0.48\textwidth]{figures/train_loss_llm.pdf}
%   \end{center}
%   \caption{Birds}
% \end{wrapfigure}
% \paragraph{Observations}:

% 1. Different $\phi_p$ Choices: Lion, LionL1.5, LionL2, and LionL3 correspond to $p = 1, 1.5, 2, 3$, respectively, in the formulation of the Lion optimization method.

% 2. Monotonicity of $H(x, m)$: The Hamiltonian function $H(x, m)$ exhibits a monotonically decreasing behavior during the optimization process. As the optimization progresses, $H(x, m)$ decreases, reflecting the convergence of the algorithm.

% 3. Sensitivity to Quadratic Objective Functions: When applied to quadratic objective functions, Lion has a tendency to overshoot the optimal solution compared to LionL1.5, LionL2, and LionL3, which exhibit more controlled behaviors in such scenarios.

% 4. Impact of $p$: The parameter $p$ is in the positive real number domain ($p \in \mathbb{R}^+$). The choice of $p$ significantly influences the trajectory of the optimization process. Different $p$ values lead to distinct optimization paths, resulting in variations in convergence speed and final solution quality.
\iffalse 
\begin{figure}[h!]
    % \centering
    \includegraphics[width=0.5\textwidth]
    {figures/imgnet_loss_pow1.pdf}
    \includegraphics[width=0.5\textwidth]
    {figures/train_loss_llm.pdf}
    \caption{
    (Left) Training loss of ImageNet using of different $\ell_p$ norms. (Right) Training loss of GPT-2 using of different $\ell_p$ norms.}
    \label{fig:pow}
\end{figure}
\fi 




% \red{\textbf{Question:}} How does $p$ influence the result?

% \blue{\textbf{Lizhang}: Let me quickly loop a range of p. 
% Also, is $\dd \phi_p (x)$ an element-wise operation or module wise? }
% \qq{Yes.}
% \qq{I feel for these it might be more illustrative to show some phoneme in toy.}
% \qq{Another different smoothing effect is to remove the non-smoothness at the zero point -- note that the norms above are all non-smooth at the zero point.
% Smoothed surrogates of $\sign$ can be $x/ (|x| + e)$, or $clip(x, -e, e)/e$)
% }

% \blue{\textbf{Lizhang}: In smoothing effect section, should we use relativistic kinetic energy, which is more consistent with our implementations in practice? Or we can briefly mention that in practice, we already add an epsilon in the denominator and it corresponds to the 1 term after scaling.}

\subsection{Grouping Effect}



In neural networks, the paramters are typically naturally partitioned into different groups, $x = [x_{\mathcal G_i} ]_i$, where
$\mathcal G_i$ denotes indices of the parameters in the $i$-th group. 
We consider the grouped $L_{p,1}$ norm: 
\bb  
\norm{x}_{\mathcal G, p, 1} = \sum_{i} \norm{x_{\mathcal G_i}}_p, 
&&
\dd_{x_{\mathcal G_i}} \phi(x) = 
\sign(x) \left (\frac{\abs{x_{\mathcal G_i}}}{\norm{x_{{\mathcal G_i}}}_p}  \right )^{p-1}. 
\ee 
Lion corresponds to the case when each parameter dimension forms its own individual group. 
%\iffalse 
\begin{figure}[h!]
    % \centering
    \includegraphics[width=0.5\textwidth]
    {figures/imgnet_loss_module.pdf}
    \includegraphics[width=0.5\textwidth]{figures/llm_module.pdf}
    \caption{(Left)Training loss of ImageNet using model wise Lion-$\ell_2$ (in red) and module wise Lion-$\ell_2$ (in blue) methods. (Right) Training loss of GPT-2 using model wise Lion-$\ell_2$ (in red) and module wise Lion-$\ell_2$ (in blue) methods.
    }
    \label{fig:group}
\end{figure}
%\fi 
% \red{\textbf{Question:}} Does the grouping mechanism help?  

\paragraph{Advantages of Grouping:} Grouping the parameters can provide several advantages in the optimization process. 
The standard SGD uses the same learning rate for all layers.
The gradients of the linear layer are not on the same scale as those of other layers. Additionally, certain layers have very small gradient norms, indicating significant variations in the magnitude of gradients across different modules.

Based on this observation, it appears reasonable to consider performing updates module-wise. A potential improvement in the optimizer could involve adopting module-wise learning rates, where each module in the neural network is updated with a learning rate tailored to its specific characteristics. This approach would likely help address the issue of varying gradient magnitudes across different modules and improve the overall optimization process and convergence behavior.

\paragraph{Comparisons to Model-wise and Layer-wise Approaches:} While Lion corresponds to individual-wise treatment, other algorithms have been proposed that utilize adaptive layer-wise scalings in combination with base optimization algorithms\citep{you_large_2020,you_large_2017}. By comparing these approaches, we can understand the benefits and trade-offs of different grouping strategies in the context of optimization for neural networks.

\paragraph{Experiment on ImageNet:} Figure~\ref{fig:pow} illustrates the training loss of ResNet-50~\citep{he2016deep} on ImageNet~\citep{ILSVRC15}
using Lion and Lion-L2, showcasing the impact of the grouping effect on the optimization performance for a large-scale model. Throughout the training process, LionL2 consistently achieves lower training loss and higher top-1 accuracy compared to Lion. This result indicates that LionL2, which corresponds to the choice of $p=2$ in the Lion optimization method, leads to improved convergence and better final performance on the ImageNet dataset for the ResNet-50 model.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=\textwidth]{figures/imgnet_loss_acc.pdf}
%     \caption{Comparison of Training Loss and Top-1 Accuracy for ResNet-50 on ImageNet using Lion and Lion-L2 Optimization Methods. Throughout the training process, LionL2 consistently achieves lower training loss and higher top-1 accuracy compared to Lion. This result indicates that LionL2, which corresponds to the choice of $p=2$ in the Lion optimization method, leads to improved convergence and better final performance on the ImageNet dataset for the ResNet-50 model.
%     \qq{remeber to unify the legends in the last step}
%     }
%     \label{fig:imgnet}
% \end{figure}


\iffalse 
\subsection{Combination weights of Hamiltonian and Mirror Descent Components}
%Introduce 
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/heatmap.pdf}
    \caption{ImageNet accuracy of ResNet-50 trained from scratch after 4K steps of training when we vary lr and $u$ for $\ell_2$ and $\ell_1$: (Left) $\ell_1$ norm based weighted combination of the Hamiltonian and Mirror Descent Components; (Right)$\ell_2$ norm based weighted combination of the Hamiltonian and Mirror Descent Components \bo{we need to emphasize how many steps we train, these are too low}}
    \qq{what is the conclusion here? a curve might be easier to see.}
    \label{fig:heatmap}
\end{figure}
\fi  
% By taking a weighted combination of the Hamiltonian and Mirror Descent Components, we get 
% \bb 
% x_{t+1} & = x_t  - \gamma \left [ u  \dd\phi(m_t + \beta \dd f(x_t)) + (1- u)\dd \phi(m_t) \right ] \\ 
%  m_{t+1}&  =  m_t + \beta (\dd f(x_t) - \red{u} m_t),
% \ee 
% where $u$ can be any positive number. If $u>1$, it corresponds to extrapolating the direction towards the $\phi(m_t + \beta \dd f(x_t)) - \dd \phi(m_t)$ direction.


% \red{we can add $\red{u}$ on the damping term or not. Equivalent but could influence the search space.} 
% \blue{\textbf{Lizhang}: I think we should add $u$ on the damping term here, it looks consistent and straightforward, then illustrate that if $\nabla \phi$ is scale free, then it is equivalent without damping. }


% \red{\textbf{Question}:} Can we search for better $u$ than $u=1$? 

% \blue{\textbf{Lizhang}: $u = 1$ is exactly Lion, based on my experiments on ImgNet and CIFAR-10, $u = 2$ also works well. I think we should add $u$ on the damping term here, make sure it's consistent, then illustrate that if $\nabla \phi$ is scale free, then it is equivalent without damping. }

\subsection{Distributed Lion}
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/test_acc_results1.pdf}
    \includegraphics[width=\textwidth]{figures/train_loss_results1.pdf}
    \caption{Train loss and test acuracy of distributed Lion, global Lion, deep gradient compressing, and signum on CIFAR-10. Number of workers is from 8 to 32 with total batch size from 128 to 4096. 
    % \qq{the figures are too small, we do not need these many plots}
    }
    \label{fig:distribut_}
\end{figure}
We consider a more general Hamiltonian that  introduces $N$  copies momentum vectors: 
$$
H(x, m_1\ldots m_k) 
= f(x) + \sum_{i=1}^k 
\phi_i(m_i), 
$$
where $m_i \in \RR^d$, and 
each $\phi_i\colon \RR^d \to \RR^d$ is  a convex function. 


We introduce $N$ copies of momentums that are averaged: 

\bb
x_{t+1} & = x_t + \epsilon \frac{1}{N} \sum_i u_{t,i} \ant{workers only need to pass binary $u_{t,i}$ to center} \\
m_{t+1,i} & = \beta_{2,i} m_{t,i} + (1-\beta_{2,i} )\dd f(x_t)  \ant{parallel on $i$th worker with sgd} \\
u_{t+1,i} & = \phi'_i(\beta_{1,i} m_{t,i} + (1-\beta_{1,i}) \dd f(x_t)) \ant{parallel on $i$th worker with sgd}
\ee

\paragraph{Mixture of Lions} When using different $\phi'_i $ and $\beta_{1,i}$, $\beta_{2, i}$, this is an ensemble of lion. We  can see if we can search a good algorithm. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\textwidth]{figures/test_acc_distributed.pdf}
%     \includegraphics[width=\textwidth]{figures/train_loss_distributed.pdf}
%     \caption{Train loss and test acuracy of distributed Lion, global Lion, deep gradient compressing, and signum on CIFAR-10. Number of workers is from 1 to 32 with total batch size from 128 to 4096. 
%     \qq{the figures are too small, we do not need these many plots.}}
%     \label{fig:distribut}
% \end{figure}




\paragraph{Communication efficiency} Even if all $\phi$ and $\beta$ are the same, when the gradient $\dd f(x)$ are evaluated with different data from different workers, the $m_i, u_i$ would be different. And when $\phi$ is the sign function, we only need to pass the binary vector $u_i$ for high communication efficiency. 

A simple and quick experiment: compare this with the standard Lion with $\sign(\sum m_i)$ (other than $\sum_i u_i$) which need to pass $m_i$ rather than $u_i$. Hopefully the performance drop is not significant when the batchsize of each individual worker is large, so that the variance between different workers are not large. 


==> old_content/intro.tex <==
\section{Introduction}
\label{sec:intro}
Training large-scale deep foundation models, 
such as large language models (LLM)~\citep{OpenAI2023GPT4TR} and large vision models (LVM)~\citep{kirillov2023segment}, 
forms the cornerstone of modern artificial intelligence systems. 
As the time, financial, and environmental costs of training large AI systems continue to rise, identifying the most efficient optimizer becomes critically important.

Traditionally, machine learning experts have devised optimizers based on theoretical insights. 
\adam{}~\citep{kingma2014adam} (or its variant \adamw{}~\citep{loshchilov2017decoupled}), remains to be the most widely employed method in deep learning. 
%
Recently, however, a new optimization called 
\lion{} (evolved sign momentum)~\citep{chen2023symbolic}  has been shown to gain performance surpassing that of Adam in a wide range of tasks while reducing the memory cost and training time. 
What sets \lion{} apart from conventional optimizers is that it was founded through an evolutionary program employing symbolic search. Hence, despite the good practical performance, there exists no a priori theoretical guarantee that LION will serve as a reliable and valid general-purpose algorithm for general optimization problems. 
However, intriguingly, \lion{},
 with a simple and elegant form, 
consistently excels across diverse domains, enveloping an unsolved mystery surrounding its remarkable adaptability.

This work aims to draw a principled understanding of the dynamical behaviors of \lion{}, through the lens of Hamiltonian dynamics. % in the continuous-time limit. 
In particular, we identify a Hamiltonian function, 
for which Lion can be viewed as a Hamiltonian mirror descent algorithm,
consisting of the conservative (Hamiltonian) component that leaves the Hamiltonian function invariant, 
and a mirror descent (dissipative) component that monotonically decreases the Hamiltonian function to enable optimization.  
This framework lays a theoretical
foundation for understanding, improving, and extending \lion{}. 
In this work, 
we exemplify the power of the framework 
by 
%In particular, we leverage our framework to 
(1) providing convergence analysis of \lion{} 
in both continuous-time and discrete-time settings, 
and (2)
exploring various extensions of \lion{}, 
including a broad \lion{}-$\phi$ family, 
and a distributed version of Lion that enjoys low communication cost 
while gaining good performance. 

%theoretical understanding and algorithmic extensions and improvement of \lion{}. 

%We show \red{....}

% keen understanding
% serve as a springboard for future researchers, not only offering a detailed understanding of LION's functionality but also providing fresh insights into the broader landscape of optimizer design for deep learning. 
% Lion corres
% Through a dynamical systems view. 
%We show that 
%Our work seeks to demystify the underlying mechanisms behind its exceptional performance by conducting a surprising revelation - LION lends itself to a straightforward yet elegant analysis, which hitherto remained concealed from scrutiny.Through rigorous investigation and extensive empirical studies, we shed light on the inner workings of LION, unveiling the profound reasons behind its dominance. By doing so, we bridge the gap between the empirical success of LION and its theoretical foundation, cementing its status as a trans formative optimizer for efficient deep learning.

%The groundbreaking revelations within this paper promise to propel the field towards more efficient, powerful, and widely applicable optimizers, cementing LION's place as an influential and award-winning breakthrough in the realm of deep learning optimization.


\paragraph{Overview} 
Let $f\colon \RR^d\to \RR$ be a differentiable cost function that we want to minimize. 
Despite being discovered via evolutionary search,  
\lion{} yields a simple and elegant form: 
\bbb \label{equ:lionalg} 
\begin{split} 
\vv m_{t+1} &  =  \beta_2\vv m_t + (1-\beta_2) \dd f(\vv x_t) \\ 
\vv x_{t+1} 
& = \vv x_t - 
\gamma ~ \sign( 
\beta_1 \vv m_t + (1-\beta_1) \dd f(\vv x_t)
), 
\end{split} 
\eee 
where $m_t$ is a momentum variable,  
$\gamma$ is the step size,  
$\beta_1,\beta_2 \in[0,1]$ are hyperparameters, and $\sign(\cdot)$ denotes the sign function, with  $\sign(0) = 0$ and $\sign(x)=x/\abs{x}$ for $x\neq 0$.
The update of $m_t$ is a standard momentum accumulation that estimates the exponential moving average of the gradient as classical momentum algorithms, 
but the update 
$x_{t}$ sets it apart from a standard existing method 
due to the use of $\sign(\cdot)$ and the convex combination of gradient and momentum. 
See Section~\ref{sec:lion} 
for more discussion.

%With the default parameter $\beta_2 = 0.99$ and $\beta_2 = 0.9$ recommend in \eqref{equ:lionalg}, the \lion{} update is  
%\bb \vv x_{t+1} \gets \vv x_t + \gamma \times \sign\left ( \med{\vv g_{t}} + \blue{0.09  \vv g_{t-1} + 0.089\vv g_{t-2} + 0.088 \vv g_{t-3} +  0.087 \vv g_{t-4} + \cdots } \right ).\ee 
%\bb \vv x_{t+1} \gets \vv x_t + \gamma \times \sign\left ( \med{0.99\vv g_{t}} + \left(\blue{0.091 \vv g_{t}  + 0.090  \vv g_{t-1} + 0.089\vv g_{t-2} + 0.088 \vv g_{t-3}  + \cdots }\right) \right ).\ee 


We propose to study Lion through 
the following ordinary differential equation (ODE):  
%continuous time limit of Lion:
\bbb \label{equ:lionode}
\text{\lion{}-$\phi$ ODE:}~~~~~~~~
\begin{split} 
\ddt m_t & =  \alpha \dd f(x_t) - \eta m_t, \\ 
\ddt x_t 
& =  - \dd\phi(m_t + \beta \dd f(x_t)),  
~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
\end{split} 
\eee  
where $\alpha,\beta, \eta >0$ are parameters and  $\phi\colon \RR^d \to \RR$ 
is a convex function with $0$ as the unique minimum point. 
We show in Section~\ref{sec:lion-discretization}
that \lion{} \eqref{equ:lionalg} corresponds to a time discretization 
of \eqref{equ:lionode} 
when $\phi$ is the $\ell_1$ norm 
with 
with $\phi(m) =  \norm{m}_1$, and $\dd \phi(m) = \sign(m)$.

A key observation is that \eqref{equ:lionode} system yields a Hamiltonian (and Lyapunov) function, 
\bbb  \label{equ:hxm}  
H(x, m) = f(x) + \alpha^{-1} \phi(m), 
\eee  
which decreases monotonically along the trajectories of \eqref{equ:lionode}, that is, 
$\ddt H(x_t, m_t) \leq 0.$
%Therefore
Moreover, the system in \eqref{equ:lionode}  
can be decomposed the sum of two components: 
%a combination of conservative and descending components: 
\bbb \label{equ:decomp}
\ddt 
\begin{bmatrix}
x_t\\
m_t 
\end{bmatrix} = 
\blue{\underbrace{\begin{bmatrix}
-\dd\phi(m_t)\\
\alpha \dd f(x_t) 
\end{bmatrix}}_{\text{Hamiltonian}}}
+ 
\med{\underbrace{\begin{bmatrix}
-\dd\phi(m_t + \beta \dd f(x_t)) +\dd\phi(m_t) \\
\textcolor{brown}{- \eta m_t}
\end{bmatrix}}_{\text{Mirror Descent}}}, 
\eee 
where we have a conservative component, which the standard Hamiltonian system that leaves $H(x_t,m_t)$ invariant, and a descending (or dissipative) component that monotonically decreases $H(x_t, m_t)$
following a special type of mirror descent direction. 
\red{
This provides a clear characterization of the mathematical nature of the Lion dynamics. 
}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{figures/conformal.png}
    \vspace{-2\baselineskip}
    \caption{
    The Hamiltonian component (a),  mirror descent component (b),  and  the overall vector field    (c)  of Lion on 1D loss function $f(x) = x^2$, $x\in\RR^d$. 
    %Vector field of Hamiltonian system, Mirror Descent system, and the combination of those two.
    }
    \label{fig:vector-field}
\end{figure}

The value of this framework is 2-fold: 
\begin{enumerate}
    \item It provides 
a principled way to gain theoretical insights 
underpinning the empirical successes of Lion. The double-$\beta$ scheme is closely related to the Nesterov acceleration. The $\sign(\cdot)$ operator plays the role of mirror descent.
    \item It provides a flexible space of convergent  algorithms in which we can improve and extend \lion{}. For instance, we show that replacing $\sign(\cdot)$ with the derivative of other $\ell_p$-norms ($p \geq 1$) also works in practice. 
\end{enumerate}

The rest of the paper is organized as follows. 


\begin{enumerate}
    \item Section~\ref{sec:lion} - Generalization and Connection to Nesterov Momentum: This section will extend the use of the sign function and explore the link between the Lion algorithm and Nesterov Momentum. It will also examine different discretization schemes within the continuous framework.

\item  Section~\ref{sec:lion_analysis} - Monotonicity Proof: This part will demonstrate the monotonicity of the function \(H(x_t,m_t) = f(x_t) + \frac{1}{\alpha} \phi(m_t)\), following the ODE in equation \eqref{equ:lionode}. It will also prove that this function is a Lyapunov function, indicating stability.

\item Section~\ref{sec:hamiltonian-mirror-descent} - Hamiltonian and Mirror Descent Decomposition: Here, the paper will describe the decomposition of the Lion-$\phi$ ODE into Hamiltonian and mirror descent components. The space of algorithms whose convergence can be verified using a Lyapunov function will be characterized, with Lion-$\phi$ identified as a particular case.

\item  Section~\ref{sec:disc_lion} - Discrete Time Analysis: This section will focus on the discretization of the proposed ODE scheme, providing an analysis in both strong and weak smoothness conditions.

\item  Section~\ref{sec:exp} - Experimental Results: Finally, the paper will present experimental findings in three areas: 1) the selection of the function \(\phi\), 2) the grouping effect, and 3) the distributed implementation of Lion.
\end{enumerate}



==> old_content/method.tex <==

%\section{Lion: %EvoLved Sign Momentum} 
\section{Lion and Lion-$\phi$}
\label{sec:lion}

We provide some general discussion on Lion and Lion-$\phi$,
 comparing and connecting it with the existing optimizing algorithms, including Sign gradient descent, adaptive gradient methods, Hamiltonian descent, 
 and Nesterov momentum. 

\subsection{Lion-$\phi$: Discretization Schemes}
\label{sec:lion-discretization}
The  Lion-$\phi$ ODE in \eqref{equ:lionode}
can be solved using different discretization schemes. 
When $\phi$ is homogeneous as in the case of \lion{},
the different schemes
yield equivalent updates 
when the parameters are adjusted properly. The explicit Euler Discretization of \eqref{equ:lionode} yields 
\bb 
m_{t+1} & = m_t + \gamma  
(\alpha \dd f(x_t) - \eta m_t) \\
x_{t+1} & = x_t - \gamma\dd\phi(m_t + \beta \dd f(x_t)).
\ee 
With $\dd\phi(x) = \sign(x)$ and noting 
$\sign(ax)=\abs{a} \sign(x)$ recovers Lion in \eqref{equ:lionalg} with 
$\beta_1 = 1/(1+\beta)$, 
and $\beta_2 =\gamma \alpha = \gamma \eta.$ 

Because the ODE for updating $m_t$ 
is linear on $m_t$, 
\eqref{equ:lionode} can also be approximated via the following semi-implicit Euler scheme: 
\bbb 
m_{t+1} & = m_t + \gamma  
(\alpha \dd f(x_t) - \eta m_{t+1}) \\ 
x_{t+1} & = x_t - \gamma\dd\phi(m_{t+1} + \beta \dd f(x_t)), 
\label{equ:eulersymp}
\eee
where the updates for both $x_t$ and $m_t$ use the most recent $ m_{t+1}$ rather than $m_t$. 
However, 
when $\phi$ is $q$-homogeneous in that $\phi(ax) = \abs{a}^q\phi(x)$ for $q\in\RR$,    
the explicit and semi-implicit 
schemes can be reduced to each other with proper adjustment of the parameters,
and hence yield the same family of practical algorithms. 
We will use the semi-implicit scheme for theoretical analysis 
as it enjoys some nice properties 
in connection to symplectic integrators for Hamiltonian systems~\citep{ruth1983canonical}. 




With  $\beta_2 = 1/(\gamma \alpha +1)$, $  \alpha = \eta$, $\hat \beta_1 = 1/(1+\beta)$, and $\dd\phi = \sign$ in \eqref{equ:eulersymp}, we get a reform  of the Lion update rule: 
\bbb  
\begin{split}
m_{t+1} & = \beta_2 m_t + (1-\beta_2) m_{t+1} \\
%x_{t+1} & =  x_{t} - \gamma \sign(\hat \beta_1 m_{t+1} + (1-\hat \beta_1) \dd f(x_t)), 
x_{t+1} & =  x_{t} - \gamma \sign( m_{t+1} + (\beta_2 - \beta_1) \dd f(x_t)), 
\end{split} 
\label{equ:lionalg2} 
\eee 
which, compared with \eqref{equ:lionalg}, uses the most recent update $m_{t+1}$ for updating $x_t$, and adjusts the coefficients inside $\sign(\cdot)$ accordingly. 
%It is equivalent to \eqref{equ:lionalg} with $\hat \beta_2 = \beta_1/\beta_2$. 
%However, because $\sign(ax)=\sign(x)$ for $a>0$, \eqref{equ:lionalg2} 
%is equivalent to \eqref{equ:lionalg}  when $\hat \beta_2 = \beta_1/\beta_2$. 
This form makes it clear that we should take $\beta_2 > \beta_1$ to make the gradient term assigned with a positive sign, 
%This suggests that we should have $\beta_2 \geq  \beta_1$  in \eqref{equ:lionalg} to make $\hat \beta_1 \leq 1$, 
which is consistent with the default choice of $\beta_1=0.9$ and $\beta_2 = 0.99$ in 
 \citet{chen2023symbolic}. 



\iffalse 
%To draw an intuitive understanding, 
\begin{rem}
For intuition, 
we write down the explicit $x_t$ update of \lion{}~\eqref{equ:lionalg} (with $ \vv g_t = \dd f(\vv x_t)$):  
%\bb \vv x_{t+1} \gets\vv x_t + \gamma \times \sign\bigg((1-\beta_1) \vv g_{t} + \beta_1 (1-\beta_2) \left (\vv g_{t-1}  + \beta_2 \vv g_{t-2} + \cdots +  \beta_2^{t-1} \vv g_0  + \beta_2^t \vv m_0\right)\bigg), \ee 
\bb 
\vv x_{t+1} \gets\vv x_t 
+ \gamma \times 
\sign\bigg(
\med{(1- \hat \beta_1) \vv g_{t} }
%- \frac{\beta_1}{\beta_2} 
%(1-\beta_2) g_t  
+ 
%\frac{\beta_1}{\beta_2}
\med{\hat \beta_1} 
\blue{ (1-\beta_2) 
\left (
 g_{t} + 
\beta_2 \vv g_{t-1}  + \beta_2^2 \vv g_{t-2} + \cdots +  \beta_2^{t} \vv g_0  + \beta_2^{t+1} \vv m_0\right)}\bigg), 
%&&&
\ee 
where $\hat \beta_1 = \beta_1/\beta_2$. 
It combines the current gradient $g_t$ and a exponential moving average of past gradients accumulated by the momentum update. 
Note that the weight of the current gradient is enhanced when 
 $\beta_1 < \beta_2$ and hence $\hat \beta_1 <1$; 
 and would be weaknend when $\beta_1 > \beta_2$. 
 %it introduces an extra gradient term in addition to the typical momentum (the blue part). 
%By setting $\beta_2 > \beta_1$, the update gives larger weights to the current gradient $\vv g_t$, while still using relatively slow exponential decay on the older gradients. 

With the default parameter $\beta_2 = 0.99$ and $\beta_2 = 0.9$ recommend in \eqref{equ:lionalg}, the \lion{} update is  
%\bb \vv x_{t+1} \gets \vv x_t + \gamma \times \sign\left ( \med{\vv g_{t}} + \blue{0.09  \vv g_{t-1} + 0.089\vv g_{t-2} + 0.088 \vv g_{t-3} +  0.087 \vv g_{t-4} + \cdots } \right ).\ee 
\bb 
\vv x_{t+1} \gets \vv x_t + 
\gamma \times \sign\left ( \med{0.99\vv g_{t}} + 
\left(\blue{
0.091 \vv g_{t}  + 
0.090  \vv g_{t-1} + 0.089\vv g_{t-2} + 0.088 \vv g_{t-3}  + \cdots }\right) \right ).
\ee 
\end{rem} 
\fi 

%\paragraph{SignGD, Signum, Adam}
\subsection{On the Use of $\sign(\cdot)$ and $\phi$} 
The use of the sign function in \lion{} is closely related to 
the Sign gradient descent (SignGD) and Signed momentum (Signum) \citep{bernstein2018signsgd}:
\begin{align*}
\text{SignGD:} ~~~~~
\vv x_{t+1} = \vv x_t - \epsilon ~\sign(\dd f(\vv x_t)),  
&&&&&&&&& \text{Signum:} ~~~~~ \vv x_{t+1} =\vv  x_t - \gamma ~\sign(\vv m_{t}), 
\end{align*}
which can be viewed as the 
extreme cases of Lion
when $\beta_1 = 0$ and $1$, respectively. 
%Hence, Lion can be viewed as a 
With $\beta_1 \in (0,1)$, 
Lion can be viewed as interpolating between SignGD and Signum. 
Importantly, 
the interpolation here is nonlinear because the convex combination $\beta_1 m_t + (1-\beta_1)\dd f(x_t)$ is applied 
\emph{inside} the sign function. 
In comparison, the more straightforward linear combination would yield 
\bbb  \label{equ:linearlion}
x_{t+1} = x_t + \gamma  \left ( 
\beta_1 \sign(m_t) + 
(1-\beta_1) \sign(\dd f(x_t)) \right ). 
\eee  
%\vspace{-1\baselineskip}
\setlength{\intextsep}{6pt} % Vertical space around wrapped figure
\begin{wrapfigure}{r}{0.3\textwidth}
  \centering
  \includegraphics[width=0.28\textwidth]{figures/imgnet_loss_linearlion}
  \vspace{-1\baselineskip}
  \caption{Lion and the Linear-Lion in Eq~\eqref{equ:linearlion} on ImageNet with ResNet-50.}
  \label{fig:linearlion}
\end{wrapfigure}
%\vspace{-2\baselineskip}
This algorithm, however,
as shown in figure~\ref{fig:linearlion}, does not perform as well as Lion in practice, and 
is not what was found by the evolved search of \citet{chen_symbolic_2023}.


%The use of sign is mainly motivated to yield
%Sign gradient-based methods have attracted 
%a considerable body of literature due to its simpliflow communicate cost for distributed 

Besides its simplicity and 
low communication cost that makes it attractive to distributed learning, 
sign gradient-based methods have been shown to be beneficial 
for optimization performance in deep learning, 
as the sign function $\sign(x) = x/\abs{x}$ provides 
a coordinated-wise gradient normalization mechanism, similar to adaptive gradient methods such as Adam \citep{kingma2017adam} and RMSprop \citep{tieleman2012lecture}. 
In fact, Adam is reduced to signGD if its momentum accumulation is turned off.  
A number of works have argued that 
the sign descent-like behavior 
stands as the main factor behind the gap between
SGD and Adam \citep[e.g.,][]{balles2018dissecting, 
kunstner2023noise}.
%Dozat2016IncorporatingNM
%,zhang_adam_2023}. 
%^kingma2014adam}.
Along a similar direction, 
signGD can be generalized to 
normalized gradient methods  
in which the gradient (or momentum direction)
is normalized by its norm, 
which is shown to accelerate the escaping 
of flat regions where unnormalized gradient methods tend to get stuck~\citep[e.g.,][]{ 
levy2016power, 
murray2019revisiting}.

% \red{merge the related work section here.}
\input{content/related}
%during optimization
%\bb
%m_{t+1} = \beta_1 m_t + (1-\beta_1) m_t, &&
%v_{t+1} = \beta^{\text{adam}}_2 \dd f(x_t)^2 + (1-\beta^{\text{adam}}_2) v_t ,  && 
%x_{t+1} = x_t + \gamma \frac{m_{t+1}/(1-\beta_1^{t+1})}{\sqrt{v_{t+1}/(1-(\beta_2^{\text{adam}})^{t+1}} + e}.   
%\ee 
%It reduces to signGD when $\beta_1 = \beta_2^{\text{adam}} = 0$.  
%Also related to normalized gradient. 

%Among previous works, 
%More generally, 
%\paragraph{Hamiltonian Descent} 
%The use of a general function $\phi$ within momentum methods
In terms of exploiting a general $\phi$ function in momentum algorithms, 
the Lion-$\phi$ ODE in \eqref{equ:lionode} 
is closely related to the conformal Hamiltonian system~\citep{mclachlan2001conformal} 
employed by the Hamiltonian descent method of \citet{maddison2018hamiltonian}: 
\bbb
\ddt m_t  = \alpha \dd f(x_t)  - \eta m_t,  
&&&
\ddt  x_t   = - \dd\phi(m_t), 
\label{equ:ch}
\eee 
which uses a general convex function $\phi$
like \eqref{equ:lionode}, but sets  $\beta=0$.  
This yields an dissipative Hamiltonian system of $H(x,m)$ 
in \eqref{equ:hxm} 
with a damping force $(-\eta m_t)$ applied on $\phi(m_t)$. In comparison, 
by introducing an extra gradient term inside $\phi(\cdot)$,  
Lion-$\phi$ provides an extra damping on $f(x_t)$ with a special mirror descent direction, 
which also 
yields connection to Nesterov momentum 
 shown in Section~\ref{sec:nesterov}. 
\red{This includes Relativistic gradient descent \citet{francca2020conformal} which uses $\phi(x) = \sqrt{\norm{x}_2^2 + \varepsilon}$. ref this in the figure.} 

%As we show in sequel, introducing the gradient term $\beta\dd f(x_t)$into $\dd\phi(m_t + \beta \dd f(x_t))$ yields connection to Nesterov momentum (Section~\ref{sec:nesterov}), 
%and provides an extra descent on $f$ is equivalent to  conducting a special type of mirror descent to provide extra descent on $f$ beyond the conformal Hamiltonian system in \eqref{equ:ch}.

\paragraph{Examples of $\phi$}
Beyond the $\ell_1$ norm, 
a canonical family of $\phi$ is power of $\ell_p$ norms: 
%Consider the $L_p$ norm: 
\bb 
\phi_{p,q}(x) \defeq  \norm{x}_p^q 
=\left ( \sum_{i=1}^d \abs{x_i}^p \right )^{q/p},  && 
\dd \phi_{p,q}(x) 
=  q % d^{q/p} 
\norm{x}_p^{q-1}
%\sign(x)
%\left (  \frac{{x}^{p-1}}{\norm{x}^{p-1}_p} \right )^{p-1},
\left (  \frac{[ x]^{p-1}}{\norm{x}^{p-1}_p} \right ),
%\sign(x) \left (  \frac{\abs{x}}{\norm{x}_p} \right )^{p-1},
\ee
which is convex when $p,q \geq 1$; 
we write $[x]^{p-1} = \sign(x) \abs{x}^{p-1}$. 
%Moreover, 
%Along another dimension, 

In neural networks, the parameters 
are naturally partitioned into different groups 
(layers or modules), 
whose magnitude may differ significantly.  
%which may deserve different treatment. 
%whose magnitude may vary dramatically. 
We may want to normalize them separately, with a group $\ell_p$ norm: 
%This can be addressed by taking $\phi$ to be a group norm, e.g., 
\bb 
\phi(x) \defeq \norm{x}_{\mathcal G, p} = \sum_{i} \norm{x_{\mathcal G_i}}_p,  && 
\dd_{x_{\mathcal G_i}} \phi(x) = 
%\left (
\frac{ [ x_{\mathcal G_i}]^{p-1}}{\norm{x_{{\mathcal G_i}}}_p^{p-1}}  . %\right )^{p-1}. 
\ee 
where $x = \{ x_{\mathcal G_i}\colon i \}$, and $\mathcal G_i$ is the $i$-th module in the neural network.  It reduces to L1 when each element is a group, but we find that it may be beneficial to apply the normalization in a group. 


%^ which is convex when $p,q \geq 1$. 
%It reduces to Lion when $p=1$. 
%Of special 

Here $p$ and $q$ plays different roles, 
$p$ controls how much we want to \emph{reshape} the direction with power $p-1$, 
while $q$ controls how much 
we want to \emph{normalize} the update 
magnitude. % into account
When $q=1$,
the update is \emph{fully} 
normalized by the $\ell_p$ norm. 
When $p=q=2$, on the other hand, 
we have $\dd\phi(x) = x$, 
which does not apply 
any reshaping or normalization. 
%

\iffalse 
\begin{wrapfigure}{r}{0.52\textwidth}
  \centering
    \includegraphics[width=0.25\textwidth]
    {figures/imgnet_loss_pow1.pdf}
    \includegraphics[width=0.25\textwidth]
    {figures/train_loss_llm.pdf}
    \vspace{-1\baselineskip}
  \caption{
    Training loss of Lion-$\ell_p$ 
    with 
    (Left)  ImageNet using of different $\ell_p$ norms. (Right) Training loss of GPT-2 using of different $\ell_p$ norms.
    \qq{larger legends and fonts, write ImageNet, and GPT-2 inside the figure}
    }
    \label{fig:pow}    
\end{wrapfigure}
\fi 

In practice, we find the fully normalized setting $q=1$ is always favored, 
because 
it helps stabilize the training as the gradient magnitude varies dramatically, and  
avoid slow updates in flat regions ~\citep[e.g.,][]{ 
levy2016power, 
murray2019revisiting}. 
\qq{do we have results?}
In addition, using group norm tends to outperform 
the model-wise norm as shown in Figure~\ref{fig:group}(b)-(a) on ImageNet and  GPT-2. 

On the other hand, 
the use of $\ell_1$ norm ($p=1$) 
as advocated by Lion is not always the best. 
The relative performance of different $\ell_p$ seems to be rather problem dependent. 
Figure~\ref{fig:group}(c)-(d)  
shows that using group $\ell_p$ norm  with 
larger $p$ (e.g., Lion-$\ell_2$ with $p=2$) outperforms 
Lion with $p=1$ on  ImageNet with ResNet,  
but degenerate on GPT-2.  

%nonlinear transform; 
%In particular, when $p=q=2$, we have $\dd\phi(x) = x$, which does not apply nonlinear transform; when $p=2$, $q=1$, we have $\dd \phi_p(x) = \frac{x}{\norm{x}_2}$, which normalizes the gradient by its L2 norm. When In general, when using $q = 1$, we obtain a direction normalized by the $\ell_p$ norm.


\begin{wrapfigure}{r}{.3\textwidth}
    \vspace{-\baselineskip}
    \includegraphics[width=0.3\textwidth]{figures/imgnet_lossl2_eps.pdf}
    \vspace{-\baselineskip}
    \caption{
    Lion-$\phi$ 
    with $\phi(x) = \sqrt{\norm{x}_2^2 + \varepsilon}$ 
    %We use ResNet-50 for ImageNet training, the above are training loss curves of the first 3k iteration steps:
    %(Left) Comparison of the straightforward linear SIGN combination and original Lion. 
    (Middle) Comparison of model-wised Lion-$\ell_2$ and  module-wised Lion-$\ell_2$. 
    (Right) Comparison of module-wised Lion-$\ell_2$ with different $\epsilon$ values.
    }
    \vspace{-\baselineskip}    
    \label{fig:bench}
\end{wrapfigure}

The norm functions (when $q=1$) 
are non-smooth at the zero point. A consequence of this is that the update does not decay to zero 
even when the solution is near optimal. 
This can be fixed by introducing smooth surrogates of $\ell_p$ norms, 
which can help improve the convergence in theory. 
For example, the $\ell_p$ norm 
can be  approximated by $\phi(x) = \sqrt{\norm{x}_p^2 + \varepsilon}$ with small $\epsilon>0$. 
%especially in the later phase to close the optimum point.
%One can further introduce smoothness via $\phi(x) = (\norm{x}_p + \varepsilon)^q$ for some small number $e$. 
%Introducing such $e>0$ makes $\phi$ smooth and 
%can help improve the convergence in theory, especially in the later phase to close the optimum point. 
However,   we did not observe significant difference by introducing $\varepsilon$ on ImaegNet 
as shown in figure~\ref{fig:bench}.

%1) The choice of $\phi$. We study the potential of replacing $\norm{x}_1$ with other types of norms. One candidate we considered is $$



%\begin{rem}
%Our framework suggests that $\phi$ can be taken to be a general convex function. The particular choice of $\phi(x) = \norm{x}_1$ made by \lion{} does not seem to be a universally optimal one, because it is easy to find counterexamples that make it fail. As shown in figure~\ref{fig:quadra}, Lion-$\ell_2$ decreases faster than Lion, while Lion has serrated trajectories with overshooting.

%In fact, due to the binary gradients, after the discretization, \lion{} can converge at best in the range $\gamma$ ball of the optimal solution.Hence, in practice, it is advised to set a small step size for \lion{} (suggested $\gamma=1e-4, 3e-5$ in the \lion{} paper~\citep{chen2023symbolic}), and using decaying learning rates. 
%\end{rem}




%The framework itself does not provide a clear justification on why $\sign$ outperforms the other straightforward choices, such as $\phi(x) = x^2/2$ yielding $\phi(x) = x$. 

%1) $\sign$ is definitely not universally the best choice. A simple counter-example is $f(x) = \norm{x}^2_2$ where gradient descent and momentum goes to the optimal point following a straight trajectory, while signed methods have to follow the zig-zag trajectories. 

%2) Instead, the good performance of $\phi$ on deep neural network models might be similar reason why coordinate-wise adaptive methods like adam work by noting that $\sign(x) = \frac{x}{|x|}$.  It might be a problem dependent choice. Open question and need further studies. 
%gradient and momentum 

%However, our framework suggests that we can potentially test more choices of $\phi$ and hopefully find the best. 
%the best for deep 

\begin{figure}[t]
    % \centering
    \begin{tabular}{cccc} 
        \includegraphics[width=0.25\textwidth]
    {figures/imgnet_loss_module.pdf} & 
    \includegraphics[width=0.25\textwidth]{figures/llm_module.pdf} & 
    \includegraphics[width=0.25\textwidth]
    {figures/imgnet_loss_pow1.pdf} & 
    \includegraphics[width=0.25\textwidth]
    {figures/train_loss_llm.pdf} \\
    \small (a) & \small (b) & \small (c) &\small  (d)
    \end{tabular}
    \caption{
    Training loss on ResNet-50 and GPT-2. 
    (a)-(b): Lion-$\phi$ with $\phi(x) =\norm{x}_2$ (Lion-$\ell_2$ (model)) 
    and the  group $\ell_2$ norm $\phi(x) =\norm{x}_{\mathcal G, 2}$ (Lion-$\ell_2$ (module)).  
    (c)-(d): Lion-$\phi$ 
    with group $\ell_p$ norm $\phi(x) = \norm{x}_{\mathcal G, p}$ with different $p$.  
    %(Left)Training loss of ImageNet using model wise Lion-$\ell_2$ (in red) and module wise Lion-$\ell_2$ (in blue) methods. (Right) Training loss of GPT-2 using model wise Lion-$\ell_2$ (in red) and module wise Lion-$\ell_2$ (in blue) methods.
    }
    \label{fig:group}
\end{figure}


\subsection{Connection to 
Nesterov Momentum}
\label{sec:nesterov} 
When removing the sign operator, 
the \lion{} update in \eqref{equ:lionalg2} 
reduces to
\bbb   
\begin{split} 
m_{t+1} & = \beta_2 m_t + (1-\beta_2)\dd f(x_t), \\ 
x_{t+1} & = x_t - \gamma (\beta_1 m_{t} + (1- \beta_1) \dd f(x_t)). 
\end{split}
\label{equ:lionalg2None}
\eee   
This reduces to the 
classical (Polyak's) momentum when $\beta_1 = \beta_2$. 
When $\beta_1 < \beta_2$, the update places a higher weight on the gradient $\dd f(x_t)$, and hence can be viewed as correcting the behavior of momentum with gradient direction. 
%
In the following, we show that 
this turns out to be equivalent 
to Nesterov momentum,
which suggests a connection between the extra gradient term  with the Nesterov acceleration phenomenon well studied in the optimization literature. 
\newcommand{\epsilontmp}{\gamma} 
\begin{pro}
The update in \eqref{equ:lionalg2None} 
is equivalent to the Nesterov momentum update of the form 
%\bb v_{t+1} & =  \mu v_t- \varepsilon  \dd f(y_t + \nu v_t), \\y_{t+1} & = y_t + v_{t+1}, \ee 
\bb 
m_{t+1} & =  \beta_2 m_t + (1-\beta_2)\dd f(y_t - b \epsilontmp m_t), \\
y_{t+1} & = y_t - \epsilontmp m_{t+1}, 
\ee 
with $x_t = y_t - b \epsilontmp m_t$, 
 $\beta_1 = \beta_2 - (1-\beta_2) b$. 
\end{pro} 
\begin{proof}
Let $x_t = y_t - b \epsilontmp m_t$. Then 
$
m_{t+1} =  \beta_2 m_t +  (1-\beta_2) \dd f(x_t), 
$
and 
\bb 
x_{t+1} 
& =   y_{t+1} - b \epsilontmp m_{t+1} \\ 
& = y_t - (1+b )\epsilontmp m_{t+1}  \\ 
& = x_{t} + b \epsilontmp m_t   - (1+b)\epsilontmp m_{t+1} \\ 
& = x_{t} + b \epsilontmp m_t   - (1+b)\epsilontmp (\beta_2 m_t + (1-\beta_2)\dd f(x_t))\\  
& = x_{t} 
- \epsilontmp 
[ ((1+b) \beta_2  - b) m_t 
+ (1+b) (1-\beta_2) \dd f(x_t) ] \\ 
& = x_{t} 
- \epsilontmp 
[\beta_1 m_t 
+ (1-\beta_1)\dd f(x_t) ], 
\ee 
where the last equality comes from noting that  $ \beta_1 = (1+b) \beta_2  - b$ and $ (1+b) (1-\beta_2) = 1-\beta_1$. 
\end{proof}
\paragraph{Remark}
Unlike the case of \lion{}, the popular implementations of Nesterov momentum are typically parameterized by a single parameter $\beta_2$, while with $b$ fixed, and hence does not fully exploit the full algorithm space. 
% 
For example, the form in Geoffrey Hinton's paper~\citep{sutskever2013importance} (in their Eq.(3, 4)), which is widely referenced in deep learning implementation, is equivalent to taking $b = \beta_2$, which yields $\beta_1 = \beta_2^2$. Taking $\beta_2 = 0.99$ as an example, we would have $b = 0.99$ and  $\beta_2^2 = 0.98\approx \beta_2$, making \eqref{equ:lionalg2None} behave almost the same as the classical momentum. On the other hand, with the default $\beta_1 = 0.9$ and $\beta_2 = 0.99$ in Lion, we need to take $b = 9$, which is much large.
% 
The power of Nesterov momentum may have not been fully exploited for this insufficient search of hyperparameters. 
%With the default $\beta_1=0.9$ and $\beta_2 = 0.99$ in Lion, we have $b = 0.09/(0.01) = 9$. \red{In Pytorch implementation, however, is equivalent to taking $b = 1/(1-\beta_2)$, which would yield $\beta_1 = \beta_2 - 1 <0$?} 

%\subsection{Convex Functions} 


\paragraph{Remark}
 The connection with Nesterov momentum can also be seen through the ODEs.  
 Eliminating $m_t$ in the Lion-$\phi$ ODE \eqref{equ:lionode} yields 
 $$
 \dd^2 \phi^*(-\dot x_t) \ddot x_t 
 + \beta \dd^2 f(x_t) \dot x_t 
 - \eta \dd\phi^*(- \dot x_t) 
 + (\alpha + \eta \beta) \dd f(x_t) = 0.
 $$
 When $\phi(x) = x^2/2$, it yields 
\bbb 
\label{equ:hode}
\ddot x_t + 
\beta \dd^2f(x_t) \dot x_t  + 
\eta \dot x_t + (\alpha + \eta \beta) \dd f(x_t) = 0, \eee
which coincides with the 
\emph{high-resolution} ODE 
 of \citet{shi2021understanding} for modeling  
 %the behavior of  
 Nesterov momentum. 
 The key feature of \eqref{equ:hode} 
 is the Hessian-dependent damping term $\dd^2 f(x_t) \dot x_t$, arising from the gradient correction term in Lion-$\phi$, which is key to the accelerating analysis 
 of Nesterov momentum \citep{shi2021understanding}. 
 
 % for strongly convex functions.  
 %was characterized by a \emph{high-resolution} ODE: 
 %$$\ddot x_t  + a \dot x_t + b \dd ^2 f(x_t) \dot x_t + b \dd f(x) =0.$$

%\paragraph{Remark}
There has been a line of works on 
developing  accelerated mirror descent extensions of Nesterov accelerated gradient \citep[e.g.,][]{krichene2015accelerated, diakonikolas2021generalized}. The ODEs systems are different from Lion-$\phi$.   \red{...}


%\subsection{Choices of $\phi$}
%\red{todo}
 
\section{Analysis of Lion-$\phi$: Continuous Time} \label{sec:lion_analysis}
%We study Lion from an ODE perspective, and find a Lyapunov function that secure its asymptotic convergence. 
%Let $H(x, m ) = f(x) + \phi(m)$, where $\phi$ is any (sub-)differentiable convex function.  For example, $\phi(m) = \norm{m}_p$ is the case of Lion ($p=1$) and LionL2 ($p=2$); it can be group norm which would correspond to Lion module wise.  

We study the properties of Lion-$\phi$ ODE \eqref{equ:lionode} by 
constructing Lyapunov functions, and 
analyzing its Hamiltonian and mirror descent components. In this section, we  assume that $\phi$ is continuous differentiable for technical simplicity; this is not a substantial restriction: We 
extend the results to non-smooth $\phi$ in continuous time in Section~\ref{sec:non-diff} 
and our results on discrete time analysis in Section~\ref{sec:disc_lion} requires no smoothness on $\phi$. 


We first prove the monotonicity of $H(x_t,m_t) = f(x_t) + \frac{1}{\alpha} \phi(m_t)$ following the ODE in \eqref{equ:lionode}. 
Recall that the Bregman divergence of a differentiable convex function $\phi$ 
is defined as 
$$B_\phi(x, y) 
= \phi(x) - \phi(y) - \dd \phi(y) \tt (x-y)\geq0. 
$$
Bregman divergence is not symmetric. One can define a symmetric Bregman divergence as 
$$
D_\phi(x,y) 
= B_\phi(x, y)  + B_\phi(y, x) 
= (\dd \phi(x) -\dd \phi(y)) \tt (x-y) \geq 0.  
$$

\begin{thm}
%In \eqref{equ:lionode}, assume 
%and that
Assume that 
$f$ and $\phi$ are differentiable and $\phi$ is convex with $\dd\phi(\vv 0)=\vv 0$,
and $\alpha, \eta, \beta >0$. 
Then following the trajectories of  \eqref{equ:lionode}, 
the Hamiltonian $H(\vv x,\vv m)$ decreases monotonically in that 
%in is reviewed a%
\bbb 
\label{equ:dh}
\begin{split}
 &\ddt  H(\vv x_t, \vv m_t) =
- \Delta(x_t, m_t) \leq 0, &  \\ 
%&&&& 
&D(x_t, m_t) = 
D_{\phi_{m_t,\beta}}( \dd f(\vv x_t), 0) 
+ \frac{\eta}{\alpha} D_\phi(\vv m_t, \vv 0), &
\end{split} 
\eee 
where 
$\phi_{m_t,\beta}(x) \defeq \frac{1}{\beta} \phi(m_t + \beta x). 
$
Moreover, % \red{more}
if $x=0$ is the unique minimizer of $\phi$,  
and $f,\phi$ are continuously differentiable, 
and $\{x \colon H(x,m) \leq H(x_0,x_0)\}$ is 
a compact set,  
then we have 
$m_t \to 0$ and $x_t \to x^*$ as $t\to+\infty$, where $x^*$ is a stationary point of $f$ with $\dd f(x^*)=0$.  
%the system must converge to a stationary point of $H(\vv x,\vv m)$%on which we have $\vv m =0 $ and $\dd f(\vv x) =0$. 
%\red{check coefficients} 
\end{thm} 
\begin{proof}
\bb 
\ddt H(\vv x_t, \vv m_t) 
& = \dd_{\vv x} H(\vv x_t, m_t) \tt \dot{\vv x}_t + \dd_{\vv m} H(\vv x_t, \vv m_t) \tt \dot m_t  \\
& =  -  \dd f(\vv x_t) \tt \dd \phi(\vv m_t + \beta \dd f(\vv x_t)) +  \frac{1}{\alpha} \dd \phi(\vv m) \tt (
\alpha \dd f(\vv x_t) - \eta \vv m_t)  \\
& =  - \dd f(\vv x_t) \tt (\dd \phi(\vv m_t + \beta \dd f(\vv x_t))  - \dd \phi(\vv m_t))   - \frac{\eta}{\alpha} \dd \phi(\vv m_t )\tt  \vv m_t \\
& = - 
D_{\phi_{m_t,\beta}}( \dd f(\vv x_t), ~ 0) - \frac{\eta}{\alpha}  D_{\phi}(\vv m_t, \vv 0) \leq 0. 
\ee 
%\bo{above misses the $\frac{1}{\alpha}$ term for the %$\eta\nabla \phi(m_t)^\top m_t$}
\iffalse 
Integrating on $t$ on both sides gives
\bb
\int_0^t %\frac{1}{\beta} D_\phi(\vv m_s+\beta \dd f(\vv x_s), \vv m_s)
D_{\phi_{m_t,\beta}}( \dd f(\vv x_t), ~ 0) 
+ 
 \frac{\eta}{\alpha} D_\phi(\vv m_s, \vv 0)\d s = 
 H(x_0,m_0) - H(x_t, m_t) 
 \leq H(x_0,m_0) - H^*, 
 %\frac{H(x_0,m_0) - H^*}{t}, ~~~~\forall t > 
\ee 
which leads to \eqref{equ:minDphi} when dividing both sides by $t$. 
\fi 

When  $m=0$ is the unique minimum point of $\phi(m)$, we have $\dd\phi(m)=0$ iff $m=0$.  %\bo{shouldn't we say when assuming $\dd\phi(m)=0$, $m=0$ is the unique minimum point of $\phi(\cdot)$?}. 
Hence, the invariant set of dynamics is 
\bb 
\mathcal S 
& = \{(x,m)\colon \dd\phi(m+\beta \dd f(x)) =0,  \dd f(x) = \eta m \} \\
& = \{(x,m) \colon \dd f(x)=0, m=0\}.
\ee 
Note that by the convexity of $\phi$ and that $0$ is the \emph{unique} minimum of $\phi$, 
$$D_\phi(\vv m_t, \vv 0)=\dd\phi(\vv m_t) \tt \vv m_t \geq \phi(m_t) - \phi(0) > 0,~~~ \forall m_t \neq 0. 
$$
%\bo{Why is the last inequality $>$ instead of $\geq$? we only assume $\phi$ convex and $\inf_m \phi(m) = 0$?}
Therefore, we have $\ddt H(\vv x_t, \vv m_t) <0$ outside of the invariant set. 
The convergence to the invariant set then follows La Salle’s invariance principle~\citep{lefschetz1961stability}. %\qq{Some extensions of Liapunov's second method}
%Hence, if $m=0$ is the unique minimum point of $\phi(m)$, we have $D(\vv m_t, \vv 0) =0$ iff $m_t = 0$.   
%The convergence 
\end{proof} 

\paragraph{Remark}
The $\Delta(x_t,m_t)$ can be viewed as 
an indication of the stationarity of the system. 
By integrating \eqref{equ:dh} with time, we can see that 
 the best  $\Delta(x_t, m_t)$ upto time $t$ decays with a $O(1/t)$ rate: %average: 
\bbb \label{equ:minDphi} 
\min_{s \leq t} \Delta(x_s, m_s) \leq 
\frac{1}{t}\int_0^t  \Delta(x_s, m_s) \d s
%\frac{1}{t}\int_0^t 
%\left \{ D_{\phi_{m_t,\beta}}(\dd f(x_s), 0)+  \eta D_\phi(\vv m_s, \vv 0)\right\} 
\leq \frac{H(x_0,m_0) - H^*}{t}, ~~~~\forall t > 0,
\eee  
 where we assume $H^* = \inf_{x,m} H(x, m) > -\infty$. 


\paragraph{Remark}
The two terms in $\Delta(x_t, m_t)$ correspond to the descend on $f$ and $\phi$, respectively. 
The $D_\phi(m_t, 0)$ term measures how far we are from the optimum $(m_t =0)$ of $\phi(m)$.  If $m_t = 0$, 

%\paragraph{Remark 1}The differentiability of $\phi$ is mainly to avoid distracting technical considerations here. It can be relaxed as we show in Section~\ref{sec:non-diff} where $\dd f$ should be interpreted as a subgradient of $f$. The discrete-time analysis also does not require differentiability and hence includes the $\phi(m) = \norm{m}_1$ case. 

%\paragraph{Remark 2}  Because $\frac{1}{\beta} D_\phi(\vv m_t + \beta \dd f(\vv x_t), ~ \vv m_t) + \eta D_{\phi}(\vv m_t, \vv 0) = 0$ implies $m_t =0$ and $\dd f(x_t) =0$, it serves as a indicator for the stationarity of the system. When $\phi(m) = \norm{m}_p^q$, we have $D_\phi(x,y) = q \norm{m}_p^{q}$, yielding  \red{...}
%\paragraph{Remark 3} 
%The two terms on the right hand side of \eqref{}.
To see the role of the gradient correction term $\beta \dd f(x)$, we consider the conformal Hamiltonian system \eqref{equ:ch}  employed in the Hamiltonian Descent~\citep{maddison2018hamiltonian}, 
which yields a similar result: 
$$
\ddt H(x_t, m_t) = - \eta D_\phi (m_t, 0) \leq 0, 
$$
which misses the negative term $ \frac{1}{\beta} 
D_\phi(\vv m_t + \beta \dd f(\vv x_t), ~ \vv m_t) $. 
Hence, introducing $\beta \dd f(x)$ 
is to introduce an additional .
%making the Hamiltonian decreases faster. 
As we show in Section~\ref{sec:hmd-descend-compo}, 
this can be viewed as introducing a special mirror descent on $f(x)$. 

%\qq{todo: prove convergence rate $ \min_{t\leq T}\phi(\dd f(x_T)) = O(1/T)$.}
%Hence, the 
%\qq{Discuss the relation with hamiltonian descent here. Sayig that it brings extra descent on $f$. }

\paragraph{Another Lyapunov Function}
%\subsection{Convex $f$}
\begin{thm}
\qq{either add $\alpha$, or say that $\alpha = 1$ for simplicity}

Assume $f$ is twice differentiable. 
Assume that $\phi$ is differentiable convex with $0$ as a minimum point.  
Define 
\bb 
\tilde H(x,m) =  (1+\eta \beta )f(x_t) +  \frac{1}{\alpha}\phi(m_t + \beta \dd f(x_t)). 
\ee 
Then, 
\bb 
\ddt \tilde H(x_t,m_t)  =  -\tilde \Delta(x_t, m_t), 
\ee 
with 
$$
\tilde \Delta(x_t, m_t) =  \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
+ \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t),  
$$
Hence, $\ddt \tilde H(x_t,m_t) \leq 0$ if $f$ is convex and $\beta, \eta\geq 0$. 
Moreover,  with $\tilde H^* = \inf_{x,m} \tilde H(x,m)$, 
%which gives 
\bb 
 %\eta \dd \phi(\tilde m_t) \tt \tilde m_t  
 \min_{s\leq t} \left\{  \eta D_\phi(\tilde m_s, 0) 
 + \beta \dd\phi(\tilde m_s) \tt \dd^2 f(x_s)  \dd\phi(\tilde m_s)  \right \}  \leq \frac{\tilde H(x_0,m_0) - \tilde H^*}{t}. 
\ee 
\end{thm} 

\paragraph{Remark} 
An interesting feature of this Lyapunov function, 
when $f$ is convex and $\beta>0$, is that it provides control 
on the Hessian related term $H_t \defeq \dd\phi(\tilde m_t) \tt \dd ^2 f(x_t) \dd \phi(\tilde m_t)$, 
which coincides with the notion of 
\emph{directional sharpness} proposed in \citep{pan2023toward} 
for characterizing the benefit of adaptive gradient methods. 
We can see that larger $\beta$ provides stronger control on directional sharpness. 

%\paragraph{Remark} 


\begin{proof}
Write $\tilde m_t = m_t + \beta \dd f(x_t)$. Note that 
\bb 
\ddt f(x_t)   &  = - 
\dd f(x_t)\tt \dd\phi(\tilde m_t) \\ 
%\ddt \phi(m_t) & = \dd \phi(m_t) \dd f(x_t) - \eta \dd \phi(m_t) m_t  \\ 
\ddt \phi(\tilde m_t) 
& = 
\dd \phi(\tilde m_t) \tt \dd f(x_t) 
- \eta \dd \phi(\tilde m_t) \tt m_t  
- \beta  \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) \\
& = 
\dd \phi(\tilde m_t) \tt \dd f(x_t)
- \eta \dd \phi(\tilde m_t) \tt (\tilde m_t  - \beta \dd f(x_t))
- \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) \\ 
& = 
(1 + \eta \beta) \dd \phi(\tilde m_t) \tt \dd f(x_t) 
- \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
- \beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t). 
\ee 
Hence, 
\bb 
\ddt \tilde H(x,m) & =
 (1+\eta \beta) (- \dd f(x_t) \tt \dd \phi(\tilde m_t) )   \\ 
& ~~~ + (1 + \eta \beta) \dd \phi(\tilde m_t) \tt \dd f(x_t) 
- \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
-\beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t) \\ 
& =  - \eta \dd \phi(\tilde m_t) \tt \tilde m_t  
-\beta \dd\phi(\tilde m_t) \tt \dd^2 f(x_t)  \dd\phi(\tilde m_t)  \leq 0. 
\ee 
\end{proof} 

\section{\lion{} as a Hamiltonian Mirror Descent}
\label{sec:hamiltonian-mirror-descent}


\begin{figure}[h!]
    % \centering
    \includegraphics[width=\textwidth]{figures/quadratic.pdf}
    \caption{From left to right: iteration trajectories, $f(x)$, $\phi(m)$, and $H(x,m)$ of Lion, LionL2, and LionL3 methods for minimizing $f(x_1,x_2) = x_1^2 + x_2^2$, from the initial value $(4.7, -3.0)$ and initial momentum $m = (0,0)$. Monotonicity of $H(x, m)$: The Hamiltonian function $H(x, m)$ exhibits a monotonically decreasing behavior during the optimization process. As the optimization progresses, $H(x, m)$ decreases, reflecting the convergence of the algorithm.
    }
    \label{fig:quadra}
\end{figure}


We now introduce the decomposition \eqref{equ:decomp} 
of the  \lion{}-$\phi$ ODE as the sum of a Hamiltonian component and mirror descent component. 
We first characterize 
the space of algorithms 
whose convergence can be verified by the monotonic decreasing of a Laypunov function, 
and then locate \lion{}-$\phi$ as a special case. 

\subsection{The Lyapnunv verifiable algorithm space}
We describe a general procedure for constructing convergent algorithms for minimizing $f(x)$. 
The first step is to introduce 
a Hamiltonian like function $H(x,m)$ with an auxiliary momentum-like variable $m$, such that minimizing $f$ reduces to minimizing $H(x,m)$, that is, if $(x^*, m^*)$ minimizes $H(x,m)$ then $x^*$ minimizes $f(x)$. 
Obviously, $H(x,m) = f(x) + \frac{1}{\alpha} \phi(m)$ satisfies this condition, for any function $\phi$. 
Introducing $H$ allows us to deal with momentum-based algorithms that monotonically decrease  $H(x,m)$, but not necessarily the original loss $f(x)$. 

Let $z = [x,m]$. We are interested in systems $\dot z = v(z)$ that monotonically decreases $H$ in that 
$$
\ddt H(z_t) = \dd H(z_t)\tt v(z_t)  \leq 0. 
$$
The velocity field $v$ can always be decomposed into the 
$$
v(z) = v_{\perp}(z) +  v_{\parallel}(z), 
~~~~~~ v_{\perp}(z)\tt \dd H (z)=0,~~~~~~~ 
v_{\downarrow}(z) \tt \dd H(z) \leq 0, 
$$
where $v_{\perp}$ is orthogonal 
to $\dd H$ and hence keeps $H$ invariant, and $v_{\downarrow}$ has negative inner product with $\dd H$ and is responsible for decreasing $\dd H$. We just need to design the $v_{\perp}$ and $
v_{\downarrow}$ parts separately. 

\subsubsection{The Conservative component}
Following the sub-system $\dot z_t = v_\perp(z_t)$, 
the Hamiltonian is kept invariant in as $\ddt H(z_t) = \dd H(z_t) \tt v_\perp(z_t) =0$. 
A general approach to construct such directions, as employed in Hamiltonian systems, is 
$$v_{\perp}(x) = A_t(z) \dd H(z_t),$$
where $A_t$ is a skew-symmetric matrix satisfying $A_t\tt=-A_t$; in this case we have $\dd H \tt v_{\perp} = (\dd H)\tt A (\dd H) = (\dd H)\tt A\tt (\dd H)  = - (\dd H)\tt A (\dd H)  = 0.$  
%$g \tt A_t g = 0$ for any $g\in \RR^d$. This would give $\dd H\tt A\dd H = 0$.

In particular, for $H(x,m)= f(x)+\frac{1}{a}\phi(m)$ with $m,x\in \RR^d$, we obtain the Hamiltonian component of Lion-$\phi$ in \eqref{equ:decomp} via 
\bb 
A = 
\begin{bmatrix}
I & -I  \\ 
- I & I 
\end{bmatrix}&& 
v_{\perp}(z) = \begin{bmatrix} 
- \dd_m H(x,m)  \\
\dd_x H(x,m) 
\end{bmatrix} 
\propto \begin{bmatrix} 
- \dd \phi(m_t)  \\
\alpha \dd f(x_t)
\end{bmatrix}. 
\ee 


\subsubsection{Descending component}
\label{sec:hmd-descend-compo}
In general, the descending (or dissipative) component $v_{\downarrow}$ can be expressed as 
$$
v_{\downarrow}(z) =  - \psi_t(\dd H(z)), 
$$
where $\psi_t\colon \RR^d \to \RR^d$ is a monotonic operator satisfying $\psi_t(z) \tt z  \geq  0$ and $\psi_t(0) =0$. 
One rich family of monotonic operators 
are subgradients of convex functions %\bo{shall we use $\phi$ instead of $h$?}: 
%is when $\psi(z) = \dd h(z)$ where $h$ is a convex function with $\dd h(0) =0$, yielding 
\bb 
v_\downarrow(z) = - \dd \Phi_t(\dd H(z)),  
&&& \text{where $\Phi_t\colon \RR^d\to \RR$ is convex and $\dd \Phi_t(0)=0$.}
\ee 
Following $\dot z_t  = v_{\downarrow}(z_t)$, 
the decreasing rate of the objective $H(z_t)$  equals the symmetric Bregman divergence of $\Phi_t$: % $D_{\Phi_t}(\dd H(z_t),0)$: 
\bb
\ddt H(z_t) = - \dd \Phi_t(\dd H(z_t)) \tt \dd H(z_t) = -D_{\Phi_t}(\dd H(z_t), 0) \leq 0.
\ee 
Such $v_{\downarrow}$ 
can be derived from mirror descent as a local steepest descent procedure: 
assume we update $z_t$ via $z_{t+\epsilon} = z_t - \epsilon \delta_t$, 
$\epsilon$ is a small step size and 
 $\delta_t $  solves 
% on $f$ with $h^*$ as the 
%Such directions can be 
%The discretizating the descending component  $\dot z_t = v_\downarrow(z_t)$ yields $z_{t+1} - z_t = - \epsilon  \dd h(\dd H(z)) $, it can bederived as a steepest descent that yields the best local descend on $f$ subjecting to $h^*(x)$ the penalty function:  
%a proximal gradient descent: 
%This yields the family of mirror descent. 
\bbb \label{equ:mirror} 
\delta_t =\argmin_{\delta} \bigg \{ H(z_t +\delta) +  \Phi_t^*\left (-\frac{\delta}{\epsilon}\right )  \bigg \} \approx 
\argmin_\delta 
\bigg \{  \dd H(z_t) \tt \delta +  \Phi_t^*\left (-\frac{\delta}{\epsilon}  \right )  \bigg \}, 
\eee  
yielding $\delta_t = - \dd \Phi_t(\dd H(z_t)) $, where $\Phi_t^*$ is the conjugate function of $\Phi_t$.   
\paragraph{Remark}
For convex $H$ with conjugate $H^*$, 
the ideal choice of $\Phi_t$ is the Bregman divergence of $H^*$, i.e., $\Phi_t(z) =  B_{H^*}(z, 0)$,   because in this case $v_{\downarrow}(z) = -(z-z\opt)$, 
$v_{\downarrow}$ always directly point to 
the minimum of $H$. 
Specially, when $H,H^*$ are differentiable, 
and $z\opt$ the unique minimum point of $H$, we have with $\Phi_t(z) =  B_{H^*}(z, 0)$, 
%directly pointing to the optimal point $z\opt$ of $H$.  
%\begin{pro}
%Let $H^*$ be the convex conjugate of $H$ and both $H$ and $H^*$ are differentiable and convex. Let $z\opt$ be the unique minimum point of $H$,  and $\Phi_t(z) = B_{H^*}(z,0)$, then 
\bb 
\dd \Phi_t(z) = \dd H^*(z) - \dd H^*(0) = \dd H^*(z) - z\opt, 
&&\text{and hence}
&&
v_{\downarrow}(z) = z - z\opt. 
\ee 
%\end{pro}

For Lion-$\phi$, the descending component in \eqref{equ:decomp} is  
we have 
\bb 
\dot x_t & = - \dd\phi(m_t + \beta \dd f(x_t)) + \dd\phi(m_t) \\
\dot m_t & =  - \eta m_t, 
\ee 
which corresponds to using
\bb
\dd \Phi_t([g_x, g_m]) = \begin{bmatrix} 
\dd \phi(m_t +  \beta g_x) - \dd\phi(m_t)  \\
\red{\eta }\dd\phi^*(\red{\alpha} g_m) 
\end{bmatrix} , &&
\forall [g_x, g_m] \in \RR^{2d}, 
\ee 
where we used $m = \dd \phi^*(\dd\phi(m))$ for the $m$ component and set $\alpha = 1$. Correspondingly, we should take $\Phi_t$ to be  a sum of two Bregman divergences as follows 
%and hence 
\bb 
\Phi_t([g_x,g_m])
& =\frac{1}{\beta}
\left ( \phi(m_t + \beta g_x) -  \phi(m_t)  - \beta  \dd  \phi(m_t)\tt  g_x    \right )+ \red{\eta} \phi^*(\alpha g_m)  \\
& = \frac{1}{\beta} B_\phi(m_t+\beta g_x, m_t) + \red{\eta} B_{\phi^*}(\red{\alpha} g_m, 0),  
\ee 
where $B_{\phi^*}(m, 0) = \phi^*(m)$ 
because $\phi^*(0) = 0$ and $\dd\phi^*(0)=0$ 
when $\phi(0)= 0$ and $\dd \phi(0)=0$; see Appendix~\ref{sec:ht}.  
 %where we note that $\dd\phi^*(\dd\phi(m))=m$. 
 The conjugate $\Phi_t^*$ of $\Phi_t$ is  
\bb 
\Phi_t^*([x, m]) = \frac{1}{\beta} B_{\phi^*}(\dd\phi(m_t) + y, \dd\phi(m_t)) + 
\red{\eta} B_\phi\left (\frac{m}{\red{\alpha \eta}}, 0 \right ). 
\ee
See Appendix~\ref{sec:ht} for the derivation. 

\red{
We can see that $\phi^*$ already employ the optimal convex function $B_{\phi^*}(\cdot, 0)$, 
but the descent on $x$ would be good if $\phi(m_t + \beta x) - \phi(m_t)$ is close to the conjugate $f^*(x)$ of the loss function.
}





\section{Discrete Time Analysis}\label{sec:disc_lion}

Consider the following semi-implicit Euler scheme of \eqref{equ:lionode}:  
\bb 
m_{t+1} &= \beta_2 m_t +  (1- \beta_2) \dd f(x_t) \\
x_{t+1} &= x_t - \epsilon\dd\phi( m_{t+1} + \beta \dd f(x_t)),
\ee 
where $\epsilon >0$ is the step size. For initialization, we assume $m_{0} = 0$. 

\begin{thm}\label{thm:strong_smooth}
Assume $f$ is $L$-smooth and lower bounded ($\inf_x f(x) >-\infty$), and $\phi$ is convex. Let  $\dd \phi$ be a subgradient of $\phi$ with $\dd \phi(0) = 0$.  Assume $D\defeq \sup_t \norm{\dd\phi(m_t)}_2  < +\infty$. 
We have 
$$
\frac{1}{T+1}\sum_{t=0}^T 
%\frac{1}{\beta} D_\phi(\tilde m_{t+1}, m_{t+1}) 
D_{\phi_{m_t,\beta}}(\dd f(x_t), 0) 
+  D_\phi(m_{t+1},0) \leq \frac{A}{\epsilon (T+1)}  + B \epsilon, 
%= O\left (\frac{1}{\epsilon T} + \epsilon  \right ), 
%\frac{(H_0 - H_{T+1}) + \frac{L d \epsilon^2}{2} }{\epsilon T}. 
$$ 
where $A = f(x)  - \inf_x f(x)$, 
and $B = L D^2/2$. 
\end{thm}
 
%\subsection{\red{Try to use a weaker smoothness condition: with constant $\beta_2$}}

\subsection{Weaker Smoothness on $f$}
\begin{mydef}
$\phi\colon \RR^d\to \RR$ is said to be $q$-homogeneous for $q\in\RR$ if 
\bb 
\phi(a x) = \abs{a}^q \phi(x) 
~~~~~\text{for any $x\in\RR^d$, $a \in \RR$}. 
\ee 
\end{mydef}
The canonical example is when $\phi(x) = \norm{x}^q$ for some norm $\norm{\cdot}$. 
% is  norm function. \red{See Section \red{XXX} for examples.}
 
\begin{mydef}[Weak Smoothness] 
We say that  $f\colon\RR^d\to\RR$ is $\phi$-weak smooth if there exists $L_0,L_1<+\infty$ and $L_3 > 0$, such that when $\norm{x - y}_2\leq L_3$, 
$$
f(y) - f(x) 
\leq   \dd f(x)\tt (y-x)  +
\frac{1}{2} (L_0 + L_1 \phi(\dd f(x))) \norm{y-x}^2_2. 
%~~~~\forall x,y\in\RR^d.
$$
%for some $L_0,L_1 <+\infty$. 
\end{mydef} 

\begin{thm}\label{thm:weaksmooth}
Assume $f$ is $\phi$-weak smooth  as above  
and lower bounded ($\inf_x f(x) >-\infty$), and $\phi$ is convex and $q$-homogeneous for $q\in\RR$. Let  $\dd \phi$ be a subgradient of $\phi$ with $\dd \phi(0) = 0$.  Assume $\sup_t \norm{\dd\phi(m_t)}_2\defeq D < +\infty$. 
We have when $\epsilon \leq \min\left (\frac{L_3}{D}, \frac{1}{\bar L_1} \left (\frac{1-\beta_2}{1+\beta_2}\right)^q \right )$,
$$
\frac{1}{T+1}\sum_{t=0}^T 
\red{D_{\phi_t,\beta}(\dd f(x_t), 0)} 
+  \frac{\beta}{2}D_\phi(m_{t+1},0)
%= O\left (
\leq 
\frac{A}{\epsilon T} + B \epsilon, 
%\frac{(H_0 - H_{T+1}) + \frac{L d \epsilon^2}{2} }{\epsilon T}. 
$$ 
where $\phi_{m_t,\beta}(x) = \phi(m_t + \beta x),$ and 
where $A = \beta (f(x_0) - \inf_{x} f(x))$  and $B = \beta L_0 D^2/2$. 
\end{thm}
\paragraph{Remark}
The $O(\epsilon)$ term is due to discretization. It can be eliminated by assuming $\dd\phi(m)$ is continuous, which, however, 
does not include the important case when $\phi$ is a norm function, i.e., $\phi(m) = \norm{m}$, which is discontinuous at $m=0$.

In fact, due to the binary gradients, 
after the discretization, \lion{} can converge at best in the range $\gamma$ ball of the optimal solution.
Hence, in practice, it is advised to set a small step size for \lion{} (suggested $\gamma=1e-4, 3e-5$ in the \lion{} paper~\citep{chen2023symbolic}), 
and using decaying learning rates. 

\paragraph{Remark} 
This result provides a control on the gradient magnitude $\phi(\dd f(x_t))$, because, by Lemma~\ref{lem:m2df}, we have under conditions of Theorem~\ref{thm:weaksmooth}, 
$$
\sum_{t=0}^T \phi(\dd f(x_t)) 
%\leq \left (\frac{1+ \beta_2}{\bar\beta_2}\right)^q \sum_{t=0}^T \phi(m_{t+1}) 
\leq \left (\frac{1+ \beta_2}{1-\beta_2} \right)^q \sum_{t=0}^T D_\phi(m_{t+1}, 0). 
$$




\begin{thm}\label{thm:weaksmooth2}
Assume $f$ is $\phi$-weak smooth  as above  
and lower bounded ($\inf_x f(x) >-\infty$), and $\phi$ is convex and $q$-homogeneous for $q\in\RR$. Let  $\dd \phi$ be a subgradient of $\phi$ with $\dd \phi(0) = 0$.  Assume $\sup_t \norm{\dd\phi(m_t)}_2\defeq D < +\infty$. 
We have when $\epsilon \leq \min\left (\frac{L_3}{D},  \frac{1}{\kappa L_1(1+\beta)} \left(\frac{1-\beta_2 + \beta}{1 + \beta}\right)^q  \right )$,
\bb
\frac{1}{T+1} \sum_{t=0}^T D_\phi(\tilde m_{t+1}, 0)  \leq 
\frac{\tilde A}{\epsilon (T+1)} + \frac{\epsilon D^2}{2}\tilde B
\ee
where $\tilde A = 2(1+\beta)(f(x_0) - \inf_{x} f(x))(1+\epsilon)$  and $\tilde B =2(1+\beta) L_0 D^2/2$. 
\end{thm}
\paragraph{Remark}
The $O(\epsilon)$ term is due to discretization. It can be eliminated by assuming $\dd\phi(m)$ is continuous, which, however, 
does not include the important case when $\phi$ is a norm function, i.e., $\phi(m) = \norm{m}$, which is discontinuous at $m=0$.

\paragraph{Remark} 
This result provides a control on the gradient magnitude $\phi(\dd f(x_t))$, because, by Lemma~\ref{lem:tmbound}, we have under conditions of Theorem~\ref{thm:weaksmooth2}, 
$$
\sum_{t=0}^T \phi(\dd f(x_t)) 
\leq \left(\frac{1+\beta}{1-\beta_2 + \beta}\right)^q \sum_{t=0}^T\left( D_\phi(\tilde m_{t+1}, 0) + \beta D_\phi(m_{t}, 0)\right)
$$
\qq{transfer the bound with $\beta = (1-\hat\beta_1)/\hat\beta_1$?}

% \subsection{\red{Try another way to control $\dd f$ with $m_t$}}

% We have $m_t = \beta_1 \sum_{s =0}^t (1-\beta_1)^{t-s} g_{s}$. 

% \bb 
% m_t - \beta_1 \frac{1-\beta_1^t}{1-\beta_1} g_t 
% & = \beta_1 \sum_{s =0}^t (1-\beta_1)^{t-s} (g_{s} - g_t) \\
% & = \beta_1 \sum_{s =0}^t (1-\beta_1)^{t-s} (L_0 + L_1 \phi(g_t)) \norm{x_t - x_s} \\ 
% & = \beta_1 \sum_{s =0}^t (1-\beta_1)^{t-s} (L_0 + L_1 \phi(g_t)) (t-s) \epsilon D. .... 
% \ee 



% \section{Strongly Convex Analysis}
% \textbf{\red{TODO}} 


==> old_content/notes.tex <==






\newpage \clearpage 
\bb
H_\rho (x, m)
& = H(x, m) +  \rho  m \tt (x - x^*) \\
\ee 

$0=\phi(0) \geq \phi(m) - \dd\phi(x) m $.
So $\dd\phi(m) m \geq \phi(m) - \phi(0).$

$$
B_\phi(u,v) 
= B_\phi(w,v) + B_\psi(u,w) 
+ (\dd \psi(w) - \dd \psi(v))\tt(u-w). 
$$
$$
(\dd \psi(w) - \dd \psi(v))\tt(w-u)
= B_\phi(w,v) + B_\psi(u,w) - B_\phi(u,v) 
$$


\bb 
\dot H _\rho 
= -\dd f (\dd \phi(m + \beta \dd f) - \dd \phi(m)) - \eta \dd \phi(m) m 
+ \rho (\dd f - \eta m) (x - x^*) 
+ \rho m (- \dd\phi(m + \beta \dd f))
\ee 

\newpage
\clearpage

\section{ Lion as Hamiltonian + Mirror descent}

\subsection{Background} 
Let us recall basic mirror descent on $f(x)$. 
Define Bregman divergence: 
$$
D_h(x'; x) = h(x') - h(x) - \dd h(x) (x '- x).
$$
Let us consider the following update: 
$$
x' = \argmin_{x'} \dd f(x) \tt(x' - x)  + \frac{1}{\alpha} D_h(x'; x). 
$$
Zero gradient yields
$$
\dd f(x) + \frac{1}{\alpha} (\dd h(x') - \dd h(x)),
$$
yielding 
$$
x' = \dd h^{-1}( \dd h(x) - \alpha \dd f(x)). 
$$

\subsection{Lion as a Hamiltonian Mirror Descent }
Let us consider the steepest descent of $H(x, m) = f(x) + \phi(m)$ under the following metric:
\bb 
D((x', m'), (x, m)) = 
& \frac{\epsilon}{\alpha}
\bigg \{
\phi^*( \dd \phi(m) - \epsilon^{-1}(x' - x)) - \phi^*(\dd \phi(m))  + m \tt (\epsilon^{-1} (x' - x)  ) \bigg \} \\
& +  
\frac{\epsilon}{\eta}\bigg \{
 \phi( -\frac{1}{\epsilon}( m' - m) )- \phi(0) +  \dd \phi(0)\tt \frac{1}{\epsilon} (m'-m) \bigg \}  \\
 & 
 B_{\phi^*}
 (\dd \phi(m) + 
 )
%B_\phi(m + (x' - x), m)  + B_\phi(m', m). 
\ee 
where $B_\phi(x, y) = \phi(x) - \phi(y) - \dd \phi(y)\tt (x - y)$ is the Bregman divergence. 
So we consider the update of form
$$
(x', m') = \argmin_{x',m'} 
\dd f(x) \tt (x' - x) + \dd \phi(m)\tt (m' - m)
+ D((x', m'), (x, m)) 
% B_\phi(m + (x' - x), m)  +    \frac{1}{\alpha } B_\phi(m', m). 
$$
Taking zero gradient w.r.t. $x'$:  
\bb 
& \dd f(x) - \frac{\epsilon}{\alpha} ( \epsilon^{-1} \dd \phi^*( m+ \epsilon^{-1}( x' - x)) - \epsilon^{-1} m ) = 0 \\
\ee 
Yielding 
\bb
& \dd f(x) - \frac{1}{\alpha} (\dd \phi^*( \dd\phi(m)- \epsilon^{-1}( x' - x)) - m ) = 0 \\
\implies & m + \alpha \dd f(x) =\dd \phi^*( \dd\phi(m) - \epsilon^{-1}( x' - x))  \\
\implies & \dd \phi(m + \alpha \dd f(x)) =\dd\phi( m) - \epsilon^{-1}( x' - x) \\ 
\implies & x' = x - \epsilon( \dd \phi(m + \alpha \dd f(x)) - \phi(m))  \\ 
\ee
\bb 
x' =  x - \epsilon(\dd\phi( \dd\phi( m) +  \alpha \dd f(x)) - \phi(m) )\\ 
\ee
Taking gradient w.r.t. $m'$:
\bb
&  \eta \dd \phi(m) -  \dd \phi(- \epsilon^{-1} (m' - m)) + \dd \phi(0) = 0\\
\implies & \eta \dd \phi(m)  + \dd \phi(0) =  \dd \phi(- \epsilon^{-1} (m' - m))  \\
\implies & \dd \phi^{-1}(\eta \dd \phi(m)  + \dd \phi(0)) =  - \epsilon^{-1} (m' - m)   \\
\implies & - \epsilon \dd \phi^{-1}(\eta \dd \phi(m)  + \dd \phi^*(0)) =  (m' - m)   \\
\implies &  m' = m - \epsilon \dd \phi^{-1}(\eta \dd \phi(m)  + \dd \phi(0)) \\
%(\dd \phi(m') - \dd \phi(m))  = 0.
\ee 
Assume $\dd\phi(0) = 0$ and  $\eta =1$, yielding 
$$
m' = m - \epsilon m. 
$$
%Hence, taking derivative
Hence, in the limit when $\epsilon \to 0$, we have 
\bb 
\dot x_t  & = - \dd \phi(m_t + \alpha \dd f(x_t)) + \dd\phi(m_t) \\
\dot m_t  & =  - m_t.
\ee 
On the other hand, the Hamiltonian of $H(x,m) = f(x) + \phi(m)$ is 
\bb
\dot x_t = - \dd\phi(m_t) \\
\dot m_t =  \dd f(x_t)
\ee
Adding them together with 
\bb
\dot x_t  & = - \dd \phi(m_t + \alpha \dd f(x_t)) \\
\dot m_t  & = \dd f(x_t)  - m_t.
\ee 


==> old_content/notes_2.tex <==

\href{run:2023-04-10.tex}{\Huge April 10} %##@@TitleDateString@@##

\section{Try to Understand Lion}

\url{https://arxiv.org/pdf/2302.06675.pdf} 

The update is 
\bb 
 & update = (1-\beta_1) \times gradient + \beta_1 \times  momentum  \\ 
& update = sign(update)  \\ 
& momentum = (1-\beta_2) \times gradient + \beta_2 \times momentum \\ 
&   update = update \times  lr.
\ee 
Default: $\beta_2 = 0.99$ and $\beta_1 = 0.9$. 
Examples of learning rate: $lr = 10^{-4}$, $3\times 10^{-5}$. 


\begin{enumerate}
\item Make sense: \emph{``This choice of EMA factor and interpolation allows Lion to balance between remembering a $\sim $10x longer history of the gradient in momentum and putting more weight on the current gradient in the update."} 

\item It reduces to SignGrad when $\beta_2 = 0 $, and to SignMomentum when $\beta_2 = 1.$ 
So in some sense it is the combination of the two. 
\red{but another way to combine is $update =  (1-\beta_2) sign(grad) + \beta_2 sign(momentum)$,
or $update = sign( (1-\beta_2) sign(grad) + \beta_2 sign(momentum))$.} 

\item \emph{``Users should be aware that the uniform update calculated using the sign function usually yields a larger norm compared to those generated by SGD and adaptive methods. Therefore, Lion requires a smaller learning rate lr, and a larger decoupled weight decay $\lambda$ to maintain the effective weight decay strength. "} 

\item \emph{``our experiments show that the gain of Lion increases with the batch size and it is more robust to different hyperparameter choices compared to AdamW"}

\item \emph{``For limitations, the difference between Lion and AdamW is not statistical significant on some large-scale language and image-text datasets. The advantage of Lion is smaller if using strong augmentations or a small batch size (<64) during training." }
\end{enumerate}

$$
m_{t+1} = 0.99 m_t + 0.01 g_t. 
$$

\bb 
& m_0 = 0 \\ 
& m_1 =  0.01 g_0  \\
& m_2 =  0.99 \times  0.01 g_0 + 0.01 g_1 \\ 
& m_3 = 0.99\times  0.99 \times  0.01 g_0 + 0.99\times  0.01 g_1 + 0.01 g_2 \\
\ee 

$$
m_{t+1} = (1-\beta_2)\left ( g_t  + \beta_2 g_{t-1} + \cdots +  \beta_2^t  g_0 \right).
$$
If $t$ is very large, then we have approximately
$$
m_{t+1} \approx \frac{ g_t  + \beta_2 g_{t-1} + \cdots +  \beta_2^t  g_0 }{1  + \beta_2  + \cdots +  \beta_2^t }.
$$

\bb 
v_{t+1} 
& =(1-\beta_1) g_{t+1} +  \beta_1 m_{t+1} \\ 
& =(1-\beta_1) g_{t+1} +  \beta_1(1-\beta_2)\left ( g_t  + \beta_2 g_{t-1} + \cdots +  \beta_2^t  g_0 \right)
\ee 


\bb
m_{t+1} 
& = (1-\beta_2)\left ( g_t  + \beta_2 g_{t-1} + \cdots +  \beta_2^t  g_0 \right) \\ 
& =  0.01 \times \left (g_t + 0.99 g_{t-1} + 0.98 g_{t-2} + \cdots \right )
\ee 

\bb 
v_{t+1}
&  = 0.1 g_{t+1} +  0.9 m_{t+1} \\
& = 0.1 g_{t+1} + 0.9 \times  0.01 \times \left (g_t + 0.99 g_{t-1} + 0.98 g_{t-2} + \cdots \right ) \\
& = \med{0.1 g_{t+1}} +\blue{ 0.009  g_t + 0.0089 g_{t-1} + 0.0088 g_{t-2} +  0.0087 g_{t-3} + \cdots } \\
\ee 
The final update is 
$$
\boxed{update_{t+1} = \sign\left ( \med{0.1 g_{t+1}} + \blue{0.009  g_t + 0.0089 g_{t-1} + 0.0088 g_{t-2} +  0.0087 g_{t-3} + \cdots } \right ).}
$$

\red{So  $g_{t+1}$ is weighted 10 times more than $g_t$. There is a cliff  drop of the weights from $g_{t+1}$ to $g_t$. 
How about we delay the cliff drop to be between $g_{t-k}$ and $g_{t-k-1}$ for some $k$? How about } 

\bb 
 & update = (1-\beta_1) \times ( g_t  +\red{ \eta_1  g_{t-1} +  \cdots  \eta_k g_{t-k}}) + \beta_1 \times  m_t  \\ 
& update = sign(update)  \\ 
& m_{t+1} = (1-\beta_2) \times g_t + \beta_2 \times m_t \\ 
&   update = update \times  lr.
\ee 

This can be viewed as introducing a $\beta_3$? 
\bb 
 & update = (1-\alpha_1 - \alpha_2 ) \times  g_t   +  \alpha_1 \times  m_t  + \alpha_2 \times n_t \\ 
& update = sign(update)  \\ 
& m_{t+1} = (1-\beta_2) \times g_t + \beta_2 \times m_t \\ 
& n_{t+1} = (1-\beta_3) \times g_t + \beta_3 \times n_t \\ 
&   update = update \times  lr.
\ee 



==> old_content/related.tex <==
\iffalse 
\section{Related Work}
\label{sec::related}

\paragraph{SIGN and Double-$\beta$}
The sign operation adds noise to the updates, which acts as a form of regularization and helps with generalization\cite{chen2022vision,298623}. There have been many popular Sign-based algorithms~\cite{bernstein_signsgd_2018, crawshaw_robustness_2022,298623}. 
SignGD~\cite{bernstein_signsgd_2018} is an algorithm that follows the negative gradient sign direction to perform the update. \cite{crawshaw_robustness_2022} provided a generalized SignSGD algorithm, which recovers the SignSGD with the Momentum algorithm, but ~\cite{bernstein_signsgd_2018,crawshaw_robustness_2022} have a different momentum update rule from \lion{}, which is the double-$\beta$ scheme. 
\cite{sun2023momentum} provides a convergence theory that does not require the assumption of bounded stochastic gradient or increased batch size.


\paragraph{Hamiltonian Dynamics and Mirror Descent}
\cite{maddison2018hamiltonian}  looks at the continuous time ODE limit of optimization methods from a Hamiltonian perspective. \cite{jin_accelerated_2017} introduced Hamiltonian to get a convergence rate of stationary points. Mirror Descent~\cite{tzen2023variational} exhibits an efficiency estimate that is mildly dependent in the decision variables dimension, and thus suitable for solving very large scale optimization problems~\cite{krichene_accelerated_2015,tzen2023variational}.


\paragraph{Distributed Training}

Researchers have made significant strides in overcoming the communication bottleneck in distributed training, focusing on asynchronous SGD~\cite{chen2016revisiting}, gradient quantization, and sparsification. Asynchronous SGD speeds up training by immediate parameter updates, while gradient quantization techniques like 1-bit SGD~\cite{seide20141}, QSGD~\cite{alistarh2017qsgd}, and TernGrad~\cite{wen2017terngrad} reduce communication bandwidth. Gradient sparsification approaches, including threshold quantization and Gradient Dropping~\cite{aji2017sparse}, allow selective sending of significant gradients~\cite{aji2017sparse}. Recently, Deep Gradient Compression (DGC)~\cite{lin2017deep} utilizes momentum correction, local gradient clipping, momentum factor masking, and warm-up training to preserve accuracy but causes higher computation cost.
\fi 
